Bankruptcy Shocks and Legal Labor Markets: Evidence from the Court Competition Era

We study how Chapter 11 bankruptcies affect local legal labor markets. We document that bankruptcy shocks increase county legal employment and corroborate this finding by exploiting a stipulation of the law known as Forum Shopping during the Court Competition Era (1991-1996). We quantify losses to local communities from firms forum shopping away from their local area as follows. First, we calculate the unrealized potential employment gains implied by our reduced-form results. Second, we structurally estimate a model of legal labor markets and quantify welfare losses. We uncover meaningful costs to local communities from lax bankruptcy venue laws.

==> Drafts/Avg_Wage.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    \subsection{Bankruptcy Shocks and Legal Wages}\label{sec:wag}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Thus far we have shown the effect of bankruptcy shocks on local legal sector employment. We complete our analysis by studying the effect on average wages.
    
    \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE_noBRsplit}{tab:avg_wage_reg_noBRsplit}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}

    
    Table \ref{tab:avg_wage_reg_noBRsplit} reports a \textit{negative} and non statistically significant effect of bankruptcy shocks, both in our benchmark model (Column (1), model \eqref{eq:spec_bench_BR}) or we account for forum shopping (Column (2), model \eqref{eq:spec_bench_BR}).
    
% \marginpar{\scriptsize{\textcolor{red}{If our story is that the shock means that avg wage goes down b/c more unskilled labor is hired do sticky wages matter?}}}
    
    Before discussing the sign of our findings, we explore their significance. Prices tend to be stickier than quantities (CITATION HERE ON PAPER WITH STICKY WAGE ESTIMATION). Hence, larger shocks may be needed in order to trigger a general equilibrium effect (EXAMPLES OF PAPER WHEN THIS HAPPENED).
    We explore this idea in Column (3) by splitting bankruptcy and forum shopping in Lopucki (large firms' bankruptcies) and Compustat (small firms' bankruptcies) group.
    Consistent with this interpretation, we find a statistically significant effect for the large (Lopucki) bankruptcy group, but not in the small group. 
    
    Similar to the results on employment level, Table \ref{tab:avg_wage_reg_noBRsplit} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had.
    
    The sign of our finding is puzzling. Bankruptcy shocks are demand shocks to the level of legal services. Basic economic theory would suggests the associated increase in the conditional input factor demands to increase wages, not decrease them. 
    Next section uses a model with skilled and unskilled workers to reconcile this finding via a compositional channel.
    Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %, i.e. quantity in the market for labor in the legal sector. 
%     %In this section we investigate bankruptcy shocks impact on price levels in the form of average wage to get a more complete picture of how legal sector labor markets respond to bankruptcy shocks.
    
%     In this section we investigate the effect on the average wage.
%     However, it is much more difficult to measure the impact of labor demand shocks on wage than on employment levels, because wages tend to be ``stickier'' than employment levels in the short run. Consistent with this predicted ``stickiness'' our results in Table \ref{tab:avg_wage_reg_noBRsplit} show a much smaller impact on wages than we saw on employment levels, and in turn lower significance with only column (3) estimating a significant impact from the bankruptcy shocks. 
    
%     Yet, despite the minimal significance, the direction of the estimated effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
%     Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
    
    
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % OLD VERSION WITH EXTRA COLUMN FOR LP CS BR SPLIT
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% Table \ref{tab:avg_wage_reg} reports our results for average wage in the legal sector. Columns (1), and (2), fail to show significance and column (3) shows minimal significance for the estimated effect of a bankruptcy on average wage. 
% This result is consistent with the idea that wages tend to be ``stickier" than employment levels in the short run and require a larger shock to record a meaningful change. 
% Column (4) corroborates this hypothesis, showing that large firm bankruptcy shocks ``Bankruptcies (LP)'' indeed have a statistically and economically significant effect.

% Yet, the direction of the effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
% Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.

% Similar to the results on employment level, Table \ref{tab:avg_wage_reg} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 
% \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE}{tab:avg_wage_reg}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}
% \fi
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Drafts/Intro_BR_Venue_Bill_8-30.tex <==
% \iffalse
% \textcolor{red}{
% % On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck presented the bipartisan Bankruptcy Venue Reform Act to the press.
% On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% }

% \textcolor{red}{
% TO BE CONTINUED: 
% - we complement this view (Focusing on stakeholder) by assessing the general equilibrium implications of forum shopping
% - attache literature that says that health of major employees is important
% - ISSUE: why time period. Maybe we get around by doing the analysis only for Lopucki bankruptcy for the entire time period and then focus on the court competition era for justify the claim
% }
% \fi





Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
The adverse effects of bankruptcy shocks on overall local employment, however, hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).
We contribute to the literature by focusing on a sector that directly relates to bankruptcy shocks via a demand channel: the legal services. 
%studying the effect on the labor market of a particular sector, which relates to bankruptcy shocks via a demand channel: the legal services. 
% This paper is the first to document  
% the labor market response of a sector which is directly related to bankruptcy shocks via a demand channel: the \textit{legal} labor market.
%This paper contributes to the literature by identifying 
%is the first to study both theoretically and empirically 
%, which at odds with the rest of the local economy, benefits from the higher demand of legal services produced by the bankruptcy shocks.
%This paper is the first to document the effect on the legal industry labor markets, a sector related to bankruptcy shocks via a demand channel. 

% At odds with the contractionary effect observed in the local economy,
% %In opposition to the usual local contractionary impacts, 
% the labor market for the legal industry benefits from the increased demand for legal services, and subsequently acts as a potential channel for growth in the bankrupt firm’s surrounding area.
% We estimate that during the early 90's the Chapter 11 bankruptcy of a publicly traded firm is associated with a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. 
% Yet, this channel is muted when firms are allowed to file away from their headquarters. Focusing on a time period where the phenomenon of foru

\iffalse
%%%% 1
the legal industry covers professions in the areas of law, courts, law enforcement, and corrections and rehabilitation. However, this industry also includes a wide range of legal-related occupations that are found in other fi elds and industries. Many of these professions offer different litigation services to attorneys, such as trial con- sulting, expert witness services, or private investigation.
%%% 2 
Among the legal support positions that law offi ces seek to fi ll are qualifi ed paralegals, legal secretaries, receptionists, and legal technology support staff.
%%% 3 JUDICIAL ASSISTANT
Judicial Assistants help judges in local, state, federal, and tribal courts oversee judicial activities so that courts work effectively and efficiently every day. Their job is to provide judges with administrative, secretarial, and clerical support.
%%% 4 
paralegals, lawyers, clerks of courts, or court administrators
Judicial Law Clerk 16
Staff Attorney, Court 18
Bankruptcy Judge 62
% LEGAL SUPPORT PROFESSIONALS
(Legal Support Professional 82 Legal Receptionist 85 Legal Word Processor 87 Information Technology (IT) Professional 89 Legal Secretary 92 Paralegal 94 Legal Administrator 96 Human Resources Manager (Law Firm) 98 Marketing Manager (Law Firm) 100 Legal Technology Consultant 102 Legal Search Consultant 104
LITIGATION)
% COURT SUPPORT STAFF
Bailiff (Local and State Courts) 138 Court Administrator 140 Court Analyst 142 Court Clerk 144 Court Interpreter 146 Court Reporter 149 Judicial Assistant 152 Scopist 154
% PARALEGAL
Paralegals, or legal assistants, have been trained in substan- tive and procedural law and are qualified to perform various legal tasks. They may be involved in transactional matters, such as drafting contracts or reviewing trust instruments, or they may work on civil litigation or criminal defense cases. However, paralegals, unlike attorneys, cannot practice law. Paralegals cannot offer legal advice. They cannot accept clients or represent clients in courts, and paralegals cannot establish

\fi

The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
%%%%%%%%%%%%%%%
In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} 
    % $^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
%%%%%%%%%%%%%%%    
At odds with the rest of the local economy, local legal labor markets benefit from the increased demand for legal services, partially offsetting the contractionary effect on the bankrupt firm’s surrounding area.
%. Hence, they balance the contractionary effect of bankruptcy shocks on the distressed firm’s surrounding area.

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we
%We 
estimate that during the early 90's 
%the Chapter 11 bankruptcy of a publicly traded firm is
bankruptcy reorganizations are associated with 
a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars.  
%Despite this we estimate that 
Across the U.S. bankruptcies contribute an average of roughly 10,000 jobs, with wages adding up to nearly \$1 billion in 2021 dollars, each year.\footnote{
    In nominal terms we estimate this to be an average of \$523 million worth of employment each year from 1991 to 1996 inclusive.}

Our results also show that these gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We document that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).
% We document that more than 23\% of the potential employment gains are \textit{exported away} each year, on average. 
% Despite this, we estimate that bankruptcies contribute an average of \$523 million (not adjusted for inflation) worth of employment each year to local communities, or roughly 10,000 jobs. 

We measure the demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. Chapter 11 bankruptcy cases for large firms are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
    The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Lawyers and judges: those are the two occupations—and career options—that people usually think of when it comes to law or the legal industry. Indeed, lawyers and judges are the major players, but they would not be able to perform their jobs without legal, offi ce, and administrative assistance from paralegals, legal clerks, secretaries, document proces- sors, administrators, technology specialists, and other pro- fessionals. All those support professionals in the law offi ce and courtroom are part of the legal industry.
% BOOK CAREER OPPORTUNITIES IN LAW AND THE LEGAL INDUSTRY
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textcolor{purple}{We contribute to the literature, by building a unique database that expands the universe of large bankruptcies in \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.}\footnote{
%         Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).}
This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
} to a critical industry.
%vastly understudied industry that is critical to the overall economy. 
% Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
%     \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
% In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
%     Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%     \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
% } 
%Bankruptcy shocks provide a unique source of variation to disentangle internal dynamics of this industry.

    %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
    Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
    Unlike much of the applied economics literature that exploits an event study framework our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
    Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
    We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.
    We adopt an economic history approach and  focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
        For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}

    
    %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
    The historical period we focus 
    on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
    Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.
    %This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
    %%%%%%%%%%%
    During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
        \cite{ellias_bankruptcy_2019} finds that in recent years more than \%60 of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
        }
    %%%%%%%%%

% \iffalse
% %%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
% % @Ale -- I the first sentence of the Court competition era paragraph to the previous paragraph so it leads into the next paragraph better and the second paragraph is more focused on one thing. 
% %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
% Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
% Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
% Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
% We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.

% We adopt an economic history approach and 
% %Similar to the economic history approach, we 
% focus our analysis
% %To handle the complex nature of our treatment, we distinguish from previous work (cite XXX XXX XXX) and propose a novel identification strategy.differentiate from previous work treatment from Chapter 11 bankruptcies, we propose an approach that differentiates us from the previous literature. 
% %a different approach.  
% %Due to the complex nature of treatment from Chapter 11 bankruptcies, our identification strategy uses an approach similar to much of the economic history literature that focuses 
% on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
%     For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
% %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
% In particular, we focus 
% on the `Court Competition Era', a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
% Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law in order to file for Chapter 11 bankruptcy reorganization far away from their headquarters.
% This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping' (see Section \ref{sec:ForumShopping} for more details).
% \fi

%%%%%%%%%
Our identification strategy focuses on this abrupt change in bankruptcy filings practices\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
to create variations in the location of demand for legal service from Chapter 11 bankruptcies.
\textcolor{red}{Although it is well established that the strategic bankruptcy plan is drafted by a handful of highly specialized law companies (mostly located in New York), the material handling of Chapter 11 bankruptcy requires hiring a lot of unskilled, etc.\\
WE ESTIMATE THAT 20\% of the jobs LOST TO DELAWARE AND NEW YORK. 
}
\\
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus when a firm forum shops the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
% The legal services for bankruptcy proceedings will typically be located near the filing court because they must be certified to practice in that area, be familiar with local bankruptcy practices, and be able to attend proceedings and file paperwork at the courthouse.
% Thus when a firm forum shop the legal sector demand shock is effectively exported away from their local economy. This transfer in potential legal service demand is particularly pronounced because forum shopping firms often file a great distance away from their local area. 
% For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
%     Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the filing court which are exogenous to the local economy where the firm is headquartered.

A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.    

% One of our empirical strategy's identifying assumptions is that
% % Our identification strategy relies on 
% Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
% The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
% To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
% Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.

% \textcolor{red}{Equal pretrends/placebo stuff/matching}

%%%%%%%%%%% THEORETICAL ECONOMETRIC APPROACH %%%%%%%%%%% 
% \textcolor{red}{FUZZY DID \citet{de_chaisemartin_two-way_2020} also cite the package stuff}
    

% \marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
% During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% % where they \textbf{believed judges of that court would be more favorable to debtors}. 
% This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
% During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).
    
    
    

%, in hopes that the judges of that court will be more favorable to debtors.
% In particular we focus our analysis 
% on the `Court Competition Era', a period from 1991 to 1997 where stipulations of US corporate bankruptcy law created exogenous variations in the location of the court where the bankruptcy was filed (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
%In this period, firms started exploit US corporate bankruptcy law's flexible criteria for where a debtor must file.
%This variation arises because large firms are able 
%During the 1991-1997 period, 
%In this period, bankruptcy judges starting competing against each other in order to attract Ch 11 filings.

\iffalse
%%%%%%%%%%% WHY REORG NOT LIQ %%%%%%%%%%% 
We focus on Chapter 11 `reorganization' bankruptcies for three main reasons. First, it allows us to exploit forum shopping which creates variation in filing location allowing for clearer identification. Second, the legal proceedings for Chapter 11 bankruptcies are considerably more complex and require much larger legal teams than Chapter 7 bankruptcies, thus creating a larger demand shock on legal services.\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
}
Third, the vast majority of publicly traded corporations choose Chapter 11 when they file in hopes of achieving a better outcome for shareholders than they likely would with Chapter 7 cases.\footnote{
    In the \LP\; between 1980 and 2014 only one instance of a Chapter 7 bankruptcy compared to 962 Chapter 11 bankruptcies during that time.} 


\textcolor{purple}{
In doing so we make several incidental contributions to the literature. 
\marginpar{\scriptsize\textcolor{red}{CHOOSE BETWEEN THIS OR THE PURPLE SECTIONS THAT SAY THE SAME THING IN OTHER PLACES. \\~\ maybe move this paragraph to end of the intro?}}
First, we create a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
% Second, we contribute to a considerable body of literature from legal professionals and academics pertaining to forum shopping (e.g. \cite{Baird87}; \cite{EisenbergLopucki1999}; \cite{warren_bankruptcy_1987};
% \cite{Baird97}; \cite{Algero99}; \cite{Lopucki06}; \cite{LopuckiKalin00}; \cite{ThomasRasmussen01}; \cite{Cole03}; \cite{Zywicki06}; \cite{skeel_1998})
% which analyzes the implications of forum shopping on bankruptcy outcomes for the firm and it's creditors, and debates the ethics of forum shopping within the scope of the bankruptcy per se. Our focus differs from this literature. Rather than focusing on the bankruptcy outcomes for the creditors and debtors involved, we explore the general equilibrium implications of bankruptcies and forum shopping for the firm's local area. Instead of taking a side of the debate on the ethics of forum shopping we add meaningful and overlooked context to their debate.
}
Furthermore, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy.


This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping'.
When a firm forum shops they are filing in a bankruptcy court different from the local court that typically services the area where the firm's headquarters are located.\footnote{
    In our context we only consider district level forum shopping. It is worth noting that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.} 

\marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% where they \textbf{believed judges of that court would be more favorable to debtors}. 
This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).


\fi
    
    
%%%%%%%%%%% MAIN FINDINGS %%%%%%%%%%% 
To address our question, we construct a novel database 
%that contributes to literature relating to both forum shopping and Chapter 11 bankruptcies in general. Our database
that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, yearly fixed effects for each of the 94 U.S judicial districts and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
Thus we show it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million worth of employment.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 


%%%%%%%%%%% PUZZLE ON WAGES %%%%%%%%%%% 
Counter-intuitively, we find evidence that Chapter 11 bankruptcy reorganizations of large publicly traded firms are associated with a decrease in the county level average wage for the legal sector.
% Counter-intuitively, we find that Chapter 11 bankruptcy reorganizations of publicly traded firms are associated with a 1.5\% drop in the average county wage in the legal sector.
We reconcile this puzzling finding with a \textit{compositional} effect. 
To do this we specialize the canonical model from \citet{Acemoglu_Autor_2011} to the legal labor markets. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and unskilled labor (paralegals, law clerks, etc.).
Skilled workers are more productive but their labor supply is more inelastic than unskilled workers.
In this environment, bankruptcy shocks boost the demand of legal services, prompting an increase in the firm's demand for both types of workers.
Since skilled workers have a relatively inelastic labor supply, bankruptcy shocks shift the composition of legal workers towards unskilled workers, causing a drop in the average wage.


%%%%%%%%%%% MODEL %%%%%%%%%%% 
% Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
% In doing so we contribute to the extensive body of the empirical literature (e.g. \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}) that aims to estimate the elasticity of substitution between high and low skilled labor for CES production functions. 
% We differ from this existing literature by being the first to provide empirical evidence for the elasticity of substitution across skill levels in the context of the legal industry. With this novel setting we not only find evidence that supports previous estimates that skilled and unskilled labor are imperfect substitutes, but we are also able to find point estimates for this parameter.

Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
In doing so we contribute to the extensive body of the empirical literature that aims to estimate the elasticity of substitution between high and low skilled labor (e.g. \cite{katz_changes_1992}, \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}).
Unlike much of this literature we provide empirical evidence for the elasticity of substitution across skill levels at an industry level, and are the first to do so in the context of the legal industry. 
With this novel setting we find additional evidence supporting \citet{blankenau_industry_2011} who predict this elasticity to be higher at the industry level than it is at an aggregate level.  

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to the literature. 
First, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy. Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.

==> Drafts/Intro_Draft_V3.tex <==
Legal expenses are often treated as dead-weight loss from bankruptcy proceedings 
%The bankruptcy literature often treats legal expenses as a dead-weight loss from bankruptcy proceedings 
(e.g.
\citealp{franks_comparison_1996};
\citealp{armour_costs_2012};
\citealp{m_m_buehlmaier_debt_2014};
\citealp{mahoney_bankruptcy_2015}).
However, %these 
they 
are meaningful transfers to crucial stakeholders of bankruptcy events: 
professionals employed in the legal service sector.
In this paper we illustrate how failing to account for
%Failing to account for 
these transfers overlooks a potential source of economic stimulus,
which acts in opposition to the overall contractionary effect 
that large bankruptcies have on local employment (\citealp{bernstein_bankruptcy_2019}). 
% on local employment when a large firm files for bankruptcy (\citealp{bernstein_bankruptcy_2019}). 
%%%% GOOD BUT ON HOLD
%We contribute to the literature by studying the effect of bankruptcy shocks on the local legal service sector. %, a sector that directly relates to bankruptcy shocks via a demand channel. 
%%%% END GOOD BUT ON HOLD
We provide first evidence that local legal labor markets indeed benefit from the increased demand for legal services created by bankruptcies. 
%\textcolor{red}{We then estimate the role of lax bankruptcy venue laws} and competition among courts in exporting away these potential gains from the affected communities. 
We then illustrate how lax bankruptcy venue laws and competition among courts may hinder this effect, by exporting %contribute in exporting 
away these potential gains from the affected communities. 
%We conclude by developing and estimating a structural model of the legal sector. We quantify economically meaningful welfare looses from firms who file in courts far from their local communities (i.e. forum shop).
%After estimating a structural model of the legal sector, we quantify the missed welfare gains in the legal sector from firms who file in courts far from their local communities (i.e. forum shop).
%the missed welfare gains in the legal sector from firms who file in courts far from their local communities (i.e. forum shop).
%After estimating a structural model of the legal sector, we quantify the missed welfare gains in the legal sector from firms who file in courts far from their local communities (i.e. forum shop).
Finally,  
%developing and estimating a structural model of the legal sector, we 
we develop a structural model of the legal sector and quantify economically meaningful welfare losses in the
bankrupt firm’s surrounding area from firms who file in courts far from their local communities. 
% (i.e. forum shop).

%We then show that lax bankruptcy venue laws and competition among courts may export away these potential gains from the affected communities. 
%Finally, we structurally estimate a model of the legal sector, and perform counterfactual analysis to quantify missed welfare gains in the legal sector from firms who file in courts far from their local communities (i.e. forum shop).

%have caused a substantial amount of these potential gains to be exported away from the affected communities.
%, \textcolor{red}{acting in opposition to the contractionary effect on the bankrupt firm’s surrounding area (CUT THIS ONE)}. 
% Finally, we structurally estimate a model of the legal sector, and perform counterfactual analysis to quantify missed welfare gains in the legal sector from firms who forum shop away from their local communities.


% The vast majority of the bankruptcy literature treats
% legal expenses as a dead-weight loss from bankruptcies (CITATIONS).
% But they are not. 
% They are meaningful transfers to crucial stakeholders of bankruptcy events: 
% professionals employed in the legal service sector.\footnote{
%     LOTS OF PAPERS MAYBE FOOTNOTE} 
% We contribute to the literature by studying the effect of bankruptcy shocks on the local legal service sector-
% a sector that directly relates to bankruptcy shocks via a demand channel.
% First, we find evidence that local legal labor markets benefit from the increased demand for legal services created by bankruptcies, partially offsetting the contractionary effect on the bankrupt firm’s surrounding area. 
% Second, we show that lax bankruptcy venue laws and competition among courts may have caused a substantial amount of these potential gains to be exported away from the affected community.
% Finally, we structurally estimate a model of the legal sector, and perform counterfactual analysis to quantify missed welfare gains in the legal sector from firms who forum shop away from their local communities.

% Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
% Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
% However, the adverse effects of bankruptcy shocks on overall local employment hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).



\textcolor{red}{ ***** WE MAY WANT TO ABSORB THIS PARAGRAPH IN LATER SECTIONS. IT REPEATS THE FIRST WITH NUMBERS THAT WE CAN DISCUSS LATER ***** } 
Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we estimate that during the early 90's bankruptcy reorganizations are associated with a 1\% increase in annual legal employment for the affected county for each ongoing bankruptcy. 
% Aggregated across the U.S. this is roughly 10,000 jobs with wages adding up to nearly \$1 billion in 2021 dollars \textit{each year}. 
Aggregated across the U.S. this means that each year roughly 10,000 jobs---with wages adding up to nearly \$1 billion in 2021 dollars---are being distributed to communities dealing with the contractionary effects associated with a major employer filing for bankruptcy.\footnote{
To put this number in context, place-based job policies estimate that the cost per job ranges between \$18,000 and \$63,000. Accordingly, the cost to create 10,000 jobs is around \$180 million dollars (see Criscuolo et al (2018, AER).) \textcolor{red}{1. PUT CITATION IN BIB. 2. Not entirely clear to me.}
}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LA ON HOLD
% For a large city such as Los Angeles this is more than 4,000 jobs each year-- an even larger source of employment than the Amazon HQ2 that cities offered hundreds of millions in incentives to attract.\footnote{
%     As of September 1, 2021 there were roughly 3000 employees assigned to HQ2. \textit{Source:} \href{https://www.aboutamazon.com/news/amazon-offices/the-next-chapter-for-hq2-sustainable-buildings-surrounded-by-nature}{Amazon}. 
%     Notably Montgomery County, Md. offered \$8.5 billion in incentives to attract Amazon's new HQ2. \textit{Source:} \href{https://www.brookings.edu/research/five-economic-development-takeaways-from-the-amazon-hq2-bids/}{Brookings.edu}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
% However, it's possible that lax bankruptcy venue statutes and competition among judges to attract firms to file in their court, instead of the court in their local area, may have caused a considerable amount of these potential gains to be squandered. 
Importantly, we 
%Our results also 
show that these gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We find evidence that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).
We complement this analysis by estimating a parsimonious model of the legal labor market and \textcolor{red}{document XXXX}
\textcolor{red}{ *** MISS STRUCTURAL MODEL *** }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ORIGINAL- CH11 br are big %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We measure the demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. Chapter 11 bankruptcy cases for large firms are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
% Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
%     The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
%     For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
%     } 
% for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
%     For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
% This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
% } to a critical industry.
%% 
            % \marginpar{\scriptsize\textcolor{red}{ARGUE IN TWO STEPS- CHAPTER 11 are: \\1. large bankruptcies (ORGANIZE POINTS BEFORE);  \\2. provide a feature that we leverage for identification: forum shoppping. (THE LATTER WILL CONNECT WELL WITH THE NEXT PARAGRAPH)}}   
            

\textcolor{red}{For identification purposes,} we measure demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. % for two main reasons. 
First, Chapter 11 bankruptcies act as a considerable demand shock to legal services.
These bankruptcy cases are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Consequently, firms will often pay fees in the order of hundreds of millions of dollars\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.  
    Professional fees averaged \$82 million in 2021 dollars in the \LPlong\, over the period 1980-2014.
    %The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
\textcolor{red}{This second feature is key for our identification. EXPLAIN NEW YORK SPECIALIZED vs PARALEGAL IN LOCUS.}    
    
The second reason is that stipulations of the Chapter 11 U.S. bankruptcy statutes provide a feature that we leverage for identification: forum shopping.
Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is not straightforward.
Unlike the applied economics literature that exploits an event study framework, our research design setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2021}, \cite{sun_estimating_2020}). 
Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
We contribute to the previous literature (e.g. \citealp{bernstein_bankruptcy_2019}; \citealp{chava2021community}) by proposing an alternative identification strategy that handles the complex nature of our treatment.
We adopt an economic history approach and focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
    For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
        
        
The historical period we focus 
on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges began competing for prestigious and lucrative Chapter 11 filings (e.g. \citealp{lopucki_courting_2005}, \citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.
    } 
%This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
%%%%%%%%%%%
During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
    \cite{ellias_bankruptcy_2019} finds that in recent years more than 60\% of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
    }
    
    
Our identification strategy focuses on this period of abrupt change in bankruptcy filing practices to create exogenous variations in the location of demand for legal service from Chapter 11 bankruptcies.
% \textcolor{red}{Although it is well established that the strategic bankruptcy plan is drafted by a handful of highly specialized law companies (mostly located in New York), the material handling of Chapter 11 bankruptcy requires hiring a lot of unskilled, etc.\\
% WE ESTIMATE THAT 20\% of the jobs LOST TO DELAWARE AND NEW YORK. 
% }
% \\
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus, when a firm forum shops, the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. 
% By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    % Figures calculated using the \LPlong.}
This is a drastic increase from 18.9 miles for firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}
The exogeneity of this variation in filing location during the court competition era is supported by findings in the legal literature (e.g. \citealp{EisenbergLopucki1999}, \citealp{lopucki_courting_2005}, \citealp{Lopucki06}). 
Section \ref{sec:FS_LocalConditions} describes this in detail and provides empirical evidence. 
    
    
A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are a source of plausibly exogenous variation in the local demand for legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. We also demonstrate this exogeneity empirically in Section \ref{sec:BR_LocalConditions}.
% In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.  
% In addition, Section \ref{sec:BR_LocalConditions} demonstrates this exogeneity empirically. 


%\textcolor{red}{***Also note that for our purposes, it is unimportant \textit{why} firms forum shop; rather, our identification simply requires the forum shopping reason to be independent from the local economy.***}

% To address our question, 
For our analysis,
we construct a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, U.S judicial district-year fixed effects, and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
This indicates that it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million of wages.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. 
We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 




% Motivated by the evidence from the reduced form results we construct a parsimonious model, similar to \citet{notowidigdo_incidence_2020}, that captures the dynamics of how legal sector labor markets respond to a demand shock. 
Motivated by the evidence from the reduced form results we build on \citet{notowidigdo_incidence_2020} and construct a parsimonious model to capture the effect of demand shocks on legal labor markets.\footnote{Our model is a specialization of the canonical labor model used for studying how shocks effect labor market outcomes across skill levels (\cite{acemoglu_technical_2002}, \cite{Acemoglu_Autor_2011}, \cite{bowlus_wages_2017}).}
%the dynamics of how legal sector labor markets respond to a demand shock. 
%We model the local labor demand as in the spatial equilibrium model of \citet{notowidigdo_incidence_2020}. 
%The model builds on \citet{notowidigdo_incidence_2020}. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and less productive unskilled labor (paralegals, law clerks, etc.).
Following the work of %works such as \citet{notowidigdo_incidence_2020} and 
\citet{bai_demand_2012}, demand shocks enter this model akin to ``productivity'' shocks. 


We calibrate the model parameters using a nonlinear simultaneous-equations generalized method of moments (GMM) procedure that exploits non-forum shopped bankruptcies as exogenous demand shocks for the local area.
In doing so we contribute to the extensive body of literature that estimates the Frisch elasticity of labor supply for the extensive margin (e.g. \cite{bianchi_icelands_2001}; \cite{brown_link_2013}; \cite{rogerson_micro_2009}).
Unlike much of this literature we provide empirical evidence for the elasticity of labor supply at the industry level and are the first to do so in the context of the legal industry.
Of particular interest, we find evidence that this elasticity of labor supply is greater for unskilled labor than for skilled labor.  


 

Our calibrated model allows us to to quantitatively estimate the welfare implications of forum shopping. 
% To do so we calculate the consumption equivalent variation between the observed state of the world with forum shopping, and the counterfactual regime where all bankruptcies were filed locally. 
To do so we calculate the potential welfare gains associated with moving from the status-quo regime where firms forum shop to a counterfactual regime without forum shopping.
We find that workers would need roughly a 1\% increase in there annual consumption to receive the same level of utility they would have without forum shopping. 

While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will strengthen Chapter 11 bankruptcy venue laws and prevent firms from filing far from where they are located, likely putting a halt to the practice of forum shopping. 
If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business.
The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community\footnote{
    See press release  \textit{Lofgren, Buck Introduce Bipartisan Legislation to End Corporate Bankruptcy Forum Shopping}, from Rep. Lofgren. 
    \textit{Source:} \href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}
    }
    % (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
    City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}.}
Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate.

% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate. 

% \textcolor{red}{While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
% On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate. }



%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to other literature on the topic. 
First, we contribute to the heated debate in the law literature over the efficiency of forum shopping and court competition for bankruptcy outcomes (e.g. \citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06}, \citealp{lee_delawares_2011})--by providing first evidence of the unintended consequences on the local economy. 
\textcolor{red}{We also contribute to works such as \citet{gennaioli_judicial_2010} which looks to understand the efficiency and incentives involved with forum shopping by creating an economic model for the supply and demand of bankruptcy courts. 
We add critical context to their work by documenting evidence for general equilibrium impacts of forum shopping in corporate bankruptcies. }

% Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.



\textcolor{red}{The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}}} 



==> Drafts/Intro_v4.tex <==
Legal expenses are often treated as dead-weight loss from bankruptcy proceedings (e.g.
\citealp{franks_comparison_1996};
\citealp{armour_costs_2012};
\citealp{m_m_buehlmaier_debt_2014};
\citealp{mahoney_bankruptcy_2015}).
However, they are meaningful transfers to crucial stakeholders of bankruptcy events: 
professionals employed in the legal service sector.
In this paper, we illustrate how failing to account for these transfers overlooks a potential source of economic stimulus, which acts in opposition to the overall contractionary effect 
that large bankruptcies have on local employment (\citealp{bernstein_bankruptcy_2019}). 
We provide first evidence that local legal labor markets indeed benefit from the increased demand for legal services created by bankruptcies. 
We then illustrate how lax bankruptcy venue laws and competition among courts may nullify this effect, by exporting away these potential gains from the affected communities. 
Finally, we develop a structural model of the legal sector and quantify economically meaningful welfare losses in the
bankrupt firm’s surrounding area from firms who file in courts far from their local communities. 

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we estimate that during the early 90's bankruptcy reorganizations are associated with a 1\% increase in annual legal employment for the affected county for each ongoing bankruptcy. 
Aggregated across the U.S. this means that each year roughly 10,000 jobs---with wages adding up to nearly \$1 billion in 2021 dollars---are being distributed to communities dealing with the contractionary effects associated with a major employer filing for bankruptcy.\footnote{
To put this number in context, place-based job policies estimate that the cost per job ranges between \$18,000 and \$63,000. Accordingly, the cost to create 10,000 jobs is around \$180 million dollars (see Criscuolo et al (2018, AER).) \textcolor{red}{1. PUT CITATION IN BIB. 2. Not entirely clear to me.}
}
Crucially, %we show that 
these employment gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We find evidence that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).
Building on the work of \citet{notowidigdo_incidence_2020}, we structurally estimate a labor model of the legal sector and estimate a consumption equivalent variation loss of $\approx$1\% in affected communities as as a result of forum shopping.%estimate a labor model with skilled and unskilled workers to the legal sector(\citealp{acemoglu_technical_2002}, \citealp{Acemoglu_Autor_2011}, \citealp{bowlus_wages_2017}), and 
 
We measure demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms for two main reasons. 
First, Chapter 11 bankruptcies act as a considerable demand shock to legal services.
These bankruptcy cases are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Consequently, firms will often pay fees in the order of hundreds of millions of dollars\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.  
    Professional fees averaged \$82 million in 2021 dollars in the \LPlong\, over the period 1980-2014.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
%\textcolor{red}{This second feature is key for our identification. EXPLAIN NEW YORK SPECIALIZED vs PARALEGAL IN LOCUS.}    
The second reason is that stipulations of the Chapter 11 U.S. bankruptcy statutes provide a feature that we leverage for identification: forum shopping.

Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is not straightforward.
Unlike the applied economics literature that exploits an event study framework, our research design setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2021}, \cite{sun_estimating_2020}). 
Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
We contribute to the previous literature (e.g. \citealp{bernstein_bankruptcy_2019}; \citealp{chava2021community}) by proposing an alternative identification strategy that handles the complex nature of our treatment.
We adopt an economic history approach and focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
    For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
        
        
The historical period we focus 
on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges began competing for prestigious and lucrative Chapter 11 filings (e.g. \citealp{lopucki_courting_2005}, \citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.
    } 
%This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
%%%%%%%%%%%
During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
    \cite{ellias_bankruptcy_2019} finds that in recent years more than 60\% of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
    }
    
    
Our identification strategy focuses on this period of abrupt change in bankruptcy filing practices to create exogenous variations in the location of demand for legal service from Chapter 11 bankruptcies.
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus, when a firm forum shops, the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. 
This is a drastic increase from 18.9 miles for firms who did not forum shop.\footnote{
    Figures are calculated using the \LPlong.}
The exogeneity of this variation in filing location during the court competition era is supported by findings in the legal literature (e.g. \citealp{EisenbergLopucki1999}, \citealp{lopucki_courting_2005}, \citealp{Lopucki06}). 
Section \ref{sec:FS_LocalConditions} describes this in detail and provides empirical evidence. 
    
    
A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are a source of plausibly exogenous variation in the local demand for legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. We also demonstrate this exogeneity empirically in Section \ref{sec:BR_LocalConditions}.

For our analysis,
we construct a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
we estimate a regression with county level fixed effects, U.S judicial district-year fixed effects, and county-year controls. 

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
This indicates that it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million of wages.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. 
We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 



In Section \ref{sec:struct_est} we build on 
%Motivated by the evidence from the reduced form results we build on 
\citet{notowidigdo_incidence_2020} and construct a parsimonious model to capture the effect of demand shocks on legal labor markets.\footnote{Our model is a specialization of the canonical labor model used for studying how shocks effect labor market outcomes across skill levels (\cite{acemoglu_technical_2002}, \cite{Acemoglu_Autor_2011}, \cite{bowlus_wages_2017}).}
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and less productive unskilled labor (paralegals, law clerks, etc.).
In the spirit of \citet{bai_demand_2012}, demand shocks enter this model akin to ``productivity'' shocks. 


We calibrate the model parameters using a nonlinear simultaneous-equations generalized method of moments (GMM) procedure that exploits non-forum shopped bankruptcies as exogenous demand shocks for the local area.
Using this novel identification approach, we provide first empirical estimates for the elasticity of labor supply of skilled and unskilled workers in the legal industry.
%Using this novel identification approach, we estimate the elasticity of labor supply of skilled and unskilled workers in the legal industry. 
%that unskilled workers have a higher elasticity of labor supply than skilled labor. 
This finding adds to the body of literature that estimates the Frisch elasticity of labor supply for the extensive margin (e.g. \cite{bianchi_icelands_2001}; \cite{brown_link_2013}; \cite{rogerson_micro_2009}). 
%Unlike much of this literature we provide empirical evidence for the elasticity of labor supply at the industry level and are the first to do so in the context of the legal industry.
% In doing so, we provide insights into the labor markets of an industry that plays a key role in the functioning of the judiciary system of modern economic societies, but has been comparatively understudied with respect to similarly-sized sectors, such as agriculture.\footnote{In 2019 the industry GDP measured 280 billion, while the US agricultural sector measured 175 billion.
In doing so, we provide insights into the labor markets of an industry that plays a key role in the functioning of modern economic societies (\citealp{bennett_corporate_2018}), but has been comparatively understudied with respect to similarly-sized sectors, such as agriculture.\footnote{
    In 2019 the legal industry GDP measured 280 billion, while the US agricultural sector measured 175 billion.
     \textit{Source:} Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
  \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}}
  %\footnote{Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}}

%%%%%%%%%%%%%%%%%%%%%%%%% OLD
% Incidentally, we contribute to the extensive body of literature that estimates the Frisch elasticity of labor supply for the extensive margin (e.g. \cite{bianchi_icelands_2001}; \cite{brown_link_2013}; \cite{rogerson_micro_2009}).
% Unlike much of this literature we provide empirical evidence for the elasticity of labor supply at the industry level and are the first to do so in the context of the legal industry.
% Of particular interest, we find evidence that this elasticity of labor supply is greater for unskilled than for skilled labor.  
% \textcolor{red}{Although key to the functioning of the judiciary system of modern economic societies, the legal industry is comparatively understudied with respect to similarly-sized key sectors, like agriculture.\footnote{In 2019 the industry GDP measured 280 billion, while the US agricultural sector measured 175 billion.
%     \textit{Source:} Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%  \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}}
% }

Our calibrated model allows us to to quantitatively estimate the welfare implications of forum shopping. 
To do so we calculate the potential welfare gains associated with moving from the status-quo regime where firms forum shop to a counterfactual regime without forum shopping.
We find that workers would need roughly a 1\% increase in there annual consumption to receive the same level of utility they would have without forum shopping. 

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
%By considering the channel of forum shopping we
These results incidentally contribute to the heated debate in the law literature over the efficiency of forum shopping and court competition for bankruptcy outcomes (e.g. \citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06}, \citealp{lee_delawares_2011}), by providing first evidence of unintended consequences on the local economy. 
Accordingly, our findings have direct economic relevance on the ongoing policy debate in the U.S. Congress about the Bankruptcy Venue Reform Act.
%While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business.
The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community\footnote{
    See press release  \textit{Lofgren, Buck Introduce Bipartisan Legislation to End Corporate Bankruptcy Forum Shopping}, from Rep. Lofgren. 
    \textit{Source:} \href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}
    }
and put to an end ``the single most significant source of injustice in Chapter 11 bankruptcy cases''.\footnote{
    City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}.}
Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate.

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
% By considering the channel of forum shopping 
% %we also make several incidental contributions to other literature on the topic. First, we 
% we incidentally
% contribute to the heated debate in the law literature over the efficiency of forum shopping and court competition for bankruptcy outcomes (e.g. \citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06}, \citealp{lee_delawares_2011}), by providing first evidence of the unintended consequences on the local economy. 
% Second, the legal industry plays a key role in the functioning of the judiciary system of modern economic societies. 
% Our work
% %\textcolor{red}{
% %We also contribute to works such as \citet{gennaioli_judicial_2010} which looks to understand the efficiency and incentives involved with forum shopping by creating an economic model for the supply and demand of bankruptcy courts. 
% %We add critical context to their work by documenting evidence for general equilibrium impacts of forum shopping in corporate bankruptcies. }


% %%%%%%%%%%%%%%%%%%%%%%%
% \textcolor{red}{The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
% In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
%     Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%     \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
% }
% Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
%     2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}}} 



==> Drafts/Intro_v4_ParkingLot.tex <==
Legal expenses are often treated as dead-weight loss from bankruptcy proceedings (e.g.
\citealp{franks_comparison_1996};
\citealp{armour_costs_2012};
\citealp{m_m_buehlmaier_debt_2014};
\citealp{mahoney_bankruptcy_2015}).
However, they are meaningful transfers to crucial stakeholders of bankruptcy events: 
professionals employed in the legal service sector.
In this paper we illustrate how failing to account for these transfers overlooks a potential source of economic stimulus, which acts in opposition to the overall contractionary effect 
that large bankruptcies have on local employment (\citealp{bernstein_bankruptcy_2019}). 
We provide first evidence that local legal labor markets indeed benefit from the increased demand for legal services created by bankruptcies. 
We then illustrate how lax bankruptcy venue laws and competition among courts may hinder this effect, by exporting away these potential gains from the affected communities. 
Finally, we develop a structural model of the legal sector and quantify economically meaningful welfare losses in the
bankrupt firm’s surrounding area from firms who file in courts far from their local communities. 

\textcolor{red}{ ***** WE MAY WANT TO ABSORB THIS PARAGRAPH IN LATER SECTIONS. IT REPEATS THE FIRST WITH NUMBERS THAT WE CAN DISCUSS LATER ***** } 
Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we estimate that during the early 90's bankruptcy reorganizations are associated with a 1\% increase in annual legal employment for the affected county for each ongoing bankruptcy. 
Aggregated across the U.S. this means that each year roughly 10,000 jobs---with wages adding up to nearly \$1 billion in 2021 dollars---are being distributed to communities dealing with the contractionary effects associated with a major employer filing for bankruptcy.\footnote{
To put this number in context, place-based job policies estimate that the cost per job ranges between \$18,000 and \$63,000. Accordingly, the cost to create 10,000 jobs is around \$180 million dollars (see Criscuolo et al (2018, AER).) \textcolor{red}{1. PUT CITATION IN BIB. 2. Not entirely clear to me.}
}

Importantly, we show that these gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We find evidence that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).
We complement this analysis by estimating a parsimonious model of the legal labor market and \textcolor{red}{document XXXX}
\textcolor{red}{ *** MISS STRUCTURAL MODEL *** }

\textcolor{red}{For identification purposes,} we measure demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. % for two main reasons. 
First, Chapter 11 bankruptcies act as a considerable demand shock to legal services.
These bankruptcy cases are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Consequently, firms will often pay fees in the order of hundreds of millions of dollars\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.  
    Professional fees averaged \$82 million in 2021 dollars in the \LPlong\, over the period 1980-2014.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
\textcolor{red}{This second feature is key for our identification. EXPLAIN NEW YORK SPECIALIZED vs PARALEGAL IN LOCUS.}    
    
The second reason is that stipulations of the Chapter 11 U.S. bankruptcy statutes provide a feature that we leverage for identification: forum shopping.
Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is not straightforward.
Unlike the applied economics literature that exploits an event study framework, our research design setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2021}, \cite{sun_estimating_2020}). 
Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
We contribute to the previous literature (e.g. \citealp{bernstein_bankruptcy_2019}; \citealp{chava2021community}) by proposing an alternative identification strategy that handles the complex nature of our treatment.
We adopt an economic history approach and focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
    For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
        
        
The historical period we focus 
on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges began competing for prestigious and lucrative Chapter 11 filings (e.g. \citealp{lopucki_courting_2005}, \citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.
    } 
%This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
%%%%%%%%%%%
During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
    \cite{ellias_bankruptcy_2019} finds that in recent years more than 60\% of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
    }
    
    
Our identification strategy focuses on this period of abrupt change in bankruptcy filing practices to create exogenous variations in the location of demand for legal service from Chapter 11 bankruptcies.
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus, when a firm forum shops, the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. 
This is a drastic increase from 18.9 miles for firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}
The exogeneity of this variation in filing location during the court competition era is supported by findings in the legal literature (e.g. \citealp{EisenbergLopucki1999}, \citealp{lopucki_courting_2005}, \citealp{Lopucki06}). 
Section \ref{sec:FS_LocalConditions} describes this in detail and provides empirical evidence. 
    
    
A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are a source of plausibly exogenous variation in the local demand for legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. We also demonstrate this exogeneity empirically in Section \ref{sec:BR_LocalConditions}.

For our analysis,
we construct a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
we estimate a regression with county level fixed effects, U.S judicial district-year fixed effects, and county-year controls. 

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
This indicates that it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million of wages.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. 
We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 




Motivated by the evidence from the reduced form results we build on \citet{notowidigdo_incidence_2020} and construct a parsimonious model to capture the effect of demand shocks on legal labor markets.\footnote{Our model is a specialization of the canonical labor model used for studying how shocks effect labor market outcomes across skill levels (\cite{acemoglu_technical_2002}, \cite{Acemoglu_Autor_2011}, \cite{bowlus_wages_2017}).}
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and less productive unskilled labor (paralegals, law clerks, etc.).
Following the work of \citet{bai_demand_2012}, demand shocks enter this model akin to ``productivity'' shocks. 


We calibrate the model parameters using a nonlinear simultaneous-equations generalized method of moments (GMM) procedure that exploits non-forum shopped bankruptcies as exogenous demand shocks for the local area.
In doing so we contribute to the extensive body of literature that estimates the Frisch elasticity of labor supply for the extensive margin (e.g. \cite{bianchi_icelands_2001}; \cite{brown_link_2013}; \cite{rogerson_micro_2009}).
Unlike much of this literature we provide empirical evidence for the elasticity of labor supply at the industry level and are the first to do so in the context of the legal industry.
Of particular interest, we find evidence that this elasticity of labor supply is greater for unskilled labor than for skilled labor.  


 

Our calibrated model allows us to to quantitatively estimate the welfare implications of forum shopping. 
To do so we calculate the potential welfare gains associated with moving from the status-quo regime where firms forum shop to a counterfactual regime without forum shopping.
We find that workers would need roughly a 1\% increase in there annual consumption to receive the same level of utility they would have without forum shopping. 

While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business.
The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community\footnote{
    See press release  \textit{Lofgren, Buck Introduce Bipartisan Legislation to End Corporate Bankruptcy Forum Shopping}, from Rep. Lofgren. 
    \textit{Source:} \href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}
    }
and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
    City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}.}
Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate.

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to other literature on the topic. 
First, we contribute to the heated debate in the law literature over the efficiency of forum shopping and court competition for bankruptcy outcomes (e.g. \citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06}, \citealp{lee_delawares_2011})--by providing first evidence of the unintended consequences on the local economy. 
\textcolor{red}{We also contribute to works such as \citet{gennaioli_judicial_2010} which looks to understand the efficiency and incentives involved with forum shopping by creating an economic model for the supply and demand of bankruptcy courts. 
We add critical context to their work by documenting evidence for general equilibrium impacts of forum shopping in corporate bankruptcies. }

\textcolor{red}{The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}}} 



==> Drafts/Model_StrucEst_Proofs_Mechanism_PRE_GMM.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Model of the Legal Labor Market}\label{sec:TheModel}



This section specializes a model with skilled and unskilled workers (e.g. \cite{acemoglu_technical_2002}; \cite{Acemoglu_Autor_2011}; \cite{bowlus_wages_2017}) to study the effect of bankruptcy shocks on legal labor markets and reconcile the puzzling effect on wages.
The interested reader can refer to Appendix \ref{App:model} for a detailed discussion of the model and all derivations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                   THEORETICAL MODEL

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Environment}
We consider a dynamic partial equilibrium model of the legal sector. 
The economy is populated by a mass of heterogeneous households and a representative firm that produces legal services. 

%% HOUSEHOLDS
Households work in the legal sector and differ in their labor productivity type ($j$): skilled  ($j=s$) and unskilled  ($j=u$). Skilled workers can be thought of as highly trained specialized legal workers such as lawyers. Whereas unskilled workers can be thought of less trained and/or specialized legal workers, such as para-legals and law clerks. 
In each period $t$, households of type $j$ choose consumption $\cjt\in\mathbb{R}_{+}$ and labor hours $\njt\in\mathbb{R}_{+}$
    in order to maximize Greenwood–Hercowitz–Huffman preferences.
\begin{equation}\label{Utility}
\begin{split}
       \underset{\{\cjt,\njt\}^{\infty}_{t=0}}{\max}\quad & \sum_{t=0}^{\infty}\beta^{t}\frac{1}{1-\sigma}\left(\cjt - \gamma \frac{n_{j,t}^{1+\rho_{j}}}{1 + \rho_{j}}\right)^{1-\sigma}\\
       &\text{s.t.}\; \cjt \leq \wjt \njt
\end{split}
\end{equation}     
where $\rho_{j}>0$ captures type $j$ (inverse) Frisch elasticity of labor supply, and the terms $\sigma > 0$ and $\gamma > 0$ are shaping parameters.   
 For each hour of work supplied workers of type $j$ receive an hourly wage $\wjt$. The wage compensation is their only source of income.
 
%% FIRMS
In each period $t$, a profit-maximizing representative firm hires skilled $(s)$ and unskilled $(u)$ workers to produce legal services $L(s,u)$ (the numeraire)  
        \begin{equation}\label{eq:CES}
            L(\s,\u) = \left[ 
            (A_{u}\u)^{\frac{\delta - 1}{\delta}} + (A_{s}\s)^{\frac{\delta - 1}{\delta}}
            \right]^{\frac{\delta}{\delta - 1}}
        \end{equation}
where $\delta \in [0,\infty)$ is the elasticity of substitution between the input factors. The demand of legal services is exogenous. 
Labor markets and the market for legal services are competitive.

\subsubsection{Equilibrium Characterization and Main Results}
% \textbf{Definition} 
\begin{definition*}
An equilibrium is an allocation of consumption and labor across skilled and unskilled households, quantity of legal services, as well as wages for skilled and unskilled workers and price of legal services such that: 
\textit{(i)} households choose consumption and labor supply to solve \eqref{Utility};
\textit{(ii)} the representative firm hires workers to maximize its profits;
 \textit{(iii)} labor and legal service output markets clear.
\end{definition*}

Households and firm's first order conditions and market clearing yield the following equilibrium characterization. 
%%% LEMMA %%%
\begin{lemma}\label{eq_lem} 
    Labor Market Equilibrium for the Legal Sector:
    \vspace{-1cm}
    \begin{multicols}{2}
    \begin{equation}\label{eq_s}
    \s^{*}(L) = [\gamma^{-\delta} A_{s}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_s}}}
    \end{equation}
    
    \begin{equation}\label{eq_u}
    \u^{*}(L) = [\gamma^{-\delta} A_{u}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_u}}}
    \end{equation}
    \end{multicols}
    \vspace{-1cm}
    \begin{multicols}{2}
    \begin{equation}\label{eq_ws}
        w^{*}_{s}(L) = \gamma\left( A_{s}^{\delta - 1} L^{\rho_s}\right)^{\frac{1}{1+\delta\rho_{s}}} 
    \end{equation}
    
    \begin{equation}\label{eq_wu}
        w^{*}_{u}(L) = \gamma\left( A_{u}^{\delta - 1} L^{\rho_u}\right)^{\frac{1}{1+\delta\rho_{u}}} 
    \end{equation}
    \end{multicols}
\end{lemma}
% \noindent Equations (\ref{eq_s}) and (\ref{eq_u}) show that in equilibrium both $\s$ and $\u$ are increasing in $L$. 
Note that $L(\s,\u)$ is the production of \textit{all} legal services for a local area. When a firm files for Chapter 11 bankruptcy the demand for legal services increases, which results in an increase in the equilibrium level of $L$ in the market for legal services. These bankruptcy shocks are used as instruments for variation in $L$, and as such appear in the model as an increase in $L$. 
Forum shopping enters the model by dampening the increase in $L$ when a bankruptcy shock occurs (see Appendix \ref{App:model_forumshopping}). 

Using Lemma \ref{eq_lem} and Lemmas \ref{lem:skpremium_avgwage} and \ref{lem:ratio_su} in Appendix \ref{App:model}, we derive the response of \textit{average} wage to bankruptcy shocks.
% derive the relationship between $L$ and \textit{average wage}.
\begin{proposition}\label{prop_main}
    Given unskilled labor is relatively more elastic ($\rho_u < \rho_s$) and skilled labor has a higher wage ($\frac{w_s}{w_u} > 1$), then an increase in $L$ will yield:
    \textit{(i)} an increase in $\s^*, \u^*, w^{*}_{s}, w^{*}_{u}$; and \textit{(ii)} a decrease in $\frac{\s^*}{\u^*}$.
    
    \noindent \textbf{Compositional Channel}: The decrease in $\frac{\s^*}{\u^*}$ yields in turn a decrease in the average wage $\overline{w} = \frac{\left[ 
                    A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\s/\u\right)^{\frac{\delta - 1}{\delta}}
                    \right]^{\frac{\delta}{\delta - 1}}}{\left(1 + \s/\u\right)}$. 

    % i) Equilibrium levels of $\s^*, \u^*, w^{*}_{s}, w^{*}_{u}$ increase.
    
    % ii) $\frac{\s^*}{\u^*}$ decreases (compositional channel) $\implies \overline{w} = \frac{\left[ 
    %                 A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\s/\u\right)^{\frac{\delta - 1}{\delta}}
    %                 \right]^{\frac{\delta}{\delta - 1}}}{\left(1 + \s/\u\right)}$ \;\; decreases. 
\end{proposition}

Proposition \ref{prop_main} represents our main theoretical result.
%is our main theoretical result as predicted empirically in section \ref{sec:wag}. 
Bankruptcy shocks increase demand for legal services, $L$, so firms employ more workers of both types to increase production. In doing so, relative factor intensity of skilled labor $\frac{\s^*}{\u^*}$ decreases because unskilled labor is relatively more elastic. This influx in unskilled labor then brings the average wage for legal sector employees down. 
Proposition \ref{prop_main} proposes a compositional channel mechanism that rationalizes our empirical findings on the effect of bankruptcy shocks on legal county average wage (Section \ref{sec:wag}). 
\textcolor{red}{While we cannot exclude alternative explanations, we find our mechanism to be consistent with the empirical evidence that 
changes in wages within skill groups are small relative to the ones across skill groups (\citealp{notowidigdo_incidence_2020}).}












%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Structural Estimation of Model Parameters} \label{sec:struc_est}


In spite of its crucial role for the functioning of the judicial system of modern economic societies, the legal sector remains vastly understudied. 
This section exploits our equilibrium characterization in Lemma \eqref{eq_lem} and the exogenous nature of bankruptcy demand shocks to provide the first empirical estimate of the CES elasticity of substitution between skilled and unskilled labor in the legal sector, $\delta$ (Equation \eqref{eq:CES}).


The structural estimation proceeds as follows. After taking the logarithm of Equations (\ref{eq_s}), (\ref{eq_u}) we obtain,
\begin{equation} \label{ln_equilibrium}
               \ln (\s) = \alpha_{s} + \beta_{s}\ln(L) \qquad  \ln (\u) = \alpha_{u} + \beta_{u} \ln(L)
            \end{equation}
where $\beta_{s}=\frac{1}{1+\mathbf{\delta\rho_s}} $ and $\beta_{u}=\frac{1}{1+\mathbf{\delta\rho_u}}$. Then taking the logarithm of Equations (\ref{eq_ws}), and (\ref{eq_wu}), we get
    \begin{equation}\label{ln_equilibrium_w}
               \ln (w_s) = \alpha^{w}_{s} + \beta^{w}_{s}\ln(L) \qquad  \ln (w_{u}) = \alpha^{w}_{u} + \beta^{w}_{u} \ln(L)
    \end{equation}
where $\beta^{w}_{s}=\frac{\rho_{s}}{1+\mathbf{\delta\rho_s}}$ and $\beta^{w}_{u}=\frac{\rho_{u}}{1+\mathbf{\delta\rho_u}}$.
We then derive an expression for $\delta$
we rearrange equations (\ref{ln_equilibrium}) and (\ref{ln_equilibrium_w}), which simpilfy to:
%can then be rearranged algebraically and simplified as follows:
\begin{equation} \label{delta}
    \delta= \frac{1/\beta_{s}-1}{\frac{\beta^{w}_{s}}{\beta_{s}}}, \qquad \qquad \text{ or equivalently}, \qquad \qquad \delta= \frac{1/\beta_{u}-1}{\frac{\beta^{w}_{u}}{\beta_{u}}}
\end{equation}


To estimate equations (\ref{ln_equilibrium}) and (\ref{ln_equilibrium_w}) we collect \BLS \space data for skilled and unskilled workers in the legal industry over the period from 1991 to 2001 for the dependent variables $u$ and $w_u$.\footnote{
    We use NAICS codes 54111 and 54119 for a measure of skilled and unskilled legal sector labor respectively.}$^,$\footnote{We expand the sample to 2001 due to minimal data availability, in addition we do not consider forum shopping in this setting and thus do not need to restrict ourselves to the court competition era. Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} indicates our results hold through this period.}
Then, using bankruptcy shocks to instrument out the demand of legal services ($L$), we run a Poisson regression with county and state-year fixed effects to obtain estimates for $\beta_{u}$, and $\beta^{w}_{u}$.
Using estimates from these regression and (\ref{delta}),  
%Estimates from these regressions allow us to estimate $\delta$ using (\ref{delta})
%In doing so we are able to 
we provide first empirical estimate for the elasticity of substitution between skilled and unskilled labor for the production of legal services ($\delta$). 

Table \ref{tab:struct_est_delta} reports estimates for $\delta$, as well as $\beta$, $\beta^{w}$ for both labor types.
\begin{table}[H]
    \caption{Structural Estimation of CES parameter $\delta$.}
    \label{tab:struct_est_delta}
    \begin{threeparttable}
    \renewcommand{\TPTminimum}{\linewidth}
    \makebox[\linewidth]
        {
        \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
        \begin{tabular}{l*{5}{c}}
        \toprule
        &\multicolumn{1}{c}{}   &\multicolumn{1}{c}{(1)}        &\multicolumn{1}{c}{(2)}            &\multicolumn{1}{c}{(3)}        \\
        &\multicolumn{1}{c}{}   &\multicolumn{1}{c}{$\beta$}    &\multicolumn{1}{c}{$\beta^{w}$}    &\multicolumn{1}{c}{$\delta$}   & \multicolumn{1}{c}{Observations}   \\
        \midrule
        & Skilled               & 0.0121\sym{***}               & 0.0295\sym{***}                    & 33.445\sym{**}                & 790   \\
        &                       & (0.00225)                     & (0.000682)                        & (16.725)                      \\
        & Unskilled             & 0.0413\sym{***}               & 0.0384\sym{***}                   & 24.983\sym{*}                 & 765    \\
        &                       & (0.00984)                     & (0.00083)                         & (14.672)                      \\
        \bottomrule
        \multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
        \multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
        \end{tabular}
        }
    \begin{tablenotes}
        \item [] \textit{Note:} Columns (1) and (2) are Poisson regression estimates of log of employment level for unskilled labor in the legal industry and the log of average wage for unskilled workers in the legal industry on: \textit{(i) Treatment:} log of bankruptcies; \textit{(ii) Fixed Effects:} \countyDisY; \textit{(iii) Controls:} \controls. \clustercounty. \textit{Sample:} \sampleBRcounties. \textit{Period:} \sampleyearsExtendedPeriod. \textit{Sources:}  \sourceAVGWAGE. 
    \end{tablenotes}
    \end{threeparttable}
\end{table}



% \begin{threeparttable}
%     \makebox[\linewidth]
%     {
%     % \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%     \begin{tabular}{l*{4}{c}}
%         % Head
%         \toprule
%         &\multicolumn{1}{c}{(1)}        &\multicolumn{1}{c}{(2)}            &\multicolumn{1}{c}{(3)}        \\
%         &\multicolumn{1}{c}{$\beta$}    &\multicolumn{1}{c}{$\beta^{w}$}    &\multicolumn{1}{c}{$\delta$}    \\
        
%         % \midrule
        
%         \input{Regressions/Delta_unskilled_shock.tex}
        
%         % \bottomrule
%         \multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
%         \multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
%     \end{tabular}
%     }
% \end{threeparttable}

We estimate $\delta$ to be 33.4 and 25.0 when using data for skilled and unskilled labor, respectively. 
This result suggests that skilled and unskilled labor are strong substitutes in the legal sector. In line with the theory, these estimates are statistically equivalent to each other, both being within one standard deviation of the other.\footnote{The 95\% confidence interval for skilled ranges from .6641 to 66.2 and for unskilled  -3.77 to 53.74.}

In absence of previous estimates, to validate our identification strategy we compare our findings with previous attempts of estimating %the body of the literature that has attempted to estimate 
$\delta$
across broader sectors of the economy (e.g. \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{blankenau_industry_2011}). 
Our estimate is consistent with the findings in \citet{blankenau_industry_2011}, which document the elasticity of substitution across skill levels to be considerably higher for individual sectors than in the aggregate economy. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% APPENDIX STUFF %


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagebreak
\section{Model}\label{App:model}
This section gives a more rigorous treatment to the model discussed in section \ref{sec:TheModel}. Proofs for all results are included at the end of this section under \ref{App:Proofs}.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Households}
%%%%%%%%%%%%%%%%%%%%%%%%
    In each period $t$, households of type $j$ choose consumption $\cjt\in\mathbb{R}_{+}$ and labor hours $\njt\in\mathbb{R}_{+}$ in order to maximize \eqref{Utility}. 
    Note that because there is no savings, and the objective function is unchanged across periods, we can suppress the period index $t$ for brevity.
    From the FOC, we obtain the labor supply functions:
    \begin{multicols}{2}
        \begin{equation*}
            \s(w_s) = \left(\frac{w_{s}}{\gamma}\right)^{\frac{1}{\rho_{s}}}
        \end{equation*}
        
        \begin{equation*}
            \u(w_u) = \left(\frac{w_{u}}{\gamma}\right)^{\frac{1}{\rho_{u}}}
        \end{equation*}
    \end{multicols}
     
    It follows that the Frisch Elasticity of Labor Supply ($\epsilon_j$) for $j = \{s,u\}$ can be expressed as:
    \begin{equation}
        \epsilon_j = \frac{1}{\rho_{j}} 
    \end{equation}
    We make the following assumption on $\rho$ across households. 
    \begin{assumption}\label{elasticity}
        The elasticity of labor supply of skilled workers is lower than unskilled workers,
        i.e. $\rho_u < \rho_s$
    \end{assumption}
    \noindent This assumption is quite standard when modeling households that vary across skill and is grounded in a vast body of empirical evidence. 
    % Grounded on the vast empirical evidence for the relative elasticity of labor supply of skilled versus unskilled workers we make the following assumption.
    % We make the following assumption for


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Firms}
%%%%%%%%%%%%%%%%%%%%%%%%

    % Given CES production function \eqref{eq:CES}, 
    We consider skilled and unskilled labor to be imperfect substitutes. 
    In terms of \eqref{eq:CES} this corresponds to $\delta > 1$. \footnote{
            \citet{bowlus_wages_2017} provides a summary of the literature on this topic, where they refer to even the low end estimates being in the range of 1.4 to 1.8}\textsuperscript{,}\footnote{
            \citet{Autor18_lecture} describes the consensus estimate to be approximately 2 in the U.S. while the most commonly used estimate is 1.4.}\textsuperscript{,}\footnote{
            \citet{angrist_economic_1995} from the AER estimates implied elasticity of substitution between 16+ years of schooling and less than 12 to be approximately 2.}
    This is in accordance with the broad consensus of estimates for $\delta$ in the literature, and is without loss of generality to our main results.
    
    From \eqref{eq:CES}, $A_u$ and $A_s$ are the factor-augmenting technology terms for unskilled and skilled labor, respectively.
    \begin{assumption}\label{skillunskill}
        Skilled labor is more productive than unskilled labor, $A_u < A_s$.
    \end{assumption}
    \noindent This assumption is more of a definition, as clearly skilled labor should implicitly have a higher productivity. 
    
    Since markets are competitive, factors receive their marginal product as wages.
    \begin{equation}\label{ws=MP}
        w_{s} = 
        A_{s}^{\frac{\delta - 1}{\delta}} 
        \left[ 
        A_{u}^{\frac{\delta - 1}{\delta}}\left(\frac{\s}{\u}\right)^{-\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}
        \right]
        ^{\frac{1}{\delta - 1}} 
        = A_{s}^{\frac{\delta - 1}{\delta}} \left( \frac{L}{\s} \right)^{1/\delta}
    \end{equation}
    \begin{equation}\label{wu=MP}
        w_{u} = 
        A_{u}^{\frac{\delta - 1}{\delta}} 
        \left[ 
        A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\frac{\s}{\u}\right)^{\frac{\delta - 1}{\delta}}
        \right]
        ^{\frac{1}{\delta - 1}}
        = A_{u}^{\frac{\delta - 1}{\delta}} \left( \frac{L}{\u} \right)^{1/\delta}
    \end{equation}
    
    From (\ref{ws=MP}) and (\ref{wu=MP}) we obtain the following relationship for average wage in terms of relative factor intensity ($\s/\u$).  
        \begin{equation}\label{avg_wage}
            \overline{w} \equiv \frac{\u w_{u} + \s w_{s}}{\u + \s} 
            = \frac{\left[ 
            A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\s/\u\right)^{\frac{\delta - 1}{\delta}}
            \right]^{\frac{\delta}{\delta - 1}}}{1 + \s/\u}
        \end{equation}
    
    %%% LEMMA %%%
    \begin{lemma}\label{lem:skpremium_avgwage}
    If the skill premium is positive ($\frac{w_s}{w_u} > 1$), then the average wage $\overline{w}$ is increasing in $\frac{\s}{\u}$\\
    Where the skill premium is defined as:
    \begin{equation} \label{SP}
            \pi \equiv \frac{w_s}{w_u} = \left( \frac{A_{s}}{A_{u}} \right) ^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta}
    \end{equation}
    \end{lemma}  

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Equilibrium}
%%%%%%%%%%%%%%%%%%%%%%%%
    Lemma \ref{eq_lem} uses market clearing in the input markets of skilled and unskilled workers to derive equilibrium wages and employment for each type of worker. 

    % Note that $L(\s,\u)$ is the production of \textit{all} legal services for a local area. When a firm files for Chapter 11 bankruptcy the demand for legal services increases, which results in an increase in the equilibrium level of $L$ in the market for legal services. These bankruptcy shocks are used as instruments for variation in $L$, and as such appear in the model as an increase in $L$.
    
    % Thus, in equilibrium, the level labor for both types of workers increase in response to a bankruptcy shock, because \eqref{eq_s} and \eqref{eq_u} show that both $\s$ and $\u$ are increasing in $L$.
    
    In equilibrium, the amount of labor for both types of workers increase in response to a bankruptcy shock, because \eqref{eq_s} and \eqref{eq_u} show that both $\s$ and $\u$ are increasing in $L$.
    The next Lemma shows that the frisch elasticity of labor supply $\rho_j$ plays a crucial role in determining the responsiveness of the equilibrium levels of $\s^*$ and $\u^*$ change due to a bankruptcy shock.
    In particular, by taking the ratio of (\ref{eq_s}) and (\ref{eq_u}), we formalize the compositional effect of exogenous increases in the demand for legal services.
        
    %%% LEMMA %%%
    \begin{lemma}\textbf{Compositional Channel.}\label{lem:ratio_su}
        Given Assumptions \ref{elasticity} and \ref{skillunskill}, an increase in the demand of legal services $L$ tilts the composition of workers towards unskilled workers
        \[\frac{\partial \left[\frac{\s^*}{\u^*}\right] }{\partial L} < 0 \]
    \end{lemma}
    
    Similarly, bankruptcy shocks ($L>0$) increase wages for both skilled and unskilled labor (Eqs. \eqref{eq_ws} and \eqref{eq_wu}). Yet, the effect on \textit{average} wage is less clear.
    Proposition \ref{prop_main} uses Lemmas \ref{lem:skpremium_avgwage}, \ref{eq_lem}, and \ref{lem:ratio_su} to derive the relationship between $L$ and average wage.


%%%%%%%%%%%%%%%%%%%%%%%%
 \subsection{Forum Shopping}\label{App:model_forumshopping}
%%%%%%%%%%%%%%%%%%%%%%%%

    This section incorporates forum shopping to the model through the demand for legal services $L$. 
    We define $BR$ to be a measure of the bankruptcy shock, such as the number of local firms currently undergoing bankruptcy proceedings. 
    Similarly, let $FS$ be a measure of how much of the bankruptcy shock is being forum shopped away. When there is no shock, $BR = FS = 0$. 
    If there is a shock, then $BR \in\mathbb{R}^{++}$ and $FS \in [0,BR]$. The proportion of the bankruptcies that forum shops is the ratio $f \equiv \frac{FS}{BR} \in [0,1]$.
    
    The magnitude of the bankruptcy shock is $h(BR,f) \in \mathbb{R}^{+}$. Which takes the following functional form using $\lambda>0$ as a scaling parameter.  
    \begin{equation}
    \begin{split}
        h(BR,f) & = \lambda(1-f)BR \\
                                & = \lambda(BR-FS)
    \end{split}
    \end{equation}
    
    Next, we split $L$ into two parts, $L_{BR}$ the quantity of legal services for bankruptcy, and $L_{other}$ the quantity of all other legal services. The quantity of bankruptcy legal services $L_{BR} = \overline{L}_{BR}+h(BR,f)$. Where $\overline{L}_{BR}$ is the steady state level of legal services in the bankruptcy sector. 
    \begin{equation}
    \begin{split}
        L & = L_{BR} + L_{other} \\ & = \overline{L}_{BR}+ h(BR,f)+ L_{other}
    \end{split}
    \end{equation}
    \noindent Thus a bankruptcy has the following effect on the quantity demanded of legal services:
    \begin{equation}
    \begin{split}
        \frac{\partial L}{\partial BR} = \left(\frac{\partial L}{\partial h(BR,f)} \right) \left(\frac{\partial h(BR,f)}{\partial BR}\right) = \lambda (1-f) \geq 0
    \end{split}
    \end{equation}
    \noindent Similarly, we obtain the effect of a bankruptcy on employment in the legal sector. 
    \begin{equation}
    % \begin{split}
        \frac{\partial \s}{\partial BR}  = \left(\frac{\partial \s}{\partial L}\right) \left(\frac{\partial L}{\partial BR}\right) = \left(\frac{\partial \s}{\partial L}\right) \lambda (1-f)
    % \end{split}
    \end{equation}
    \begin{equation}
    % \begin{split}
        \frac{\partial \u}{\partial BR}  = \left(\frac{\partial \u}{\partial L}\right) \left(\frac{\partial L}{\partial BR}\right) = \left(\frac{\partial \s}{\partial L}\right) \lambda (1-f)
    % \end{split}
    \end{equation}
    Clearly both of these are decreasing in $f$, which combined with Lemma \ref{eq_lem}, gives us the following relationship between forum shopping and the shock:
    
    \begin{proposition}\label{prop:BR_FS} Skilled and unskilled labor both increase with bankruptcies;
    \begin{equation}
         \frac{\partial \s}{\partial BR} \geq 0 \qquad \frac{\partial \u}{\partial BR} \geq 0
    \end{equation}
    However, this effect is decreasing with respect to forum shopping;
    \begin{equation}
       \frac{\left[\frac{\partial \s}{\partial BR}\right]}{\partial FS} < 0\qquad \frac{\left[\frac{\partial \u}{\partial BR}\right]}{\partial FS} < 0
    \end{equation}
    \end{proposition}
    \noindent Proposition \ref{prop:BR_FS} is illustrated by figures \ref{Mech3} and \ref{Mech4} in the Appendix \ref{App:mechanism}. 

    


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{figure}{3}
\subsection{Mechanism}\label{App:mechanism}
\begin{figure}[h]
\begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width = 0.9\textwidth]{Graphs/Mechanism1.pdf}
    \caption{Isoquant $L(\s,\u)=\overline{L}_{BR}$}
    \label{Mech1}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width = 0.9\textwidth]{Graphs/Mechanism2.jpg}
    % \inkscape{Mechanism2}
    \caption{Cost minimizing bundle given $\overline{L}$}
    \label{Mech2}
\end{subfigure}

\begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width = 0.9\textwidth]{Graphs/Mechanism3.jpg}
    % \inkscape{Mechanism2}
    \caption{Shift in isoquants due to BR shock w/o FS.}
    \label{Mech3}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width = 0.9\textwidth]{Graphs/Mechanism4.jpg}
    % \inkscape{Mechanism2}
    \caption{Dampening effect of forum shopping.}
    \label{Mech4}
\end{subfigure}
\end{figure}

    This section discusses the economic intuition behind the propositions derived in the model section. Consider the isoquant for the production of legal services $L(\s,\u)=\overline{L}_{BR}$ in a local area, shown in Figure \ref{Mech1}. Here, $\overline{L}_{BR}$ refers to the steady state level of demand for bankruptcy legal services. Given the level of demand $\overline{L}_{BR}$ the firm then chooses their optimal input bundle, 
    $A = (n_{s1}, n_{u1})$, satisfying the tangency condition for cost minimization $MRTS = MP_s/MP_u = w_s/w_u$. 
    In terms of our model, this tangency condition characterizes the skill premium $(\pi)$ from Lemma \ref{lem:skpremium_avgwage}. 
    \begin{equation}\label{skpremium_avgwage}\tag{SP}
        \pi \equiv \frac{w_s}{w_u} = \left( \frac{A_{s}}{A_{u}} \right) ^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta}
    \end{equation}
    This relationship is shown in Figure \ref{Mech2}. Using (\ref{skpremium_avgwage}) the slope of the dashed line corresponds to the left side of the equality and the slope of the isoquant (MRTS) is given by the right side. Thus these two expressions are only equal in optimum, i.e. when the tangency condition is satisfied. 
    
    
    When one or more firms file for bankruptcy \textit{locally} we see an increase in demand for legal services. 
    Given that all the firms are filing locally the quantity of legal services produced increases by the full amount of the shock, $h(BR,0) = \lambda BR$. This is shown in Figure \ref{Mech3} by the outward shift in the isoquant, changing the firms optimal choice of inputs from point $A = (n_{s1}, n_{u1})$ to point $B = (n_{s2}, n_{u2})$. Proposition \ref{prop_main} characterizes the relationship between these two bundles. Proposition \ref{prop_main} tells us that while the amount of both types of labor increases, the relative factor intensity of skilled labor decreases, $\mathbf{\frac{n_{s2}}{n_{u2}} < \frac{n_{s1}}{n_{u1}}}$. 
    
    
    However, the magnitude of this shock is dampened if some, or all, of the bankrupt firms forum shop to a venue outside their local area. Accordingly, the increase in production due to the shock, $h(BR,f)= \lambda(1-f)BR$, depends on the proportion of the firms who chose to forum shop, $f$. This can be seen graphically in Figure \ref{Mech4}, where $C = (n_{s3},n_{u3})$ is the optimal bundle when forum shopping occurs. In this setting, using Proposition \ref{prop_main} and Proposition \ref{prop:BR_FS}, it is clear that the relationship between the optimal bundles satisfies $n_{s2} > n_{s3} \geq s_1$, and $n_{u2} > n_{u3} \geq u_1$. However, due to the inelastic nature of skilled labor $\mathbf{\frac{n_{s2}}{n_{u2}} < \frac{n_{s3}}{n_{u3}} \leq \frac{n_{s1}}{n_{u1}}}$. Where the weak inequalities approach equality as $f$ approaches one. 
    
    Figure \ref{Mech4} reconciles the \textit{joint} dynamics on the legal sector employment and wages observed in Table \ref{tab:MainEmpLvl_BRonlyFE} and Table \ref{tab:avg_wage_reg_noBRsplit}, respectively.


\newpage
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proofs}\label{App:Proofs}
We start by proving Lemma \ref{lem:skpremium_avgwage}, which says that if skilled wage is greater than unskilled wage, then average wage is increasing if the factor intensity of skilled workers increases.

\begin{proof1}(Lemma \ref{lem:skpremium_avgwage})\\
It follows directly from \eqref{ws=MP} and \eqref{wu=MP} that the skill premia can be written as,
\begin{equation} \tag{SP}
        \pi \equiv \frac{w_s}{w_u} = \left( \frac{A_{s}}{A_{u}} \right) ^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta}\;.
\end{equation}

\noindent Then taking the derivative of the average wage from \eqref{avg_wage},
\begin{equation}
\begin{aligned}[b]
    \frac{\partial \,\overline{w}}{\partial \frac{\s}{\u}} &=  
    \left( \frac{\overline{w}}{1 + \frac{\s}{\u}} \right)  A_{s}^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta} \left[ 1 - \left( \frac{A_{s}}{A_{u}} \right) ^{-\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {1/\delta}\right] \\
    & =  \left( \frac{\overline{w}}{1 + \frac{\s}{\u}} \right)  A_{s}^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta} \left[ 1 - \frac{1}{\pi} \right]\;,
\end{aligned}
\end{equation}
which is greater than 0, if and only if the skill premia is positive (i.e. $\pi \equiv \frac{w_s}{w_u} > 1$).
\end{proof1}



%%%%%
% Next we prove Lemma \ref{eq_lem}, in doing so we also show the derivation of labor supply and demand.

\begin{proof1}(Lemma \ref{eq_lem})\\
\noindent The period index $t$ will be suppressed for clarity. We first simplify the objective function from \eqref{Utility} by replacing consumption with the budget constraint, which will be binding in optimum. Then by taking the first order conditions we obtain the labor supply functions for type $j \in \{s,u\}$,
\begin{equation*}
    \nj = \left(\frac{\wj}{\gamma}\right)^{\frac{1}{\rho_{j}}}\; ,
\end{equation*}
and similarly the inverse labor supply,
\begin{equation*}
    \wj = \gamma \cdot \nj^{\rho_j}\; .
\end{equation*}
As usual, to get an expression for equilibrium, we set the inverse labor supply equal to inverse labor demand from \eqref{ws=MP} and \eqref{wu=MP} as follows,
\begin{equation*}
    \gamma \cdot \nj^{\rho_j} = A_{j}^{\frac{\delta - 1}{\delta}} \left( \frac{L}{\nj} \right)^{1/\delta}\;.
\end{equation*}
Then solving for $\nj$,
\begin{equation*}
    \nj^{*}(L) = [\gamma^{-\delta} A_{j}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_j}}} \;,
\end{equation*}
and plugging the expression back in to the inverse labor supply,
\begin{equation*}
    w^{*}_{j}(L) = \gamma\left( A_{j}^{\delta - 1} L^{\rho_j}\right)^{\frac{1}{1+\delta\rho_{j}}} \; ,
\end{equation*}
which completes the proof. 
\end{proof1}




%%%
\begin{proof1}(Lemma \ref{lem:ratio_su} \textit{Compositional Channel})\\
We with the expression of $\frac{\s}{\u}$ using Lemma \ref{eq_lem};
\begin{equation}
    \frac{\s}{\u} = 
    \frac{[\gamma^{-\delta} A_{s}^{\delta - 1} L]^{\frac{1}{\theta_s}}}
    { [\gamma^{-\delta} A_{u}^{\delta - 1} L]^{\frac{1}{\theta_u}}}
     = \Big(\frac{A_s^{\theta_s}}{A_u^{\theta_u}}\Big)^{\delta - 1} \gamma^{-\delta(\theta_s - \theta_u)} L^{\theta_s - \theta_u}
\end{equation}
where $\theta_j \equiv \frac{1}{1+\mathbf{\delta\rho_j}}$ for type $j \in \{s,u\}$. A bankruptcy shock enters our model as an increase in $L$, so the derivative of the above expression with respect to $L$ reflects this shock,
\begin{equation}
    \frac{\partial \frac{\s}{\u}}{\partial L} = \Big(\frac{A_s^{\theta_s}}{A_u^{\theta_u}}\Big)^{\delta - 1} \gamma^{-\delta(\theta_s - \theta_u)} L^{\theta_s - \theta_u -1}(\theta_s - \theta_u) \leq 0\;.
\end{equation}
The last inequality uses the fact that all of the terms in the above expression are positive by definition, except for $\theta_s - \theta_u$ which is negative as a result of Assumption \ref{elasticity}. 
\end{proof1}


%%%
\begin{proof1}(Proposition \ref{prop_main})\\
It is clear that Part (i) is true by taking the derivative with respect to $L$ of the equilibrium equations from Lemma \ref{eq_lem}. Then Part (ii) follows directly from Lemma \ref{lem:skpremium_avgwage} and Lemma \ref{lem:ratio_su}, given that $\rho_u < \rho_s$ and $\frac{w_s}{w_u} > 1$.
\end{proof1}


==> Drafts/Old/Avg_Wage.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    \subsection{Bankruptcy Shocks and Legal Wages}\label{sec:wag}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Thus far we have shown the effect of bankruptcy shocks on local legal sector employment. We complete our analysis by studying the effect on average wages.
    
    \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE_noBRsplit}{tab:avg_wage_reg_noBRsplit}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}

    
    Table \ref{tab:avg_wage_reg_noBRsplit} reports a \textit{negative} and non statistically significant effect of bankruptcy shocks, both in our benchmark model (Column (1), model \eqref{eq:spec_bench_BR}) or we account for forum shopping (Column (2), model \eqref{eq:spec_bench_BR}).
    
% \marginpar{\scriptsize{\textcolor{red}{If our story is that the shock means that avg wage goes down b/c more unskilled labor is hired do sticky wages matter?}}}
    
    Before discussing the sign of our findings, we explore their significance. Prices tend to be stickier than quantities (CITATION HERE ON PAPER WITH STICKY WAGE ESTIMATION). Hence, larger shocks may be needed in order to trigger a general equilibrium effect (EXAMPLES OF PAPER WHEN THIS HAPPENED).
    We explore this idea in Column (3) by splitting bankruptcy and forum shopping in Lopucki (large firms' bankruptcies) and Compustat (small firms' bankruptcies) group.
    Consistent with this interpretation, we find a statistically significant effect for the large (Lopucki) bankruptcy group, but not in the small group. 
    
    Similar to the results on employment level, Table \ref{tab:avg_wage_reg_noBRsplit} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had.
    
    The sign of our finding is puzzling. Bankruptcy shocks are demand shocks to the level of legal services. Basic economic theory would suggests the associated increase in the conditional input factor demands to increase wages, not decrease them. 
    Next section uses a model with skilled and unskilled workers to reconcile this finding via a compositional channel.
    Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %, i.e. quantity in the market for labor in the legal sector. 
%     %In this section we investigate bankruptcy shocks impact on price levels in the form of average wage to get a more complete picture of how legal sector labor markets respond to bankruptcy shocks.
    
%     In this section we investigate the effect on the average wage.
%     However, it is much more difficult to measure the impact of labor demand shocks on wage than on employment levels, because wages tend to be ``stickier'' than employment levels in the short run. Consistent with this predicted ``stickiness'' our results in Table \ref{tab:avg_wage_reg_noBRsplit} show a much smaller impact on wages than we saw on employment levels, and in turn lower significance with only column (3) estimating a significant impact from the bankruptcy shocks. 
    
%     Yet, despite the minimal significance, the direction of the estimated effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
%     Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
    
    
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % OLD VERSION WITH EXTRA COLUMN FOR LP CS BR SPLIT
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% Table \ref{tab:avg_wage_reg} reports our results for average wage in the legal sector. Columns (1), and (2), fail to show significance and column (3) shows minimal significance for the estimated effect of a bankruptcy on average wage. 
% This result is consistent with the idea that wages tend to be ``stickier" than employment levels in the short run and require a larger shock to record a meaningful change. 
% Column (4) corroborates this hypothesis, showing that large firm bankruptcy shocks ``Bankruptcies (LP)'' indeed have a statistically and economically significant effect.

% Yet, the direction of the effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
% Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.

% Similar to the results on employment level, Table \ref{tab:avg_wage_reg} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 
% \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE}{tab:avg_wage_reg}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}
% \fi
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Drafts/Old/Intro_BR_Venue_Bill_8-30.tex <==
% \iffalse
% \textcolor{red}{
% % On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck presented the bipartisan Bankruptcy Venue Reform Act to the press.
% On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% }

% \textcolor{red}{
% TO BE CONTINUED: 
% - we complement this view (Focusing on stakeholder) by assessing the general equilibrium implications of forum shopping
% - attache literature that says that health of major employees is important
% - ISSUE: why time period. Maybe we get around by doing the analysis only for Lopucki bankruptcy for the entire time period and then focus on the court competition era for justify the claim
% }
% \fi





Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
The adverse effects of bankruptcy shocks on overall local employment, however, hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).
We contribute to the literature by focusing on a sector that directly relates to bankruptcy shocks via a demand channel: the legal services. 
%studying the effect on the labor market of a particular sector, which relates to bankruptcy shocks via a demand channel: the legal services. 
% This paper is the first to document  
% the labor market response of a sector which is directly related to bankruptcy shocks via a demand channel: the \textit{legal} labor market.
%This paper contributes to the literature by identifying 
%is the first to study both theoretically and empirically 
%, which at odds with the rest of the local economy, benefits from the higher demand of legal services produced by the bankruptcy shocks.
%This paper is the first to document the effect on the legal industry labor markets, a sector related to bankruptcy shocks via a demand channel. 

% At odds with the contractionary effect observed in the local economy,
% %In opposition to the usual local contractionary impacts, 
% the labor market for the legal industry benefits from the increased demand for legal services, and subsequently acts as a potential channel for growth in the bankrupt firm’s surrounding area.
% We estimate that during the early 90's the Chapter 11 bankruptcy of a publicly traded firm is associated with a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. 
% Yet, this channel is muted when firms are allowed to file away from their headquarters. Focusing on a time period where the phenomenon of foru

\iffalse
%%%% 1
the legal industry covers professions in the areas of law, courts, law enforcement, and corrections and rehabilitation. However, this industry also includes a wide range of legal-related occupations that are found in other fi elds and industries. Many of these professions offer different litigation services to attorneys, such as trial con- sulting, expert witness services, or private investigation.
%%% 2 
Among the legal support positions that law offi ces seek to fi ll are qualifi ed paralegals, legal secretaries, receptionists, and legal technology support staff.
%%% 3 JUDICIAL ASSISTANT
Judicial Assistants help judges in local, state, federal, and tribal courts oversee judicial activities so that courts work effectively and efficiently every day. Their job is to provide judges with administrative, secretarial, and clerical support.
%%% 4 
paralegals, lawyers, clerks of courts, or court administrators
Judicial Law Clerk 16
Staff Attorney, Court 18
Bankruptcy Judge 62
% LEGAL SUPPORT PROFESSIONALS
(Legal Support Professional 82 Legal Receptionist 85 Legal Word Processor 87 Information Technology (IT) Professional 89 Legal Secretary 92 Paralegal 94 Legal Administrator 96 Human Resources Manager (Law Firm) 98 Marketing Manager (Law Firm) 100 Legal Technology Consultant 102 Legal Search Consultant 104
LITIGATION)
% COURT SUPPORT STAFF
Bailiff (Local and State Courts) 138 Court Administrator 140 Court Analyst 142 Court Clerk 144 Court Interpreter 146 Court Reporter 149 Judicial Assistant 152 Scopist 154
% PARALEGAL
Paralegals, or legal assistants, have been trained in substan- tive and procedural law and are qualified to perform various legal tasks. They may be involved in transactional matters, such as drafting contracts or reviewing trust instruments, or they may work on civil litigation or criminal defense cases. However, paralegals, unlike attorneys, cannot practice law. Paralegals cannot offer legal advice. They cannot accept clients or represent clients in courts, and paralegals cannot establish

\fi

The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
%%%%%%%%%%%%%%%
In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} 
    % $^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
%%%%%%%%%%%%%%%    
At odds with the rest of the local economy, local legal labor markets benefit from the increased demand for legal services, partially offsetting the contractionary effect on the bankrupt firm’s surrounding area.
%. Hence, they balance the contractionary effect of bankruptcy shocks on the distressed firm’s surrounding area.

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we
%We 
estimate that during the early 90's 
%the Chapter 11 bankruptcy of a publicly traded firm is
bankruptcy reorganizations are associated with 
a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars.  
%Despite this we estimate that 
Across the U.S. bankruptcies contribute an average of roughly 10,000 jobs, with wages adding up to nearly \$1 billion in 2021 dollars, each year.\footnote{
    In nominal terms we estimate this to be an average of \$523 million worth of employment each year from 1991 to 1996 inclusive.}

Our results also show that these gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We document that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).
% We document that more than 23\% of the potential employment gains are \textit{exported away} each year, on average. 
% Despite this, we estimate that bankruptcies contribute an average of \$523 million (not adjusted for inflation) worth of employment each year to local communities, or roughly 10,000 jobs. 

We measure the demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. Chapter 11 bankruptcy cases for large firms are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
    The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Lawyers and judges: those are the two occupations—and career options—that people usually think of when it comes to law or the legal industry. Indeed, lawyers and judges are the major players, but they would not be able to perform their jobs without legal, offi ce, and administrative assistance from paralegals, legal clerks, secretaries, document proces- sors, administrators, technology specialists, and other pro- fessionals. All those support professionals in the law offi ce and courtroom are part of the legal industry.
% BOOK CAREER OPPORTUNITIES IN LAW AND THE LEGAL INDUSTRY
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textcolor{purple}{We contribute to the literature, by building a unique database that expands the universe of large bankruptcies in \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.}\footnote{
%         Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).}
This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
} to a critical industry.
%vastly understudied industry that is critical to the overall economy. 
% Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
%     \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
% In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
%     Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%     \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
% } 
%Bankruptcy shocks provide a unique source of variation to disentangle internal dynamics of this industry.

    %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
    Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
    Unlike much of the applied economics literature that exploits an event study framework our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
    Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
    We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.
    We adopt an economic history approach and  focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
        For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}

    
    %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
    The historical period we focus 
    on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
    Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.
    %This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
    %%%%%%%%%%%
    During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
        \cite{ellias_bankruptcy_2019} finds that in recent years more than \%60 of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
        }
    %%%%%%%%%

% \iffalse
% %%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
% % @Ale -- I the first sentence of the Court competition era paragraph to the previous paragraph so it leads into the next paragraph better and the second paragraph is more focused on one thing. 
% %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
% Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
% Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
% Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
% We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.

% We adopt an economic history approach and 
% %Similar to the economic history approach, we 
% focus our analysis
% %To handle the complex nature of our treatment, we distinguish from previous work (cite XXX XXX XXX) and propose a novel identification strategy.differentiate from previous work treatment from Chapter 11 bankruptcies, we propose an approach that differentiates us from the previous literature. 
% %a different approach.  
% %Due to the complex nature of treatment from Chapter 11 bankruptcies, our identification strategy uses an approach similar to much of the economic history literature that focuses 
% on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
%     For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
% %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
% In particular, we focus 
% on the `Court Competition Era', a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
% Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law in order to file for Chapter 11 bankruptcy reorganization far away from their headquarters.
% This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping' (see Section \ref{sec:ForumShopping} for more details).
% \fi

%%%%%%%%%
Our identification strategy focuses on this abrupt change in bankruptcy filings practices\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
to create variations in the location of demand for legal service from Chapter 11 bankruptcies.
\textcolor{red}{Although it is well established that the strategic bankruptcy plan is drafted by a handful of highly specialized law companies (mostly located in New York), the material handling of Chapter 11 bankruptcy requires hiring a lot of unskilled, etc.\\
WE ESTIMATE THAT 20\% of the jobs LOST TO DELAWARE AND NEW YORK. 
}
\\
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus when a firm forum shops the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
% The legal services for bankruptcy proceedings will typically be located near the filing court because they must be certified to practice in that area, be familiar with local bankruptcy practices, and be able to attend proceedings and file paperwork at the courthouse.
% Thus when a firm forum shop the legal sector demand shock is effectively exported away from their local economy. This transfer in potential legal service demand is particularly pronounced because forum shopping firms often file a great distance away from their local area. 
% For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
%     Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the filing court which are exogenous to the local economy where the firm is headquartered.

A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.    

% One of our empirical strategy's identifying assumptions is that
% % Our identification strategy relies on 
% Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
% The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
% To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
% Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.

% \textcolor{red}{Equal pretrends/placebo stuff/matching}

%%%%%%%%%%% THEORETICAL ECONOMETRIC APPROACH %%%%%%%%%%% 
% \textcolor{red}{FUZZY DID \citet{de_chaisemartin_two-way_2020} also cite the package stuff}
    

% \marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
% During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% % where they \textbf{believed judges of that court would be more favorable to debtors}. 
% This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
% During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).
    
    
    

%, in hopes that the judges of that court will be more favorable to debtors.
% In particular we focus our analysis 
% on the `Court Competition Era', a period from 1991 to 1997 where stipulations of US corporate bankruptcy law created exogenous variations in the location of the court where the bankruptcy was filed (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
%In this period, firms started exploit US corporate bankruptcy law's flexible criteria for where a debtor must file.
%This variation arises because large firms are able 
%During the 1991-1997 period, 
%In this period, bankruptcy judges starting competing against each other in order to attract Ch 11 filings.

\iffalse
%%%%%%%%%%% WHY REORG NOT LIQ %%%%%%%%%%% 
We focus on Chapter 11 `reorganization' bankruptcies for three main reasons. First, it allows us to exploit forum shopping which creates variation in filing location allowing for clearer identification. Second, the legal proceedings for Chapter 11 bankruptcies are considerably more complex and require much larger legal teams than Chapter 7 bankruptcies, thus creating a larger demand shock on legal services.\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
}
Third, the vast majority of publicly traded corporations choose Chapter 11 when they file in hopes of achieving a better outcome for shareholders than they likely would with Chapter 7 cases.\footnote{
    In the \LP\; between 1980 and 2014 only one instance of a Chapter 7 bankruptcy compared to 962 Chapter 11 bankruptcies during that time.} 


\textcolor{purple}{
In doing so we make several incidental contributions to the literature. 
\marginpar{\scriptsize\textcolor{red}{CHOOSE BETWEEN THIS OR THE PURPLE SECTIONS THAT SAY THE SAME THING IN OTHER PLACES. \\~\ maybe move this paragraph to end of the intro?}}
First, we create a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
% Second, we contribute to a considerable body of literature from legal professionals and academics pertaining to forum shopping (e.g. \cite{Baird87}; \cite{EisenbergLopucki1999}; \cite{warren_bankruptcy_1987};
% \cite{Baird97}; \cite{Algero99}; \cite{Lopucki06}; \cite{LopuckiKalin00}; \cite{ThomasRasmussen01}; \cite{Cole03}; \cite{Zywicki06}; \cite{skeel_1998})
% which analyzes the implications of forum shopping on bankruptcy outcomes for the firm and it's creditors, and debates the ethics of forum shopping within the scope of the bankruptcy per se. Our focus differs from this literature. Rather than focusing on the bankruptcy outcomes for the creditors and debtors involved, we explore the general equilibrium implications of bankruptcies and forum shopping for the firm's local area. Instead of taking a side of the debate on the ethics of forum shopping we add meaningful and overlooked context to their debate.
}
Furthermore, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy.


This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping'.
When a firm forum shops they are filing in a bankruptcy court different from the local court that typically services the area where the firm's headquarters are located.\footnote{
    In our context we only consider district level forum shopping. It is worth noting that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.} 

\marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% where they \textbf{believed judges of that court would be more favorable to debtors}. 
This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).


\fi
    
    
%%%%%%%%%%% MAIN FINDINGS %%%%%%%%%%% 
To address our question, we construct a novel database 
%that contributes to literature relating to both forum shopping and Chapter 11 bankruptcies in general. Our database
that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, yearly fixed effects for each of the 94 U.S judicial districts and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
Thus we show it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million worth of employment.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 


%%%%%%%%%%% PUZZLE ON WAGES %%%%%%%%%%% 
Counter-intuitively, we find evidence that Chapter 11 bankruptcy reorganizations of large publicly traded firms are associated with a decrease in the county level average wage for the legal sector.
% Counter-intuitively, we find that Chapter 11 bankruptcy reorganizations of publicly traded firms are associated with a 1.5\% drop in the average county wage in the legal sector.
We reconcile this puzzling finding with a \textit{compositional} effect. 
To do this we specialize the canonical model from \citet{Acemoglu_Autor_2011} to the legal labor markets. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and unskilled labor (paralegals, law clerks, etc.).
Skilled workers are more productive but their labor supply is more inelastic than unskilled workers.
In this environment, bankruptcy shocks boost the demand of legal services, prompting an increase in the firm's demand for both types of workers.
Since skilled workers have a relatively inelastic labor supply, bankruptcy shocks shift the composition of legal workers towards unskilled workers, causing a drop in the average wage.


%%%%%%%%%%% MODEL %%%%%%%%%%% 
% Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
% In doing so we contribute to the extensive body of the empirical literature (e.g. \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}) that aims to estimate the elasticity of substitution between high and low skilled labor for CES production functions. 
% We differ from this existing literature by being the first to provide empirical evidence for the elasticity of substitution across skill levels in the context of the legal industry. With this novel setting we not only find evidence that supports previous estimates that skilled and unskilled labor are imperfect substitutes, but we are also able to find point estimates for this parameter.

Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
In doing so we contribute to the extensive body of the empirical literature that aims to estimate the elasticity of substitution between high and low skilled labor (e.g. \cite{katz_changes_1992}, \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}).
Unlike much of this literature we provide empirical evidence for the elasticity of substitution across skill levels at an industry level, and are the first to do so in the context of the legal industry. 
With this novel setting we find additional evidence supporting \citet{blankenau_industry_2011} who predict this elasticity to be higher at the industry level than it is at an aggregate level.  

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to the literature. 
First, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy. Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.

==> Drafts/Old/Intro_Draft_V1.tex <==
On April 7th 2021 the Bill of this forum shopping at the house.
The purpose 

Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
The adverse effects of bankruptcy shocks on overall local employment, however, hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).
% This paper is the first to document  
% the labor market response of a sector which is directly related to bankruptcy shocks via a demand channel: the \textit{legal} labor market.
This paper contributes to the literature by identifying 
%is the first to study both theoretically and empirically 
the effect on the labor market of a particular sector, which relates to bankruptcy shocks via a demand channel: the legal services. %, which at odds with the rest of the local economy, benefits from the higher demand of legal services produced by the bankruptcy shocks.
%This paper is the first to document the effect on the legal industry labor markets, a sector related to bankruptcy shocks via a demand channel. 

% At odds with the contractionary effect observed in the local economy,
% %In opposition to the usual local contractionary impacts, 
% the labor market for the legal industry benefits from the increased demand for legal services, and subsequently acts as a potential channel for growth in the bankrupt firm’s surrounding area.
% We estimate that during the early 90's the Chapter 11 bankruptcy of a publicly traded firm is associated with a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. 
% Yet, this channel is muted when firms are allowed to file away from their headquarters. Focusing on a time period where the phenomenon of foru

The legal industry plays a key role
%Despite its key role 
in the functioning of 
% the judicial system of 
modern economic societies.
Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
%%%%%%%%%%%%%%%
In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
%%%%%%%%%%%%%%%    
At odds with the rest of the local economy, local legal labor markets benefit from the increased demand for legal services, hence partially offsetting the contractionary effect on the bankrupt firm’s surrounding area.
%. Hence, they balance the contractionary effect of bankruptcy shocks on the distressed firm’s surrounding area.

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we
%We 
estimate that during the early 90's 
%the Chapter 11 bankruptcy of a publicly traded firm is
bankruptcy reorganizations are associated with 
a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. We estimate 
We also show that this channel is muted when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
%Focusing on a time period where this phenomenon was particularly pronounced, 
\textcolor{red}{We document that more than 23\% of the potential employment gains are \textit{exported away} each year, on average. Despite this, we estimate that bankruptcies contribute on average \$523 million (not adjusted for inflation) worth of employment each year to local communities, or roughly 10,000 jobs. 
TBD}

We measure the demand shocks to local legal services using Chapter 11 `reorganization' bankruptcies of publicly traded firms. Large firm's Chapter 11 bankruptcy cases are complex phenomena, that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
    The average professional fees amount to \$125 million in 2020 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
% \textcolor{purple}{We contribute to the literature, by building a unique database that expands the universe of large bankruptcies in \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.}\footnote{
%         Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).}
This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
} to a critical and understudied industry.
%vastly understudied industry that is critical to the overall economy. 
% Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
%     \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
% In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
%     Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%     \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
% } 
%Bankruptcy shocks provide a unique source of variation to disentangle internal dynamics of this industry.

    %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
    Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
    Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
    Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
    We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.
    We adopt an economic history approach and  focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
        For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}

    
    %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
    The historical period we focus 
    on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
    Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.
    %This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 



% \iffalse
% %%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
% % @Ale -- I the first sentence of the Court competition era paragraph to the previous paragraph so it leads into the next paragraph better and the second paragraph is more focused on one thing. 
% %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
% Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
% Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
% Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
% We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.

% We adopt an economic history approach and 
% %Similar to the economic history approach, we 
% focus our analysis
% %To handle the complex nature of our treatment, we distinguish from previous work (cite XXX XXX XXX) and propose a novel identification strategy.differentiate from previous work treatment from Chapter 11 bankruptcies, we propose an approach that differentiates us from the previous literature. 
% %a different approach.  
% %Due to the complex nature of treatment from Chapter 11 bankruptcies, our identification strategy uses an approach similar to much of the economic history literature that focuses 
% on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
%     For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
% %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
% In particular, we focus 
% on the `Court Competition Era', a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
% Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law in order to file for Chapter 11 bankruptcy reorganization far away from their headquarters.
% This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping' (see Section \ref{sec:ForumShopping} for more details).
% \fi

Our identification strategy, exploits forum shopping\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus when a firm forum shops the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
% The legal services for bankruptcy proceedings will typically be located near the filing court because they must be certified to practice in that area, be familiar with local bankruptcy practices, and be able to attend proceedings and file paperwork at the courthouse.
% Thus when a firm forum shop the legal sector demand shock is effectively exported away from their local economy. This transfer in potential legal service demand is particularly pronounced because forum shopping firms often file a great distance away from their local area. 
% For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
%     Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the filing court which are exogenous to the local economy where the firm is headquartered.

One of our empirical strategy's identifying assumptions is that
Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.    

    ROBUSTNESS CHECK THAT SHOW INDEPENDENT FROM LOCAL ECONOMY

% One of our empirical strategy's identifying assumptions is that
% % Our identification strategy relies on 
% Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
% The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
% To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
% Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.

\textcolor{red}{Equal pretrends/placebo stuff/matching}

%%%%%%%%%%% THEORETICAL ECONOMETRIC APPROACH %%%%%%%%%%% 
\textcolor{red}{FUZZY DID \citet{de_chaisemartin_two-way_2020} also cite the package stuff}
    

% \marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
% During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% % where they \textbf{believed judges of that court would be more favorable to debtors}. 
% This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
% During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).
    
    
    

%, in hopes that the judges of that court will be more favorable to debtors.
% In particular we focus our analysis 
% on the `Court Competition Era', a period from 1991 to 1997 where stipulations of US corporate bankruptcy law created exogenous variations in the location of the court where the bankruptcy was filed (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
%In this period, firms started exploit US corporate bankruptcy law's flexible criteria for where a debtor must file.
%This variation arises because large firms are able 
%During the 1991-1997 period, 
%In this period, bankruptcy judges starting competing against each other in order to attract Ch 11 filings.

\iffalse
%%%%%%%%%%% WHY REORG NOT LIQ %%%%%%%%%%% 
We focus on Chapter 11 `reorganization' bankruptcies for three main reasons. First, it allows us to exploit forum shopping which creates variation in filing location allowing for clearer identification. Second, the legal proceedings for Chapter 11 bankruptcies are considerably more complex and require much larger legal teams than Chapter 7 bankruptcies, thus creating a larger demand shock on legal services.\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
}
Third, the vast majority of publicly traded corporations choose Chapter 11 when they file in hopes of achieving a better outcome for shareholders than they likely would with Chapter 7 cases.\footnote{
    In the \LP\; between 1980 and 2014 only one instance of a Chapter 7 bankruptcy compared to 962 Chapter 11 bankruptcies during that time.} 


\textcolor{purple}{
In doing so we make several incidental contributions to the literature. 
\marginpar{\scriptsize\textcolor{red}{CHOOSE BETWEEN THIS OR THE PURPLE SECTIONS THAT SAY THE SAME THING IN OTHER PLACES. \\~\ maybe move this paragraph to end of the intro?}}
First, we create a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
% Second, we contribute to a considerable body of literature from legal professionals and academics pertaining to forum shopping (e.g. \cite{Baird87}; \cite{EisenbergLopucki1999}; \cite{warren_bankruptcy_1987};
% \cite{Baird97}; \cite{Algero99}; \cite{Lopucki06}; \cite{LopuckiKalin00}; \cite{ThomasRasmussen01}; \cite{Cole03}; \cite{Zywicki06}; \cite{skeel_1998})
% which analyzes the implications of forum shopping on bankruptcy outcomes for the firm and it's creditors, and debates the ethics of forum shopping within the scope of the bankruptcy per se. Our focus differs from this literature. Rather than focusing on the bankruptcy outcomes for the creditors and debtors involved, we explore the general equilibrium implications of bankruptcies and forum shopping for the firm's local area. Instead of taking a side of the debate on the ethics of forum shopping we add meaningful and overlooked context to their debate.
}
Furthermore, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy.


This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping'.
When a firm forum shops they are filing in a bankruptcy court different from the local court that typically services the area where the firm's headquarters are located.\footnote{
    In our context we only consider district level forum shopping. It is worth noting that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.} 

\marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% where they \textbf{believed judges of that court would be more favorable to debtors}. 
This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).


\fi
    
    
%%%%%%%%%%% MAIN FINDINGS %%%%%%%%%%% 
To address our question, we construct a novel database 
%that contributes to literature relating to both forum shopping and Chapter 11 bankruptcies in general. Our database
that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (Compustat), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, yearly fixed effects for each of the 94 U.S judicial districts and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
Thus we show it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million worth of employment.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

\textcolor{red}{ROBUSTNESS CHECK STUFF}




%%%%%%%%%%% PUZZLE ON WAGES %%%%%%%%%%% 
Counter-intuitively, we find evidence that Chapter 11 bankruptcy reorganizations of large publicly traded firms are associated with a drop in the county level average wage for the legal sector.
% Counter-intuitively, we find that Chapter 11 bankruptcy reorganizations of publicly traded firms are associated with a 1.5\% drop in the average county wage in the legal sector.
We reconcile this puzzling finding with a \textit{compositional} effect. 
To do this we specialize the canonical model from \citet{Acemoglu_Autor_2011} to the legal labor markets. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and unskilled labor (paralegals, law clerks, etc.).
Skilled workers are more productive but their labor supply is more inelastic than unskilled workers.
In this environment, bankruptcy shocks boost the demand of legal services, prompting an increase in the firm's demand for both types of workers.
Since skilled workers have a relatively inelastic labor supply, bankruptcy shocks shift the composition of legal workers towards unskilled workers, causing a drop in the average wage.


%%%%%%%%%%% MODEL %%%%%%%%%%% 
% Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
% In doing so we contribute to the extensive body of the empirical literature (e.g. \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}) that aims to estimate the elasticity of substitution between high and low skilled labor for CES production functions. 
% We differ from this existing literature by being the first to provide empirical evidence for the elasticity of substitution across skill levels in the context of the legal industry. With this novel setting we not only find evidence that supports previous estimates that skilled and unskilled labor are imperfect substitutes, but we are also able to find point estimates for this parameter.

Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
In doing so we contribute to the extensive body of the empirical literature that aims to estimate the elasticity of substitution between high and low skilled labor (e.g. \cite{katz_changes_1992}, \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}).
Unlike much of this literature we provide empirical evidence for the elasticity of substitution across skill levels at an industry level, and are the first to do so in the context of the legal industry. 
With this novel setting we find additional evidence supporting \citet{blankenau_industry_2011} who predict this elasticity to be higher at the industry level than it is at an aggregate level.  

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to the literature. 
First, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy. Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.

==> Drafts/Old/Intro_Draft_V1_old.tex <==
On April 7th 2021 the Bill of this forum shopping at the house.
The purpose 

Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
The adverse effects of bankruptcy shocks on overall local employment, however, hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).
% This paper is the first to document  
% the labor market response of a sector which is directly related to bankruptcy shocks via a demand channel: the \textit{legal} labor market.
This paper contributes to the literature by identifying 
%is the first to study both theoretically and empirically 
the effect on the labor market of a particular sector, which relates to bankruptcy shocks via a demand channel: the legal services. %, which at odds with the rest of the local economy, benefits from the higher demand of legal services produced by the bankruptcy shocks.
%This paper is the first to document the effect on the legal industry labor markets, a sector related to bankruptcy shocks via a demand channel. 

% At odds with the contractionary effect observed in the local economy,
% %In opposition to the usual local contractionary impacts, 
% the labor market for the legal industry benefits from the increased demand for legal services, and subsequently acts as a potential channel for growth in the bankrupt firm’s surrounding area.
% We estimate that during the early 90's the Chapter 11 bankruptcy of a publicly traded firm is associated with a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. 
% Yet, this channel is muted when firms are allowed to file away from their headquarters. Focusing on a time period where the phenomenon of foru

The legal industry plays a key role
%Despite its key role 
in the functioning of 
% the judicial system of 
modern economic societies.
Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
%%%%%%%%%%%%%%%
In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
%%%%%%%%%%%%%%%    
At odds with the rest of the local economy, local legal labor markets benefit from the increased demand for legal services, hence partially offsetting the contractionary effect on the bankrupt firm’s surrounding area.
%. Hence, they balance the contractionary effect of bankruptcy shocks on the distressed firm’s surrounding area.

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we
%We 
estimate that during the early 90's 
%the Chapter 11 bankruptcy of a publicly traded firm is
bankruptcy reorganizations are associated with 
a 1\% increase in annual legal employment for the affected county---worth about \$4 million for each year of the bankruptcy proceedings, in 2020 dollars. We estimate 
We also show that this channel is muted when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
%Focusing on a time period where this phenomenon was particularly pronounced, 
\textcolor{red}{We document that more than 23\% of the potential employment gains are \textit{exported away} each year, on average. Despite this, we estimate that bankruptcies contribute on average \$523 million (not adjusted for inflation) worth of employment each year to local communities, or roughly 10,000 jobs. 
TBD}

We measure the demand shocks to local legal services using Chapter 11 `reorganization' bankruptcies of publicly traded firms. Large firm's Chapter 11 bankruptcy cases are complex phenomena, that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
    The average professional fees amount to \$125 million in 2020 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
% \textcolor{purple}{We contribute to the literature, by building a unique database that expands the universe of large bankruptcies in \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.}\footnote{
%         Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).}
This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
} to a critical and understudied industry.
%vastly understudied industry that is critical to the overall economy. 
% Over the last decade, US legal expenses have exceeded for \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
%     \textcolor{red}{2.380 trillion 2010-2019, 1.299 trillion 2015-2019 Using same GDP data \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} }$^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
% In 2019, the industry GDP measured 280 billion, comparable in size to the US agricultural sector (175 billion).\footnote{
%     Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
%     \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
% } 
%Bankruptcy shocks provide a unique source of variation to disentangle internal dynamics of this industry.

    %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
    Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
    Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
    Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
    We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.
    We adopt an economic history approach and  focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
        For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}

    
    %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
    The historical period we focus 
    on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
    Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.
    %This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 



% \iffalse
% %%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
% % @Ale -- I the first sentence of the Court competition era paragraph to the previous paragraph so it leads into the next paragraph better and the second paragraph is more focused on one thing. 
% %%%%%%%%%%% EVENT STUDY FAIL %%%%%%%%%%% 
% Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is difficult.
% Unlike much of the applied economic literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
% Counties experiencing treatment---Chapter 11 bankruptcy shocks---are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
% We contribute to the previous literature (\citealp{bernstein_bankruptcy_2019}; \textcolor{red}{discussant paper}), by proposing an identification strategy that handles the complex nature of our treatment.

% We adopt an economic history approach and 
% %Similar to the economic history approach, we 
% focus our analysis
% %To handle the complex nature of our treatment, we distinguish from previous work (cite XXX XXX XXX) and propose a novel identification strategy.differentiate from previous work treatment from Chapter 11 bankruptcies, we propose an approach that differentiates us from the previous literature. 
% %a different approach.  
% %Due to the complex nature of treatment from Chapter 11 bankruptcies, our identification strategy uses an approach similar to much of the economic history literature that focuses 
% on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
%     For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
% %%%%%%%%%%% ECONOMIC HISTORY APPROACH %%%%%%%%%%% 
% In particular, we focus 
% on the `Court Competition Era', a period from 1991 to 1997 when bankruptcy judges started competing for prestigious and lucrative Chapter 11 filings (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
% Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law in order to file for Chapter 11 bankruptcy reorganization far away from their headquarters.
% This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping' (see Section \ref{sec:ForumShopping} for more details).
% \fi

Our identification strategy, exploits forum shopping\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus when a firm forum shops the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the legal service demand shock from Chapter 11 bankruptcies.
% The legal services for bankruptcy proceedings will typically be located near the filing court because they must be certified to practice in that area, be familiar with local bankruptcy practices, and be able to attend proceedings and file paperwork at the courthouse.
% Thus when a firm forum shop the legal sector demand shock is effectively exported away from their local economy. This transfer in potential legal service demand is particularly pronounced because forum shopping firms often file a great distance away from their local area. 
% For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
%     Figures calculated using the \LPlong.}


% Our identification strategy, exploits forum shopping\footnote{
%     In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
% to create variations in the location of the filing court which are exogenous to the local economy where the firm is headquartered.

One of our empirical strategy's identifying assumptions is that
Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.    

    ROBUSTNESS CHECK THAT SHOW INDEPENDENT FROM LOCAL ECONOMY

% One of our empirical strategy's identifying assumptions is that
% % Our identification strategy relies on 
% Chapter 11 bankruptcy filings of publicly traded firms are an exogenous proxy for the local demand of legal services.
% The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
% To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
% Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.

\textcolor{red}{Equal pretrends/placebo stuff/matching}

%%%%%%%%%%% THEORETICAL ECONOMETRIC APPROACH %%%%%%%%%%% 
\textcolor{red}{FUZZY DID \citet{de_chaisemartin_two-way_2020} also cite the package stuff}
    

% \marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
% During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% % where they \textbf{believed judges of that court would be more favorable to debtors}. 
% This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
% During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).
    
    
    

%, in hopes that the judges of that court will be more favorable to debtors.
% In particular we focus our analysis 
% on the `Court Competition Era', a period from 1991 to 1997 where stipulations of US corporate bankruptcy law created exogenous variations in the location of the court where the bankruptcy was filed (\citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}). 
%In this period, firms started exploit US corporate bankruptcy law's flexible criteria for where a debtor must file.
%This variation arises because large firms are able 
%During the 1991-1997 period, 
%In this period, bankruptcy judges starting competing against each other in order to attract Ch 11 filings.

\iffalse
%%%%%%%%%%% WHY REORG NOT LIQ %%%%%%%%%%% 
We focus on Chapter 11 `reorganization' bankruptcies for three main reasons. First, it allows us to exploit forum shopping which creates variation in filing location allowing for clearer identification. Second, the legal proceedings for Chapter 11 bankruptcies are considerably more complex and require much larger legal teams than Chapter 7 bankruptcies, thus creating a larger demand shock on legal services.\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
}
Third, the vast majority of publicly traded corporations choose Chapter 11 when they file in hopes of achieving a better outcome for shareholders than they likely would with Chapter 7 cases.\footnote{
    In the \LP\; between 1980 and 2014 only one instance of a Chapter 7 bankruptcy compared to 962 Chapter 11 bankruptcies during that time.} 


\textcolor{purple}{
In doing so we make several incidental contributions to the literature. 
\marginpar{\scriptsize\textcolor{red}{CHOOSE BETWEEN THIS OR THE PURPLE SECTIONS THAT SAY THE SAME THING IN OTHER PLACES. \\~\ maybe move this paragraph to end of the intro?}}
First, we create a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database, supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
% Second, we contribute to a considerable body of literature from legal professionals and academics pertaining to forum shopping (e.g. \cite{Baird87}; \cite{EisenbergLopucki1999}; \cite{warren_bankruptcy_1987};
% \cite{Baird97}; \cite{Algero99}; \cite{Lopucki06}; \cite{LopuckiKalin00}; \cite{ThomasRasmussen01}; \cite{Cole03}; \cite{Zywicki06}; \cite{skeel_1998})
% which analyzes the implications of forum shopping on bankruptcy outcomes for the firm and it's creditors, and debates the ethics of forum shopping within the scope of the bankruptcy per se. Our focus differs from this literature. Rather than focusing on the bankruptcy outcomes for the creditors and debtors involved, we explore the general equilibrium implications of bankruptcies and forum shopping for the firm's local area. Instead of taking a side of the debate on the ethics of forum shopping we add meaningful and overlooked context to their debate.
}
Furthermore, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy.


This phenomena of firms filing in a forum different from the local court is referred to as `forum shopping'.
When a firm forum shops they are filing in a bankruptcy court different from the local court that typically services the area where the firm's headquarters are located.\footnote{
    In our context we only consider district level forum shopping. It is worth noting that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.} 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.} 

\marginpar{\textcolor{red}{\scriptsize  Look up pro debtor judges in lit.}}
During the court competition era there was a large spike in the frequency of forum shopping because firms filing for bankruptcy (debtors) were able shop for a forum where judges of that court had reputations for giving more favorable outcomes to debtors. 
% where they \textbf{believed judges of that court would be more favorable to debtors}. 
This creates plausible independence between the firms choice to forum shop and characteristics of their local county that may affect legal employment in the firms county.
During the court competition era a small number of courts had judges that were competing to attract debtors to file in their court, which for the rest of the country created plausible exogeneity between the firms choice to forum shop and characteristics of their local county (see Section \ref{sec:ForumShopping} for more details).


\fi
    
    
%%%%%%%%%%% MAIN FINDINGS %%%%%%%%%%% 
To address our question, we construct a novel database 
%that contributes to literature relating to both forum shopping and Chapter 11 bankruptcies in general. Our database
that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (Compustat), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, yearly fixed effects for each of the 94 U.S judicial districts and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
Thus we show it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million worth of employment.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

\textcolor{red}{ROBUSTNESS CHECK STUFF}




%%%%%%%%%%% PUZZLE ON WAGES %%%%%%%%%%% 
Counter-intuitively, we find evidence that Chapter 11 bankruptcy reorganizations of large publicly traded firms are associated with a drop in the county level average wage for the legal sector.
% Counter-intuitively, we find that Chapter 11 bankruptcy reorganizations of publicly traded firms are associated with a 1.5\% drop in the average county wage in the legal sector.
We reconcile this puzzling finding with a \textit{compositional} effect. 
To do this we specialize the canonical model from \citet{Acemoglu_Autor_2011} to the legal labor markets. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and unskilled labor (paralegals, law clerks, etc.).
Skilled workers are more productive but their labor supply is more inelastic than unskilled workers.
In this environment, bankruptcy shocks boost the demand of legal services, prompting an increase in the firm's demand for both types of workers.
Since skilled workers have a relatively inelastic labor supply, bankruptcy shocks shift the composition of legal workers towards unskilled workers, causing a drop in the average wage.


%%%%%%%%%%% MODEL %%%%%%%%%%% 
% Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
% In doing so we contribute to the extensive body of the empirical literature (e.g. \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}) that aims to estimate the elasticity of substitution between high and low skilled labor for CES production functions. 
% We differ from this existing literature by being the first to provide empirical evidence for the elasticity of substitution across skill levels in the context of the legal industry. With this novel setting we not only find evidence that supports previous estimates that skilled and unskilled labor are imperfect substitutes, but we are also able to find point estimates for this parameter.

Finally, we bring theoretical predictions of the model to the data in order to estimate structural parameters. 
In doing so we contribute to the extensive body of the empirical literature that aims to estimate the elasticity of substitution between high and low skilled labor (e.g. \cite{katz_changes_1992}, \cite{bowlus_wages_2017}, \cite{angrist_economic_1995}, \cite{Autor18_lecture}).
Unlike much of this literature we provide empirical evidence for the elasticity of substitution across skill levels at an industry level, and are the first to do so in the context of the legal industry. 
With this novel setting we find additional evidence supporting \citet{blankenau_industry_2011} who predict this elasticity to be higher at the industry level than it is at an aggregate level.  

%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to the literature. 
First, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (\citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06})--by providing first evidence of the unintended consequences on the local economy. Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.

==> Drafts/Old/Intro_Draft_V2.tex <==
Fluctuations in the financial health of major employers play a critical role in the well being of local labor markets.
Much to the detriment of these local economies, when a large corporation files for bankruptcy employment falls (\cite{bernstein_bankruptcy_2019}). 
However, the adverse effects of bankruptcy shocks on overall local employment hides the differential impact across sectors in the local production network (\cite{carvalho_micro_2014}).
%
\textcolor{red}{
In particular, the legal service sector experiences a significant increase in demand from bankruptcy events.
The vast majority of the bankruptcy literature treats
legal expenses as a dead-weight loss from bankruptcies (CITATIONS)\footnote{
    LOTS OF PAPERS MAYBE FOOTNOTE
    },
but they are not. 
They are a meaningful transfers to a crucial stakeholder of bankruptcy events: 
professionals employed in the legal service sector. 
% Bankruptcy events generate significant demand of legal services.
% The vast majority of the bankruptcy literature treats
% Legal expenses as a dead-weight loss from bankruptcies (CITATIONS \footnote{LOTS OF PAPERS MAYBE FOOTNOTE}), but they are not. 
% They are transfers to crucial stakeholders of bankruptcy events: 
% professionals employed in the legal service sector. 
}

We contribute to the literature by studying the effect of these shocks on the local legal service sector,
a sector that directly relates to bankruptcy shocks via a demand channel.
%%%
%Our contribution can be broken into three main parts.
%%%
% At odds with the rest of the local economy, local legal labor markets benefit from the increased demand for legal services, partially offsetting the contractionary effect on the bankrupt firm’s surrounding area.
%%%%% ALTERNATIVE
First, we find evidence that local legal labor markets benefit from the increased demand for legal services created by bankruptcies, partially offsetting the contractionary effect on the bankrupt firm’s surrounding area. 
%First, at odds with the rest of the local economy, we find evidence that local legal labor markets benefit from the increased demand for legal services created by bankruptcies. Importantly, this can partially offset the contractionary effect on the bankrupt firm’s surrounding area. 
Second, we show that lax bankruptcy venue laws and competition among courts may have caused a substantial amount of these potential gains to be exported away from the affected community.
%Finally, to the best of our knowledge, we are the first to structurally estimate a model of the legal sector, and perform counterfactual welfare analysis to quantify losses from firm's who exploit these stipulations of the law to file in a bankruptcy venue that is located far away from their local community.
Finally, we structurally estimate a model of the legal sector, and perform counterfactual analysis to quantify missed welfare gains in the legal sector from firms who forum shop away from their local communities.




The legal industry plays a key role in the functioning of modern economic societies, covering professions in the judiciary system, law enforcement, correction and rehabilitation.
%%%%%%%%%%%%%%%
%Similar in scale to the agricultural sector (280 vs 175 billions, respectively), over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
In 2019 the industry GDP measured 280 billion, notably larger than other highly studied sectors such as the US agricultural sector (175 billion).\footnote{
    Gross Domestic Product: Legal Services (NAICS 5411) and Agriculture, Forestry, Fishing and Hunting (NAICS 11) in the United States.
    \textit{Source:} \href{https://fred.stlouisfed.org/graph/?g=FADm}{Bureau of Economic Analysis (BEA)}.\nocite{FRED_Legal_Ag_GDP}
}
Over the last decade US legal expenses have exceeded \$2 trillion (see also, \cite{bennett_corporate_2018}).\footnote{
    2.380 trillion 2010-2019, 1.299 trillion 2015-2019. \textit{Source:}  \href{https://fred.stlouisfed.org/graph/?g=FADm}{FRED}\nocite{FRED_Legal_Ag_GDP}} 
    % $^,$\footnote{\url{https://fred.stlouisfed.org/series/N4168C0A144NBEA} \textcolor{red}{1.046 trillion from wage and salary accruals from 2010-2019.}} 
%%%%%%%%%%%%%%%    

Using a novel database of Chapter 11 bankruptcies of publicly traded firms, we estimate that during the early 90's bankruptcy reorganizations are associated with a 1\% increase in annual legal employment for the affected county for each ongoing bankruptcy. 
% Aggregated across the U.S. this is roughly 10,000 jobs with wages adding up to nearly \$1 billion in 2021 dollars \textit{each year}. 
Aggregated across the U.S. this means that each year roughly 10,000 jobs-- with wages adding up to nearly \$1 billion in 2021 dollars-- are being distributed to communities dealing with the contractionary effects associated with a major employer filing for bankruptcy. 
For a large city such as Los Angeles this is more than 4,000 jobs each year-- an even larger source of employment than the Amazon HQ2 that cities offered hundreds of millions in incentives to attract.\footnote{
    As of September 1, 2021 there were roughly 3000 employees assigned to HQ2. \textit{Source:} \href{https://www.aboutamazon.com/news/amazon-offices/the-next-chapter-for-hq2-sustainable-buildings-surrounded-by-nature}{Amazon}. 
    Notably Montgomery County, Md. offered \$8.5 billion in incentives to attract Amazon's new HQ2. \textit{Source:} \href{https://www.brookings.edu/research/five-economic-development-takeaways-from-the-amazon-hq2-bids/}{Brookings.edu}}
% However, it's possible that lax bankruptcy venue statutes and competition among judges to attract firms to file in their court, instead of the court in their local area, may have caused a considerable amount of these potential gains to be squandered. 
Our results also show that these gains are lost when firms file for bankruptcy in courts that are far away from their headquarters, a phenomenon referred to as \textit{forum shopping}.
We find evidence that forum shopping \textit{exported away} more than 24\% of the potential employment gains from local communities with distressed firms each year during the Court Competition Era (1991-1996).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ORIGINAL- CH11 br are big %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We measure the demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms. Chapter 11 bankruptcy cases for large firms are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
% Accordingly, firms will often pay fees in the order of hundreds of millions of dollars\footnote{ 
%     The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.}$^,$\footnote{
%     For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.
%     } 
% for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
%     For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
% This acts as a considerable demand shock\footnote{``In addition to reporting and oversight costs, Chapter 11 bankruptcies have been notoriously expensive because procedural requirements demand substantial attorney work...'' \textit{Source:} \href{https://www.schwabe.com/newsroom-publications-chapter-11-bankruptcy-is-expensive-the-small-business-reorganization-act-provides-a-realistic-opportunity}{Schwabe} \nocite{schwabe_Ch11_Expensive}
% } to a critical industry.
%% 
            % \marginpar{\scriptsize\textcolor{red}{ARGUE IN TWO STEPS- CHAPTER 11 are: \\1. large bankruptcies (ORGANIZE POINTS BEFORE);  \\2. provide a feature that we leverage for identification: forum shoppping. (THE LATTER WILL CONNECT WELL WITH THE NEXT PARAGRAPH)}}   
            

We measure the demand shocks to local legal services using Chapter 11 reorganization bankruptcies of publicly traded firms for two main reasons. 
First, Chapter 11 bankruptcies act as a considerable demand shock to legal services.
These bankruptcy cases are complex phenomena that arbitrate over the conflicting interests of several stakeholders: creditors, shareholders, workers, managers, and so forth. 
Consequently, firms will often pay fees in the order of hundreds of millions of dollars\footnote{
    For instance, the professional fees in Kodak bankruptcy case rounded up to \$240M in 2013. \textit{Source}: \href{https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114}{Reuters} \nocite{brown_kodak_2013}.  
    The average professional fees amount to \$82 million in 2021 dollars; computed using the \LPlong, 1980-2014.
    } 
for legal teams that range from a handful of highly trained consultants and attorneys, to teams of legal clerks and paralegals.\footnote{
    For the legal industry specifically \citet{freedman_how_2005} estimates that it takes upwards of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size.}
The second reason is that stipulations of the Chapter 11 U.S. bankruptcy statutes provide a feature that we leverage for identification- forum shopping.

Identifying the causal impact of bankruptcy shocks on local legal sector labor markets is not straightforward.
Unlike much of the applied economics literature that exploits an event study framework, our setting is not conducive to such methods due to transitory and repeated treatment (\cite{callaway_difference--differences_2020}, \cite{sun_estimating_2020}). 
Counties experiencing treatment (Chapter 11 bankruptcy shocks) are often treated multiple times, can switch back and forth between treated and untreated from year to year, and do not share a clear pre-treatment and post-treatment period. 
We contribute to the previous literature (e.g. \citealp{bernstein_bankruptcy_2019}; \citealp{chava2021community}) by proposing an alternative identification strategy that handles the complex nature of our treatment.
We adopt an economic history approach and focus our analysis on a historical period where we can leverage institutional changes---in Chapter 11 proceedings---to obtain clearer identification (e.g. \citealp{rajan_anatomy_2015}, \citealp{hausman_fiscal_2016}, \citealp{hilt_turning_2016}, \citealp{cunningham_decriminalizing_2014}).\footnote{
    For example, \cite{cunningham_decriminalizing_2014} uses an institutional change where a Rhode Island judge unexpectedly decriminalized indoor prostitution to create exogenous variation in the availability and legality of sex services. As such they restrict their attention to the period from 2004 to 2009 when this institutional change was in effect.}
        
        
The historical period we focus 
on is called the `Court Competition Era' (Section \ref{sec:ForumShopping}). This is a period from 1991 to 1997 when bankruptcy judges began competing for prestigious and lucrative Chapter 11 filings (e.g. \citealp{lopucki_courting_2005}, \citealp{Lopucki06}, \citealp{LopuckiKalin00}, \citealp{EisenbergLopucki1999}, \citealp{Cole03}). 
Competition among bankruptcy judges, encouraged firms to exploit stipulations of the US corporate bankruptcy law to file for Chapter 11 bankruptcy reorganization far away from their headquarters, i.e. forum shopping.\footnote{
    In our context we only consider district level forum shopping. It is important to note that Lopucki also considers within district forum shopping. However this applies to only a handful of cases. We choose to do this because we are interested in local effects, and in some cases firms filed in the same city but in a different court and were considered as forum shopping.
    } 
%This phenomena of firms filing in a forum different from their local court is referred to as `forum shopping' 
%%%%%%%%%%%
During this short time period, the share of forum shopped bankruptcy cases  tripled (Figure \ref{BR_FS_RATIO80_07}), from 20\% in 1990 to a new long run average of 60\%, which persists until today (\citealp{ellias_bankruptcy_2019}).\footnote{
    \cite{ellias_bankruptcy_2019} finds that in recent years more than 60\% of large firms still choose to file in the same magnet districts: Southern District of New York and District of Delaware.  
    }
    
    
Our identification strategy focuses on this period of abrupt change in bankruptcy filing practices to create exogenous variations in the location of demand for legal service from Chapter 11 bankruptcies.
% \textcolor{red}{Although it is well established that the strategic bankruptcy plan is drafted by a handful of highly specialized law companies (mostly located in New York), the material handling of Chapter 11 bankruptcy requires hiring a lot of unskilled, etc.\\
% WE ESTIMATE THAT 20\% of the jobs LOST TO DELAWARE AND NEW YORK. 
% }
% \\
These demand shocks occur where the bankruptcy court is located because legal services involved must be certified to practice in that area, familiar with local bankruptcy practices, and able to attend proceedings and file paperwork at the courthouse.
Thus, when a firm forum shops, the legal sector demand shock is effectively exported away from their local economy.
This transfer in potential legal service demand is particularly pronounced because firms typically forum shop considerable distances away from their local area. 
For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 766.1 miles. 
% By comparison, this is a drastic increase from an average distance of only 18.9 miles for the firms who did not forum shop.\footnote{
    % Figures calculated using the \LPlong.}
This is a drastic increase from 18.9 miles for firms who did not forum shop.\footnote{
    Figures calculated using the \LPlong.}
    
    
A key identification assumption is that
Chapter 11 bankruptcy filings of publicly traded firms are a source of plausibly exogenous variation in the local demand for legal services.
The large/multi-national nature of the demand faced by publicly-traded firms bolsters the plausible exogeneity of these bankruptcy shocks by decoupling the determinants of firms' bankruptcy choices from the well being of the local economy.
To illustrate this point anecdotally, consider the Chapter 11 bankruptcy of Kodak, the well-known photography company from Rochester, New York. 
Economic fluctuations in Rochester played little to no role in Kodak's decision to file for bankruptcy reorganization in 2012---which was instead motivated by the worldwide decline in the popularity of film photography. We also demonstrate this exogeneity empirically in Section \ref{sec:BR_LocalConditions}.
% In addition, we test this claim empirically in Section \ref{sec:BR_LocalConditions}.  
% In addition, Section \ref{sec:BR_LocalConditions} demonstrates this exogeneity empirically. 


%\textcolor{red}{***Also note that for our purposes, it is unimportant \textit{why} firms forum shop; rather, our identification simply requires the forum shopping reason to be independent from the local economy.***}

To address our question, 
For our analysis,
we construct a novel database that expands the universe of large bankruptcies in the widely used \LPlong \space (Lopucki BRD) with bankruptcy information of publicly traded firms in Standard and Poor's Compustat Database (CS), supplemented with information from court filing records in \PACER.\footnote{
        Web BRD (the ‘‘LoPucki’’) database can be found at        \url{http://lopucki.law.ucla.edu}. Professor Lopucki has been at the forefront of research into large chapter 11 bankruptcy cases over the last 30 years. As such, the Lopucki BRD has been the gold standard for researchers studying large corporate bankruptcies and has been used in over 200 publications since it's creation. This database consists of firm level data with approximately 1000 observations of large public companies that filed for Chapter 11 bankruptcy in the United States between 1979 and 2014. Firms qualify as large public companies only if they file a 10-K form with the SEC that reports assets worth at least \$100 million in 1980 dollars (about \$300 million in current dollars).} 
After aggregating this information at the county level, 
%employ this database---with 15,931 county-year observations that have non-zero legal employment---to 
we estimate a regression with county level fixed effects, yearly fixed effects for each of the 94 U.S judicial districts and county-year controls. % to capture trends over time across each district.

We estimate that each firm that files for Chapter 11 bankruptcy is associated with a 1\% increase in annual legal employment for the affected county for each year of the bankruptcy. 
Importantly, including the channel of forum shopping confirms our results. We document that observed changes in employment and wages for the local areas legal sector are contingent on firms filing for bankruptcy in their local court. When firms choose to file in a court that is far from their local area (i.e. forum shop) any impact on the legal sector is essentially exported away. 
This indicates that it is the actual filing of the bankruptcy that is important, and not just a confounding factor of the bankruptcy causing our observed results. 
Our results suggest that when a firm chooses to forum shop the local area loses approximately \$9.6 million worth of employment.\footnote{
    Using \$4 million each year stat, average length of bankruptcy in our sample was 2.4 years according to \LPlong.}

These results are stable to a variety of robustness checks. Most notably, to ease concerns about the relevance of the comparison group we limit our sample to only counties that could plausibly be treated. 
We also run various specifications that show potential spillover effects to neighboring counties is negligible. 
Additionally we find our results are robust to several other considerations such as: using alternative data sources or alternative measures of treatment, including additional county characteristic controls, and dropping years potentially impacted by recessions. 




% Motivated by the evidence from the reduced form results we construct a parsimonious model, similar to \citet{notowidigdo_incidence_2020}, that captures the dynamics of how legal sector labor markets respond to a demand shock. 
Motivated by the evidence from the reduced form results we construct a parsimonious model that captures the dynamics of how legal sector labor markets respond to a demand shock. 
We explicitly model local labor demand in a similar manner to the spatial equilibrium model in \citet{notowidigdo_incidence_2020}. 
In the model economy, a representative firm produces legal services using two inputs of production that act as imperfect substitutes: skilled labor (attorneys) and less productive unskilled labor (paralegals, law clerks, etc.).
Following works such as \citet{notowidigdo_incidence_2020} and \citet{bai_demand_2011}, demand shocks enter this model akin to ``productivity'' shocks. 
This model is a unique specialization of a canonical labor model used for studying how shocks effect labor market outcomes across skill levels (\cite{acemoglu_technical_2002}; \cite{Acemoglu_Autor_2011}; \cite{bowlus_wages_2017}). 


We calibrate the model parameters using a nonlinear simultaneous-equations generalized method of moments (GMM) procedure that exploits non-forum shopped bankruptcies as exogenous demand shocks for the local area.
In doing so we contribute to the extensive body of literature that estimates the Frisch elasticity of labor supply for the extensive margin (e.g. \cite{bianchi_icelands_2001}; \cite{brown_link_2013}; \cite{rogerson_micro_2009}).
Unlike much of this literature we provide empirical evidence for the elasticity of labor supply at the industry level and are the first to do so in the context of the legal industry.
Of particular interest, we find evidence that this elasticity of labor supply is greater for unskilled labor than for skilled labor.  


 

Our calibrated model allows us to to quantitatively estimate the welfare implications of forum shopping. 
% To do so we calculate the consumption equivalent variation between the observed state of the world with forum shopping, and the counterfactual regime where all bankruptcies were filed locally. 
To do so we calculate the potential welfare gains associated with moving from the status-quo regime where firms forum shop to a counterfactual regime without forum shopping.
We find that workers would need roughly a 1\% increase in there annual consumption to receive the same level of utility they would have without forum shopping. 

While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will strengthen Chapter 11 bankruptcy venue laws and prevent firms from filing far from where they are located, likely putting a halt to the practice of forum shopping. 
If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business.
The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community\footnote{
    See press release  \textit{Lofgren, Buck Introduce Bipartisan Legislation to End Corporate Bankruptcy Forum Shopping}, from Rep. Lofgren. 
    \textit{Source:} \href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}
    }
    % (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
    City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}.}
Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate.

% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate. 

% \textcolor{red}{While these estimates are relevant on their own, the recently proposed Bankruptcy Venue Reform Act gives them direct relevance to ongoing policy debate in the U.S. Congress.
% On June 28, 2021 the U.S. Representatives Zoe Lofgren and Ken Buck introduced the bipartisan Bankruptcy Venue Reform Act to the U.S. House of Representatives.
% If passed, the Reform Act will put a halt to the practice of forum shopping, the ability of firms to file for a bankruptcy court located in a different place than the principal assets or place of business. The purpose of the bill is to protect the interests of affected stakeholders (local creditors, retirees and employees) by having the case processed by a judge familiar with the community (\href{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}{Link}),
% and put to an end ``the single most significant source of injustice in chapter 11 bankruptcy cases''.\footnote{
%     City of Detroit’s Bankruptcy Judge Steven Rhodes, \textit{National Conference of Bankruptcy Judges}, 2018. \textit{Source:} \href{https://cdn.ymaws.com/www.ncbj.org/resource/resmgr/docs_public/Venue_White_Paper_-_Final.pdf}{Link}. MAYBE PUT THIS IN THE CONCLUSION}
% Our analysis suggests that a deeper look at the production network of large corporate bankruptcy cases uncovers economically significant costs to local communities, so far unaccounted for by the policy debate. }



%%%%%%%%%%% INCIDENTAL CONTRIBUTIONS %%%%%%%%%%% 
By considering the channel of forum shopping we also make several incidental contributions to the literature. 
First, we contribute to the heated debate over the efficiency of forum shopping and court competition for bankruptcy outcomes (e.g. \citealp{Zywicki06},  \citealp{ThomasRasmussen01}, \citealp{EisenbergLopucki1999}, \citealp{LopuckiKalin00}, \citealp{Lopucki06} \citealp{lee_delawares_2011})--by providing first evidence of the unintended consequences on the local economy. Furthermore, to the best of our knowledge this is the first paper to consider the channel of forum shopping when studying corporate bankruptcy in a general equilibrium setting.

==> Drafts/Old/Introduction.tex <==
Local labor markets depend on the health of their major employers. We can expect local employment to fall when a large employer files for bankruptcy\footnote{For example; \citet{bernstein_bankruptcy_2019}}. This prediction however hides complex adjustments to the local labor market. 
\begin{itemize}
    \item \textit{We use the stipulation of the law to understand the positive economic impact of plausibly exogenous bankruptcy shocks on the firm's local labor market for the legal sector.} \\
    \textbf{OR}
    \item ***\textit{In contrast to the recessionary(contractionary?) effects on the local economy that are typically associated with a large firm filing for Ch11 BR, we show that the labor market for the legal industry acts as a potential channel for economic gains in the bankrupt firm's local area. In addition, we find that this positive impact is dependent on filing locally. Our findings suggest that firms who choose to file away from their local area essentially export these potential gains away}. \\
    \textbf{OR}
    \item \textit{In contrast to the expected recessionary(contractionary?) impact on local economies from large firm's Ch11 BR, we show that the labor market for the legal industry acts as a potential channel for economic gains in the bankrupt firm's local area. In addition, we find that this positive impact is dependent on which court the firm chooses to file with. Our findings suggest that firms who choose to `forum shop', i.e. file away from their local area, are essentially exporting these potential gains away.}
\end{itemize}




% We study the labor market for the legal industry as a potential channel for economic gains to the local area where a large corporation files for chapter 11 BR. 
% Using the stipulation of the law, we show the labor market for the legal industry is a potential channel for economic gains to the local area where a large corporation files for chapter 11 BR.
% Using the stipulation of the law, we show the labor market for the legal industry is a potential channel for economic gains to the local area where a large corporation files for chapter 11 BR, despite the recessionary effects typically associated with these bankruptcies. 
% Using the stipulation of the law, we show the labor market for the legal industry is a potential channel for economic gains to the local area where a large corporation files for chapter 11 BR, in contrast to the recessionary effects typically associated with these bankruptcy shocks. 
% We show the labor market for the legal industry is a potential channel for economic gains to the local area where a large corporation files for chapter 11 BR, in contrast to the recessionary effects typically associated with these bankruptcy shocks. Using the stipulation of the law, we find that this positive impact is dependent on filing locally. Firms who choose to file away from their local area essentially export these gains away from their local economy.  

%In contrast to the recessionary/contractionary effects typically associated with bankruptcy shocks, we show the labor market for the legal industry is a potential channel for economic gains to the local area around a large corporation undergoing chapter 11 BR. In addition, we find that this positive impact is dependent on filing locally. Evidence suggests that firms who choose to file away from their local area essentially export these potential gains away from their local economy. 

% In contrast to the expected recessionary(contractionary?) impact on local economies from large firm's Ch11 BR, we show that the labor market for the legal industry acts as a potential channel for economic gains in the bankrupt firm's local area. In addition, we find that this positive impact is dependent on which court the firm chooses to file with. Our findings suggest that firms who choose to `forum shop', i.e. file away from their local area, are essentially exporting these potential gains away.

 
A large corporation filing for Chapter 11 bankruptcy is an extremely complex legal process, often with hundreds of millions of dollars of assets at stake. As such, the firm will demand a considerable amount of legal services. Which in turn will cause an increase in demand for labor in the legal sector. For such a complex and high stakes process, naturally the firm will require legal counsel from bankruptcy experts to help navigate the firm through the bankruptcy proceedings. However, this boost in labor demand is not limited to legal experts and lawyers. In addition to these highly skilled experts, the firm will also require a substantial number of less skilled workers to deal with the sizable amount of clerical and bureaucratic work generated by the bankruptcy proceedings.

When the firm files for bankruptcy locally, this stimulus to the legal sector's labor market can help to partially offset reductions in economic activity the area may experience due to the financial distress of a major employer. However, when the firm chooses to file in a forum besides their local bankruptcy court this stimulus is effectively exported away.  

Filing in a forum different from the local court is referred to as `forum shopping'. In the U.S. the headquarters of any given firm are located in one of 91 judicial districts, each with their own bankruptcy court. When a firm forum shops they are using legal workarounds to file in a bankruptcy court that is located in a different district than where the actual headquarters of the firm is located. For large publicly traded corporations who forum shop the average distance from their headquarters to the court they filed in is 749.7 miles. A drastic increase from an average distance of only 8.7 miles for the firms who did not forum shop\footnote{
    Figures calculated using the Lopucki BRD}. 
    
There is a considerable body of literature from legal academics and professionals (as well as some rather heated debate) on the topic of corporate bankruptcy law and forum shopping. The primary focus of this literature looks at the implication of forum shopping on bankruptcy outcomes for the firm and it's creditors
(e.g. \cite{EisenbergLopucki1999}; \cite{Zywicki06}; \cite{ThomasRasmussen01}; \cite{LopuckiKalin00}; \cite{Baird97}). 
Our focus differs from this literature. 
Rather than focusing on the bankruptcy outcomes for the creditors and debtors involved, we explore the general equilibrium implications of bankruptcies and forum shopping for the firm's local area.

This paper uses the era of peak court competition (1991-1997) to study the effect of large firm bankruptcy shocks on \textit{local} labor market outcomes in the legal sector. Using U.S. county year panel data we show that when the firm files locally these bankruptcy shocks have a significant and positive impact on the employment level in the legal sector. These findings are consistent with the expected labor demand shock. Accounting for the channel of forum shopping allows us to better understand how the pattern of legal employment responds to these bankruptcies. We find that the impact of these shocks completely disappears when the firm engages in forum shopping and chooses not to file locally. Indicating that the filing location plays a critical role in changes in the pattern of legal employment. 

\noindent ADD PARAGRAPH ABOUT ROBUSTNESS/EXOGENEITY STUFF HERE?

To conduct this empirical analysis we contribute a unique database that builds off of the firm level data from the UCLA-LoPucki Bankruptcy Research Database (BRD). We expand the universe of the Lopucki BRD by including additional firms found in the Standard and Poor's Compustat Database. Our contribution is the scraping of publicly available court records and SEC filings to collect data on bankruptcies for these firms\footnote{
    We use a variety of sources for our data collection including SEC filings available via the \citet{sec.gov} website, and court records from the PACER Case Locator and the individual court websites.}. \footnote{SHOULD THIS PARAGRAPH BE DELETED/MOVED?}

In addition to an increase in the level of employment, standard economic theory would suggest that in response to increased labor demand there would be an increase in wages. However, we find a counter intuitive effect on average wages. We find empirical evidence that average wages will actually \textit{decrease} in response to these demand shocks. Though initially puzzling, these findings are consistent with a differential impact on skilled vs unskilled labor predicted by our theoretical model.

The intuition behind this effect is as follows. For the bulk of the legal services required in response to a bankruptcy shock skilled and unskilled labor can be considered imperfect substitutes. Even though skilled labor is more productive, the supply of this labor is relatively inelastic. Thus, the legal sector will hire more relatively more unskilled workers, decreasing the factor intensity of skilled labor. Because unskilled labor is paid a lower wage, the average wage for the industry as a whole will decrease even though the wages for skilled and unskilled labor separately may have increased. 

The framework for our theoretical model follows in the spirit of what \citet{Acemoglu_Autor_2011} refers to as the `canonical model' for analyzing changes in wage structure. This canonical model has been enormously popular for studying the dynamics of how supply and demand factors have influenced the relative wages of skilled and unskilled labor. Where it has gained substantial prominence in the literature studying and estimating determinants of observed labor market outcomes such as increased wage inequality and stagnated average wages\footnote{see \cite{bowlus_wages_2017} ("A simple supply-demand framework has formed the basis of a large body of research on the determinants of wages and employment in the post-war US economy")}. Most notably in the body of research on determinants such as technological change (e.g. \cite{katz_changes_1992}; \cite{acemoglu_technical_2002}) or changes in availability of education (e.g. \cite{abbott_education_2018}; \cite{heckman_general-equilibrium_1998}). Similar to much of this literature (\cite{acemoglu_technical_2002}; \cite{Acemoglu_Autor_2011}; \cite{bowlus_wages_2017}) we use a constant elasticity of substitution production function (CES) with two differentiated inputs, skilled and unskilled labor, to derive an expression for average wages.

The assumption that the elasticity of supply for unskilled is greater than the elasticity of supply for skilled workers is intuitive and easily justifiable. Given the contemporaneous nature of the shock, as well as the high cost in both time and money of law school, it is easy to rationalize that the supply of lawyers would much less elastic than their counterparts such as law clerks, and paralegals which require a relatively much lower investment cost in training, specialization, and education. For the legal industry specifically \citet{freedman_how_2005} estimates that it takes an average of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size and requires more elaborate network of various management, HR, IT, and other administrative employees. In addition \citet{mcclelland_review_2012}, a recent study conducted by the United States Congressional Budget Office, finds empirical evidence that the elasticity of labor supply is decreasing with respect to income level. Indicating that the relatively higher paid skilled labor would be less elastic even without considering the additional costs of education or the traditional composition of employment in a law firm. \footnote{DELETE THIS PARAGRAPH??? REWRITE/SHORTEN}

This paper proceeds in the following manner. Section II provides a brief overview of the forum shopping debate and the court competition era. Section III presents our theoretical model and derives predictions for the compositional effect of the shock. Section IV lays out our proposed mechanism in more detail. Section V describes our database and empirical methodology. Section VI presents our main results. 

NEED TO ADD\begin{itemize}
    \item GE BANKRUPTCY LIT
    \item LABOR DEMAND SHOCK LIT
    \item STRUCTURAL ESTIMATION OF PARAMETERS
\end{itemize}
































% Local labor markets depend on the health of their major employers. We can expect local employment to fall when a large employer files for bankruptcy. This prediction however hides complex adjustments to the local labor market. We use the stipulation of the law to understand the positive economic impact of plausibly exogenous bankruptcy shocks on the firm's local labor market by looking at the market for legal employment.

% The particular stipulation of interest to our analysis is a legal phenomena known as `forum shopping'. Forum shopping refers to the act of seeking out the most advantageous venue in which to settle a legal dispute\footnote{see \cite{Algero99} ("'Forum shopping' typically refers to the act of seeking the most advantageous venue in which to try a case.")}. In the context of corporate bankruptcies this means that the firm (debtor) is using legal workarounds to file in a bankruptcy court that is located in a different district than where the actual headquarters of the firm is located in an attempt to gain some sort of more desirable outcome. 

% There is a considerable body of literature from legal academics and professionals (as well as some rather heated debate) on the topic of corporate bankruptcy law and forum shopping. The primary focus of this literature looks at the implication of forum shopping on bankruptcy outcomes for the firm and it's creditors
% (e.g. \cite{EisenbergLopucki1999}; \cite{Zywicki06}; \cite{ThomasRasmussen01}; \cite{LopuckiKalin00}; \cite{Baird97}).
% Our focus differs from this literature. We explore the general equilibrium implications of forum shopping on local employment outcomes in the legal sector.

% We construct a database for empirical analysis that builds off of the firm level data from the UCLA-LoPucki Bankruptcy Research Database. We do this by including firms from the Standard and Poor's Compustat Database. We provide a unique contribution to these existing data sets by also collecting bankruptcy data for the Compustat firms
% \footnote{We use a variety of sources for our data collection including SEC filings available via the \citet{sec.gov} website as well as Bloomberglaw.com}.  

% In the spirit of \citet{EisenbergLopucki1999} and \citet{LopuckiKalin00} we focus our attention on the "court competition era" of forum shopping from 1991 through 1996. We document a positive and significant increase of employment in the local legal sector when a firm files for Chapter 11 bankruptcy. Without controlling for the possibility of forum shopping we estimate a Chapter 11 bankruptcy filing to be associated with an increase in legal employment of about .7\% per firm filing for that particular county. The estimate of this effect increases to nearly a 1\% when forum shopping is controlled for. However, our results also show that when the firm files in a district besides their local district (forum shops) any positive effect is entirely lost. These findings suggest that in this period of heightened competition between bankruptcy courts to attract debtors, forum shopping was essentially exporting jobs and potential gains away from the firm's local labor market.  

% In addition to these results on the level of employment we also find a puzzling effect on wages. Standard economic theory would suggest that the increase in demand for legal services from a bankruptcy shock would result in an increase in the wage for workers in the legal sector. Surprisingly, we find evidence for the exact opposite. We show a large corporate bankruptcy appears to be associated with a \textit{decrease} in the average wage for workers in the legal sector. 

% We propose a theoretical framework to rationalise these findings as the result of the compositional channel effect of bankruptcy on legal employment. To do this we propose a theory of skilled and unskilled labor in the production of legal services. Where in this context skilled labor refers to legal experts such as lawyers, and unskilled labor refers to employees which have a much lower educational barrier for employment such as paralegals or law clerks. We find that our empirical results are consistent with differential elasticity of substitution between skilled and unskilled labor\footnote{In particular the difference between skilled and unskilled labor's Frisch elasticity of labor supply}. The framework we use follows in the spirit of what \citet{Acemoglu_Autor_2011} refers to as the "canonical model" for analyzing changes in wage structure. 

% Using this simple framework we derive two key predictions for the effect of a bankruptcy shock on the composition of the labor market in the legal sector. First we show that the level of employment increases relatively more for unskilled than skilled workers, given that the supply of unskilled labor is relatively more elastic. Second, as a result of this change in the relative factor intensity, average wage will decrease.

% This canonical model has been enormously popular for studying the dynamics of how supply and demand factors have influenced the relative wages of skilled and unskilled labor. Where it has gained substantial prominence in the literature studying and estimating determinants of observed labor market outcomes such as increased wage inequality and stagnated average wages\footnote{see \cite{bowlus_wages_2017} ("A simple supply-demand framework has formed the basis of a large body of research on the determinants of wages and employment in the post-war US economy")}. 
% Most notably in the body of research on determinants such as technological change (e.g. \cite{katz_changes_1992}; \cite{acemoglu_technical_2002}) or changes in availability of education (e.g. \cite{abbott_education_2018}; \cite{heckman_general-equilibrium_1998}). Similar to much of this literature (\cite{acemoglu_technical_2002}; \cite{Acemoglu_Autor_2011}; \cite{bowlus_wages_2017}) we use a constant elasticity of substitution production function (CES) with two differentiated inputs, skilled and unskilled labor, to derive an expression for average wages.

% The assumption that the elasticity of supply for unskilled is greater than the elasticity of supply for skilled workers is intuitive and easily justifiable. Given the contemporaneous nature of the shock, as well as the high cost in both time and money of law school, it is easy to rationalize that the supply of lawyers would much less elastic than their counterparts such as law clerks, and paralegals which require a relatively much lower investment cost in training, specialization, and education. For the legal industry specifically \citet{freedman_how_2005} estimates that it takes an average of 1.3 non-lawyer employees for each lawyer in a law firm. As well as indicating that this could increase as a firm grows in size and requires more elaborate network of various management, HR, IT, and other administrative employees. In addition \citet{mcclelland_review_2012}, a recent study conducted by the United States Congressional Budget Office, finds empirical evidence that the elasticity of labor supply is decreasing with respect to income level. Indicating that the relatively higher paid skilled labor would be less elastic even without considering the additional costs of education or the traditional composition of employment in a law firm. 

% This paper proceeds in the following manner. Section II provides a brief overview of the forum shopping debate and the court competition era. Section III presents our theoretical model.  

==> Drafts/Old/Model_9_1_2021.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                   THEORETICAL MODEL

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Environment}
We consider a dynamic partial equilibrium model of the legal sector. The economy is populated by a mass of heterogeneous households and a representative firm that produces legal services. Households differ in their labor productivity: skilled and unskilled. Skilled workers can be thought of as lawyers, who require an extremely large investment in training before they can work. Whereas unskilled workers can be thought of as para-legals, law clerks, and legal sector employees who require considerably less upfront costs in training relative to skilled workers.  The representative firm hires skilled and unskilled workers to produce legal services (the numeraire). The demand of legal services is exogenous. Labor markets are competitive.


% %%%% CHAD 
% In this section we use the canonical model for analyzing the compositional effects of supply and demand factors on relative wages of heterogeneous labor inputs. Our contribution here is two-fold. First, we specialize this canonical setup to explain the differential impact of a bankruptcy shock for skilled and unskilled labor in the legal sector. Additionally, we incorporate the channel of forum shopping to general equilibrium analysis of bankruptcy shocks.   

% In our context, skilled labor can be thought of as workers such as lawyers, who require an extremely large investment in training before they can work. Whereas unskilled labor is analogous to the legal sector employees who require considerably less upfront costs in training relative to skilled workers, such as para-legals, law clerks, and so on.  

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsubsection{Households}
    The economy is populated by heterogeneous households that differ in the type ($j$) of labor supplied: skilled ($j=s$) and unskilled ($j=u$).
    In each period $t$, households of type $j$ choose consumption $\cjt\in\mathbb{R}_{+}$ and labor hours $\njt\in\mathbb{R}_{+}$
    in order to maximize Greenwood–Hercowitz–Huffman preferences.\footnote{
         As such, the marginal rate of substitution between labor and consumption will only depend on labor. See \citet{GHH_Preferences_1988} p. 404.} 
%  \begin{equation}\label{Utility}
%       \underset{c_{j},j}{\max} \frac{1}{1-\sigma}\left(c_{j} - \gamma \frac{j^{1+\rho_{j}}}{1 + \rho_{j}}\right)^{1-\sigma}
%         \end{equation}

\begin{equation}\label{Utility}
\begin{split}
       \underset{\{\cjt,\njt\}^{\infty}_{t=0}}{\max}\quad & \sum_{t=0}^{\infty}\beta^{t}\frac{1}{1-\sigma}\left(\cjt - \gamma \frac{n_{j,t}^{1+\rho_{j}}}{1 + \rho_{j}}\right)^{1-\sigma}\\
       &\text{s.t.}\; \cjt \leq \wjt \njt
\end{split}
\end{equation}        
   % over consumption $c\in\mathbb{R}_{+}$ and labor $j\in\{s,u\}$, 
    In this setting, $\rho_{j}>0$ determines type $j$'s Frisch elasticity of labor supply, and the terms $\sigma > 0$ and $\gamma > 0$ are shaping parameters.   
 For each hour of work supplied workers of type $j$ receive an hourly wage $\wjt$. The wage compensation is their only source of income.
 Note that because there is no savings, and the objective function is unchanged across periods we can suppress the period index $t$ for brevity. 
    % %%%%%%%%%%%%%%%%%%%%%%%%
    % Households have  Greenwood–Hercowitz–Huffman preferences\footnote{
    %     As such, the marginal rate of substitution between labor and consumption will only depend on labor. See \cite{GHH_Preferences_1988} (p. 404)} 
    %     % The economy is populated by skilled and unskilled workers.
    %     % The economy is populated by two different kinds of households; those that supply skilled labor, and those that supply unskilled labor. 
    %     % The economy is populated by heterogeneous households. Households are differentiated into skilled and unskilled workers. 
    %     %We consider two kinds of households supplying skilled labor (\s) and unskilled labor (u). 
    %     %Households have  Greenwood–Hercowitz–Huffman preferences over consumption and labor
    %     % The household's utility function is increasing in consumption ($c$) and decreasing in labor ($s,u$) in the form of Greenwood–Hercowitz–Huffman preferences. 
    %     %Let $j={s,u}$ denote labor for skilled and unskilled workers respectively:
    %     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %     % \begin{equation*}
    %     %     U(c, G(j)) = U(c - G(j))
    %     % \end{equation*}
    %     % over consumption $c\in\mathbb{R}_{+}$ and labor $j\in\{s,u\}$, with $s,u\in\mathbb{R}_{+}$, and
    %     % where $G(j)$ models the disutility from labor. As such, the marginal rate of substitution between labor and consumption will only depend on labor.\footnote{see \cite{GHH_Preferences_1988} (p. 404)} In accordance with these preferences, utility for worker of type $j={s,u}$ takes the following functional form: 
    %     % %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %     \begin{equation}\label{Utility}
    %         U_{j}(c_{j},j) = \frac{1}{1-\sigma}\left(c_{j} - \gamma \frac{j^{1+\rho_{j}}}{1 + \rho_{j}}\right)^{1-\sigma}
    %     \end{equation}
    % over consumption $c\in\mathbb{R}_{+}$ and labor $j\in\{s,u\}$, with $s,u\in\mathbb{R}_{+}$,
    %      where $\rho_{j}>0$ determines type $j$'s Frisch elasticity of labor supply, and the terms $\sigma > 0$ and $\gamma > 0$ are shaping parameters.   
    %     As usual, households solve the following problem:
        
    %     \begin{center}
    %         $\underset{c_{j},j}{\max} \;\; U_{j}(c_{j}, j)
    %         \;\;\;\;\;\;\;\;\;\;\;\;\;\;\; 
    %         \text{s.t.} \;\;\; c_j\leq w_{j} j $
    %     \end{center}
    %     %%%%%%%%%%%%%%%%%%%%%%%%
        
        \noindent From the FOC, we obtain the labor supply functions:
        \begin{multicols}{2}
        \begin{equation*}
            \s(w_s) = \left(\frac{w_{s}}{\gamma}\right)^{\frac{1}{\rho_{s}}}
        \end{equation*}
        
        \begin{equation*}
            \u(w_u) = \left(\frac{w_{u}}{\gamma}\right)^{\frac{1}{\rho_{u}}}
        \end{equation*}
        \end{multicols}
       % As usual the key insight with Greenwood–Hercowitz–Huffman preferences is that the optimal decision to supply labor depends only on $G(j)$. Clearly, $s'(w_{s}) >0$ and $u'(w_{u}) >0$ thus there is no wealth effect on labor supply. (DOUBLE CHECK THIS CHAD)
        \noindent It follows that the Frisch Elasticity of Labor Supply ($\epsilon_j$) for $j = \{s,u\}$ can be expressed as:
        \begin{equation}
            \epsilon_j = \frac{1}{\rho_{j}} 
        \end{equation}
        Grounded on the vast empirical evidence for the relative elasticity of labor supply of skilled versus unskilled workers we make the following assumption.
        
        \begin{assumption}\label{elasticity}
        The elasticity of labor supply of skilled workers is lower than unskilled workers,
        %Elasticity of Skilled Labor Supply $<$ Elasticity of Unskilled Labor Supply \\
        i.e. $\rho_u < \rho_s$
        \end{assumption}
        %Assumption \ref{elasticity} is grounded on a vast empirical evidence (CITATON) that suggests that the labor supply of skilled workers is less elastic than their unskilled counterparts. 
%        Intuitively, the supply of skilled labor should be highly inelastic given the lengthy, expensive, and arduous nature of law school. 
        %LAWYER vs CLERKS


        % Assumption \ref{elasticity} is crucial for our results, but is hardly controversial. (
        % Intuitively, the labor supply of skilled labor is going to be relatively less elastic than their unskilled counterparts. The high level of investment costs required to change the supply of workers skilled workers such as lawyers will keep the supply relatively stable in the face of shifting market forces. 
        
%$MRT$
% Extensive Margin Interpretatiom.
% \[H = \int_{M} j dj \]
% Production possibility frontier (for workers)
% 1 Household l
% Takes workers -> Skilled and unskilled
% L -> H(L) = [S^{} + U]^{}




        
        

         
        
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsubsection{Firms}
    A profit-maximizing representative firm %(the legal industry) 
    hires skilled $(s)$ and unskilled $(u)$ workers to produce legal services %, $L(s,u)$ % with the following CES production function
        %The legal industry produces an output of ``Legal Services'' with two differentiated inputs, skilled labor $(s)$ unskilled labor $(u)$. Output of legal services, $L(s,u)$, is produced according to the following CES production function.
        
        \begin{equation}\label{eq:CES}
            L(\s,\u) = \left[ 
            (A_{u}\u)^{\frac{\delta - 1}{\delta}} + (A_{s}\s)^{\frac{\delta - 1}{\delta}}
            \right]^{\frac{\delta}{\delta - 1}}
        \end{equation}
        where $\delta \in [0,\infty)$ is the elasticity of substitution between the input factors. In accordance with the broad consensus of estimates for $\delta$ in the literature, 
        %and without loss of generality to our main results, 
        we consider the case where $\delta > 1$.\footnote{
                \citet{bowlus_wages_2017} provides a summary of the literature on this topic, where they refer to even the low end estimates being in the range of 1.4 to 1.8}\textsuperscript{,}\footnote{
                \citet{Autor18_lecture} describes the consensus estimate to be approximately 2 in the U.S. while the most commonly used estimate is 1.4.}\textsuperscript{,}\footnote{
                \citet{angrist_economic_1995} from the AER estimates implied elasticity of substitution between 16+ years of schooling and less than 12 to be approximately 2.}
        This corresponds to skilled and unskilled labor being imperfect substitutes.
                % While it is reasonable to assume a lawyer could do the work of a paralegal/law clerk we recognize that there must be some minimum threshold of lawyers in order for the firm to legally provide legal services. For simplicity, this requirement has been omitted, however it has little effect on our results as it is easy to assume firms are operating in the range where $s>0$.}.
        $A_u$ and $A_s$ are the factor-augmenting technology terms for unskilled and skilled labor, respectively. 

\begin{assumption}\label{skillunskill}
        Skilled labor is more productive than unskilled labor, $A_u < A_s$.\footnote{
                 While it is reasonable to assume a lawyer could do the work of a paralegal/law clerk we recognize that there must be some minimum threshold of attorneys in order for the firm to practice law. For simplicity, this requirement has been omitted, however it is without loss of generality to assume firms are operating in the range where $s>0$.}
\end{assumption}
        

        $L(\s,\u)$ is the production of \textit{all} legal services for a local area. When a firm files for Chapter 11 bankruptcy the demand for legal services increases, which results in an increase in the equilibrium level of $L$ in the market for legal services. These bankruptcy shocks are used as instruments for variation in $L$, and as such appear in the model as an increase in $L$. 
        
        % $L(s,u)$ is the production of \textit{all} legal services for a local area, we use bankruptcy as an instrument for this. According to our theory, when a firm files for Chapter 11 bankruptcy this is an intensive and complicated legal process and thus will require a significant amount of legal services. Therefore, the bankruptcy shock acts as an increase in demand legal services which, as standard economic theory would suggest, results in an increase in the equilibrium level of $L$ in the market for legal services. So the bankruptcy shock shows up in our model as an increase in $L$.  
        
        Since markets are competitive, factors receive their marginal product as wages %, we derive the following expression for wages.
        \begin{equation}\label{ws=MP}
            w_{s} = 
            A_{s}^{\frac{\delta - 1}{\delta}} 
            \left[ 
            A_{u}^{\frac{\delta - 1}{\delta}}\left(\frac{\s}{\u}\right)^{-\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}
            \right]
            ^{\frac{1}{\delta - 1}} 
            = A_{s}^{\frac{\delta - 1}{\delta}} \left( \frac{L}{\s} \right)^{1/\delta}
        \end{equation}
        \begin{equation}\label{wu=MP}
            w_{u} = 
            A_{u}^{\frac{\delta - 1}{\delta}} 
            \left[ 
            A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\frac{\s}{\u}\right)^{\frac{\delta - 1}{\delta}}
            \right]
            ^{\frac{1}{\delta - 1}}
            = A_{u}^{\frac{\delta - 1}{\delta}} \left( \frac{L}{\u} \right)^{1/\delta}
        \end{equation}
        % The critical insight from these expressions is that when $L$ increases due to a bankruptcy shock \textit{both $w_s$ and $w_u$ increase}. Which is to be expected given the increase in demand for $s$ and $u$ in response to the bankruptcy shock. 
        % However, the effect on average wage is not as clear.
        From (\ref{ws=MP}) and (\ref{wu=MP}) we obtain the following relationship for average wage in terms of relative factor intensity ($\s/\u$).  
            \begin{equation}\label{avg_wage}
                \overline{w} \equiv \frac{\u w_{u} + \s w_{s}}{\u + \s} 
                = \frac{\left[ 
                A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\s/\u\right)^{\frac{\delta - 1}{\delta}}
                \right]^{\frac{\delta}{\delta - 1}}}{1 + \s/\u}
            \end{equation}
        
        %%% LEMMA %%%
        \begin{lemma}\label{lem:skpremium_avgwage}
        If the skill premium is positive ($\frac{w_s}{w_u} > 1$), then the average wage $\overline{w}$ is increasing in $\frac{\s}{\u}$\\
        Where the skill premium is defined as:
        \begin{equation} \tag{SP}
                \pi \equiv \frac{w_s}{w_u} = \left( \frac{A_{s}}{A_{u}} \right) ^{\frac{\delta - 1}{\delta}} \left( \frac{\s}{\u}\right) ^ {-1/\delta}
        \end{equation}
        \end{lemma}  

        

\vspace{5mm}


    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsubsection{Equilibrium}
Lemma \ref{eq_lem} uses market clearing in the input markets of skilled and unskilled workers to %equate the supply and demand for skilled and unskilled labor and 
derive equilibrium wages and employment for each type of worker 
%we obtain the following expressions for the equilibrium levels of employment of skilled and unskilled workers %in the market for each type of worker.

        %%% LEMMA %%%
        \begin{lemma}\label{eq_lem} Labor Market Equilibrium for the Legal Sector:
        \begin{multicols}{2}
        \begin{equation}\label{eq_s}
        \s^{*}(L) = [\gamma^{-\delta} A_{s}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_s}}}
        \end{equation}
        
        \begin{equation}\label{eq_u}
        \u^{*}(L) = [\gamma^{-\delta} A_{u}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_u}}}
        \end{equation}
        \end{multicols}
        
        \begin{multicols}{2}
        \begin{equation}\label{eq_ws}
            w^{*}_{s}(L) = \gamma\left( A_{s}^{\delta - 1} L^{\rho_s}\right)^{\frac{1}{1+\delta\rho_{s}}} 
        \end{equation}
        
        \begin{equation}\label{eq_wu}
            w^{*}_{u}(L) = \gamma\left( A_{u}^{\delta - 1} L^{\rho_u}\right)^{\frac{1}{1+\delta\rho_{u}}} 
        \end{equation}
        \end{multicols}
        \end{lemma}
        \noindent Equations (\ref{eq_s}) and (\ref{eq_u}) show that in equilibrium both $\s$ and $\u$ are increasing in $L$. 
        
        The next Lemma shows that the frisch elasticity of labor supply $\rho_j$ plays a crucial role in determining the responsiveness of the equilibrium levels of $\s^*$ and $\u^*$ to a change in $L$ due to a bankruptcy shock.
        %The frisch elasticity of labor supply $\rho_j$ plays a critical role in determining the responsiveness of the equilibrium levels of $s$ and $u$ to a change in $L$ in response to a bankruptcy shock, as summarized in the next lemma. 
                %\noindent The ratio of \ref{eq_s} and \ref{eq_u} has the following relationship to $L$.
        In particular, by taking the ratio of (\ref{eq_s}) and (\ref{eq_u}), we formalize the compositional effect of exogenous increases in the demand for legal services.
        
        %%% LEMMA %%%
        \begin{lemma}\textbf{Compositional Channel.}\label{lem:ratio_su} Given Assumptions \ref{elasticity} and \ref{skillunskill}, an increase in the demand of legal services $L$ tilts the composition of workers towards unskilled workers
        \[\frac{\partial \left[\frac{\s^*}{\u^*}\right] }{\partial L} < 0 \]
        %if skilled workers have a lower elasticity of labor supply than unskilled workers $(\rho_u < \rho_s)$
        %Given the assumptions on $A_s, A_u$ and $\gamma$, if skilled workers have a lower elasticity of labor supply than unskilled workers $(\rho_u < \rho_s)$ (Assumption \ref{elasticity}) then
        %$$\text{if}\;\; \rho_u < \rho_s \implies \frac{\partial \left[\frac{s*}{u*}\right] }{\partial L} < 0 $$
        \end{lemma}
        
        As expected, bankruptcy shocks ($L>0$) increase wages for both skilled and unskilled labor (Eqs. \eqref{eq_ws} and \eqref{eq_wu}). Yet, the effect on average wage is less clear.
        %from (\ref{eq_ws}) and (\ref{eq_wu}) if a bankruptcy shock increases $L$, wages for both skilled and unskilled labor increase in response to the shock. 
         Proposition \ref{prop_main} uses Lemmas \ref{lem:skpremium_avgwage}, \ref{eq_lem}, and \ref{lem:ratio_su} to derive the relationship between $L$ and \textit{average wage}.
        \begin{proposition}\label{prop_main}
        Given $\rho_u < \rho_s$ and $\frac{w_s}{w_u} > 1$, an increase in $L$ will result in the following:
        
        i) Equilibrium levels of $\s^*, \u^*, w^{*}_{s}, w^{*}_{u}$ increase.
        
        ii) $\frac{\s^*}{\u^*}$ decreases (compositional channel) $\implies \overline{w} = \frac{\left[ 
                        A_{u}^{\frac{\delta - 1}{\delta}} + A_{s}^{\frac{\delta - 1}{\delta}}\left(\s/\u\right)^{\frac{\delta - 1}{\delta}}
                        \right]^{\frac{\delta}{\delta - 1}}}{\left(1 + \s/\u\right)}$ \;\; decreases. 
        \end{proposition}
        
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsubsection{Forum Shopping}
    This section incorporates forum shopping to the model through the demand for legal services $L$. We define $BR$ to be a measure of the bankruptcy shock, such as the number of local firms currently undergoing bankruptcy proceedings. Similarly, let $FS$ be a measure of how much of the bankruptcy shock is being forum shopped away. When there is no shock, $BR = FS = 0$. If there is a shock, then $BR \in\mathbb{R}^{++}$ and $FS \in [0,BR]$. The proportion of the bankruptcies that forum shops is the ratio $f \equiv \frac{FS}{BR} \in [0,1]$.
    
    The magnitude of the bankruptcy shock is $h(BR,f) \in \mathbb{R}^{+}$. Which takes the following functional form using $\lambda>0$ as a scaling parameter.  
    \begin{equation}
    \begin{split}
        h(BR,f) & = \lambda(1-f)BR \\
                                & = \lambda(BR-FS)
    \end{split}
    \end{equation}
    
    Next, we split $L$ into two parts, $L_{BR}$ the quantity of legal services for bankruptcy, and $L_{other}$ the quantity of all other legal services. The quantity of bankruptcy legal services $L_{BR} = \overline{L}_{BR}+h(BR,f)$. Where $\overline{L}_{BR}$ is the steady state level of legal services in the bankruptcy sector. 
    \begin{equation}
    \begin{split}
        L & = L_{BR} + L_{other} \\ & = \overline{L}_{BR}+ h(BR,f)+ L_{other}
    \end{split}
    \end{equation}
    \noindent Thus a bankruptcy has the following effect on the quantity demanded of legal services:
    \begin{equation}
    \begin{split}
        \frac{\partial L}{\partial BR} = \left(\frac{\partial L}{\partial h(BR,f)} \right) \left(\frac{\partial h(BR,f)}{\partial BR}\right) = \lambda (1-f) \geq 0
    \end{split}
    \end{equation}
    \noindent Similarly, we obtain the effect of a bankruptcy on employment in the legal sector. 
    \begin{equation}
    % \begin{split}
        \frac{\partial \s}{\partial BR}  = \left(\frac{\partial \s}{\partial L}\right) \left(\frac{\partial L}{\partial BR}\right) = \left(\frac{\partial \s}{\partial L}\right) \lambda (1-f)
    % \end{split}
    \end{equation}
    \begin{equation}
    % \begin{split}
        \frac{\partial \u}{\partial BR}  = \left(\frac{\partial \u}{\partial L}\right) \left(\frac{\partial L}{\partial BR}\right) = \left(\frac{\partial \s}{\partial L}\right) \lambda (1-f)
    % \end{split}
    \end{equation}
    Clearly both of these are decreasing in $f$, which combined with Lemma \ref{eq_lem}, gives us the following relationship between forum shopping and the shock:
    
    \begin{proposition}\label{prop:BR_FS} Skilled and unskilled labor both increase with bankruptcies;
    \begin{equation}
         \frac{\partial \s}{\partial BR} \geq 0 \qquad \frac{\partial \u}{\partial BR} \geq 0
    \end{equation}
    However, this effect is decreasing with respect to forum shopping;
    \begin{equation}
       \frac{\left[\frac{\partial \s}{\partial BR}\right]}{\partial FS} < 0\qquad \frac{\left[\frac{\partial \u}{\partial BR}\right]}{\partial FS} < 0
    \end{equation}
    \end{proposition}
    \noindent Proposition \ref{prop:BR_FS} is illustrated by figures \ref{Mech3} and \ref{Mech4} in the Appendix \ref{App_mechanism}. 


==> Drafts/Old/ORIGINAL_STRUCT_EST_SECTION.tex <==
Currently our database only has legal employment for the whole sector corresponding to $s + u$ in terms of the model. To perform the analysis suggested in this section, we will need a measure of $s$ and $u$ separately. We have found a promising lead on collecting this data and can hopefully follow up with these estimates shortly. 
    
    \begin{center}
    \textbf{Model}
    \end{center}
    Using the model's characterization of equilibrium in the market for legal employment, from Lemma \ref{eq_lem}, we develop a strategy for estimating the critical parameters $\rho_s$, $\rho_u$, and $\delta$. First, let us look at the equilibrium equations \ref{eq_u}, \ref{eq_s}, \ref{eq_wu}, and \ref{eq_ws}, which are listed again here. 
    
    \begin{minipage}{\textwidth}
        \begin{equation*}
        s^{*}(L) = [\gamma^{-\delta} A_{s}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_s}}}\qquad u^{*}(L) = [\gamma^{-\delta} A_{u}^{\delta - 1} L]^{\frac{1}{1+\mathbf{\delta\rho_u}}}
        \end{equation*}
        \begin{equation*}
            w^{*}_{s}(L) = \gamma\left( A_{s}^{\delta - 1} L^{\rho_s}\right)^{\frac{1}{1+\delta\rho_{s}}} \qquad w^{*}_{u}(L) = \gamma\left( A_{u}^{\delta - 1} L^{\rho_u}\right)^{\frac{1}{1+\delta\rho_{u}}}
        \end{equation*}
    \end{minipage}
    
    \begin{minipage}{\textwidth}
    \begin{center}
    \textbf{Data}
    \end{center}
    To bring this model to the data we take the natural log of each of these equations to obtain the following easily estimable expressions.
    \begin{equation*}
               \ln (s) = \alpha_{s} + \beta_{s}\ln(L) \qquad  \ln (u) = \alpha_{u} + \beta_{u} \ln(L)
            \end{equation*}
        
        where $\beta_{s}=\frac{1}{1+\mathbf{\delta\rho_s}} $ and $\beta_{u}=\frac{1}{1+\mathbf{\delta\rho_u}} $
        
    \begin{equation*}
               \ln w_s = \alpha^{w}_{s} + \beta^{w}_{s}\ln(L) \qquad  \ln w_{u} = \alpha^{w}_{u} + \beta^{w}_{u} \ln(L)
    \end{equation*}
        
    where $\beta^{w}_{s}=\frac{\rho_{s}}{1+\mathbf{\delta\rho_s}} $ and $\beta^{w}_{u}=\frac{\rho_{u}}{1+\mathbf{\delta\rho_u}} $
    \end{minipage}
  
    \begin{minipage}{\textwidth}
    \begin{center}
    \textbf{Identification}
    \end{center}  
    Estimating the above expressions as linear regressions we can use the following expressions to create estimates for the parameters in our model. The elasticity of the supply parameter, $\rho_{j}$, can be estimated with the ratio of the $\beta$ estimates from above. 
    
     \[\frac{\hat{\beta^{w}_{s}}}{\hat{\beta_{s}}}=\hat{\rho}_{s}\qquad\frac{\hat{\beta^{w}_{u}}}{\hat{\beta_{u}}}=\hat{\rho}_{u}\]
    
    Then we use the fact that $\delta\rho_{j} = \frac{1}{\beta_{j}}-1$, to obtain an estimate for $\delta$.
    
    
    \end{minipage}
    
    \noindent\underline{\textbf{Intuition:}} the lo As a result, we can identify aspects of the \textbf{supply} of legal services. In our context, labor supply and therefore preferences. Once we have obtained the estimate for the preference parameter, we can deduce the production's elasticity of substitution from the characterization of equilibrium.

==> Drafts/Old/Results_Draft.tex <==

    
    % This section provides our main results of primary interest to our work. First, we present our results on the impact of bankruptcies on  the level of legal employment. Then we discuss the findings of exploiting the forum shopping era and the  robustness checks that we performed to support our main results. Finally, we show the impact for the average wage in the legal sector.
    
    
    %     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \subsection{Legal Employment}
    
    
    
    Table \ref{tab:MainEmpLvl_BRonlyFE} reports the results of our benchmark estimations following specification \eqref{eq:spec_bench_BR} where the level of legal employment at the county is our outcome variable and the number of bankruptcies is our main independent variable. Our main estimation sample correspond to all U.S. counties with non-zero legal employment but omitting Delaware and New York for the period 1991-1996 as we discuss on our methodology section (see Section \ref{subsec:Methodology} for more details). Standard errors are clustered at the county level for all the results that follow. 
    
    The results in Table \ref{tab:MainEmpLvl_BRonlyFE} indicate that a bankruptcy filing from a firm headquartered in the county is associated with a significant increase in the level of legal employment. This impact is robust to different fixed effects specifications where we impose more demanding fixed effects along the geographical and time dimension.\footnote{We follow the Census Bureau definition of region and use 4 categories: Northeast, Midwest, South and West. In the case of the column (5) we introduce judicial district-year fixed effects. There are 94 judicial districts in the US. Hence this is akin to controlling for time-varying within state factors.} Also, the additional controls included in the specifications, county population and employment level outside the legal sector, have the expected sign and significance. 
    
    Our preferred specification controls for county and district-year fixed effects (see Column (6) in Table \ref{tab:MainEmpLvl_BRonlyFE}) and absorb all determinants of the legal employment level that are constant at the district level and absorb all the time-varying determinants at the state level, including state GDP, state unemployment rate, as well as any other state level measure of the business condition. In this specification, the effect is around an increase of 0.77\% per active bankruptcy filing in the county (see column (6) from Table \ref{tab:MainEmpLvl_BRonlyFE}). However, note that the impact is very stable across the different specifications varying between 0.070\% and 0.086\%. Hence, for the counties that have at least one bankruptcy filing, bankruptcies represent an increase of 1.69\% of the local legal employment in the county. This translates to an increase in wages paid of around 3.5 million per year based on the average wage and the average number of workers in the legal sector for these counties.
    
    \RegTable{MAIN_All_Counties90_97_OmitNYDE_BRonlyFE}{tab:MainEmpLvl_BRonlyFE}{Employment Level Regressions}{\tabnote{\lnLegEmp}{\regressorsBRonly}{\FEall}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
    



    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsection{Forum Shopping}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        In this subsection, we exploit the stipulation of the law known as Forum Shopping to verify our interpretation of the results by estimating specification  \eqref{eq:spec_bench_BR_FS}. Filing in a different court than the one were the firms has it headquarter was particularly easy to achieve during the period 1991-1996 (see Section \ref{sec:ForumShopping} for more details). This additional flexibility implied that the demand shock to the legal sector in the county where the firm was headquartered did not take place for certain bankruptcies filings. To get a sense of this, for large publicly traded firms the average distance from the firms headquarters to the court they filed in is 766.1 miles when the firm forum shops, compared to just 18.9 miles when the firm does not forum shop.\footnote{Computed using the \LPlong.}
        
        We exploit this stipulation of the law in two ways: first, as a type of placebo exercises and, second, to better measure the role of bankruptcies in the local legal employment level. 
        For the latter, once we allow heterogeneous effects for bankruptcy filings in the county and bankruptcy filings that are forum shopped, we find that the positive and significant effect on legal sector employment increases to a 1\% impact per bankruptcy filing (see column (2) from Table \ref{tab:MainEmpLvl}). 
        In addition, column (3) also confirms this finding by showing similar results when further disaggregating the forum shopping measurement by distinguishing between large forum shopped bankruptcies (LP) and small forum shopped bankruptcies (CS).
            
        Interestingly, when we exploit the stipulation of the law and  focus on the bankruptcies that are forum shopped we find that the effect of these forum shopped bankruptcies is null for legal employment. More specifically, the estimated impact on local legal employment for a forum shopped bankruptcy is -0.1\% and it is not significant (see column (2) for the second panel in Table \ref{tab:MainEmpLvl}). This combined effect remains null when the forum shopping measure is disaggregated in column (4). Hence, indicating that forum shopping exported away potential gains from bankruptcies filing in the county. The fact that bankruptcies only have a significant effect on legal employment when they are filed locally support our interpretation of the relationship between local legal employment and the bankruptcies filings. Table \ref{tab:LinCom_AvgEff} reports the combined effects of forum shopping and bankruptcy with greater detail under ``Linear Combination Tests''.  
            
        Exploring the heterogeneity of the impact of forum shopping depending on the size of the filing, Column (3) in Table \ref{tab:MainEmpLvl} highlights that the null effect associated with forum shopping is mostly associated with the big bankruptcies cases. If the firm that forum shopped its bankruptcy has assets worth less than \$340 million in 2021 dollars (\$100 million in 1980 dollars), the bankruptcy case has a positive impact of about 0.5\% on legal employment. 
        Which is in line with our initial estimate as reported by column (1) in Table \ref{tab:MainEmpLvl}. 
        Finally, the right panel of Table \ref{tab:DescriptiveStats} shows that county year's that have a bankruptcy shock have on average 1.70 bankruptcy cases and 0.47 of those are forum shopped. This implies that the average impact of bankruptcies after including the role of forum shopping is around 1.2\% according to our results on Column (2) in Table \ref{tab:MainEmpLvl}.
        % \footnote{Our results show that this impact is significant with a p-value of 0.0512} 
        Table \ref{tab:LinCom_AvgEff} reports the combined effects of forum shopping and bankruptcy with greater detail under ``Avg Effect Tests''.\footnote{We also estimate alternative versions of Table \ref{tab:MainEmpLvl} where we use different set of fixed effects following the approach of Table \ref{tab:MainEmpLvl_BRonlyFE}. The tables are reported in Appendix \ref{App_Fixed_Effects} and in all cases they confirm our results.}   
        % This implies that forum shopping reduces the impact by 0.07\% on legal employment.
        
        %CB-check.
        \RegTable{MAIN_All_Counties90_97_OmitNYDE}{tab:MainEmpLvl}{Employment Level Regressions}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
        
     
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsection{Robustness Checks}\label{sec:robust_check}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        This section reports several robustness exercises in order to ease the main concerns regarding our empirical results.
        
        %%%%%%%%%%
        %\subsubsection*
        \noindent\textbf{Include New York and Delaware counties:}
        %%%%%%%%%%
            We drop counties from New York and Delaware due to the fact that they benefit from the forum shopped cases in our main estimation sample. In order to evaluate if this is affecting our results, we reestimate our main results using an augmented version of our sample where New York and Delaware counties are included. Results are reported in Table \ref{tab:Rbst_NYDE}. Results show that a bankruptcy filing in the county increases the local legal employment level by almost a 0.1\% and that forum shopped bankruptcies has null impact on the employment level. We also consider whether bankruptcies and forum shopped filings have a different effect for New York and Delaware. We find that bankruptcies filings and forum shopped bankruptcies have no significant impact on local legal employment for counties in New York and Delaware.
            
        %%%%%%%%%%
        %\subsubsection
        \noindent\textbf{Extended Sample Period:}
        %%%%%%%%%%
            In order to explore whether our results hold when we consider a longer period, we rerun our main benchmark Table for the period 1991-2001. 
            % This period corresponds to one of the longest business cycle booms since the second world war.
            Importantly, these years make up the post-war era's longest business cycle expansion prior to the 2008 financial crisis.  
            The results in Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} are similar to our main finding that bankruptcy filings are associated with an increase in the local legal employment level.
        
        %%%%%%%%%%
        %\subsubsection
        \noindent\textbf{More Relevant Comparison Groups:}
        %%%%%%%%%%
            One potential issue with our estimating sample is that by including all counties where legal employment is non-zero we are including several counties that could never experience a bankruptcy filing of big corporation because there are none of this type of firm located in the county. We address these concerns by replicating our baseline results with samples that have been restricted to only include counties that could plausibly receive treatment. 
            
            First, since many smaller counties could never support a publicly traded firm at all, we restrict our estimation sample to only counties that have a publicly traded company located in the county at any point between 1980 and 1997. Imposing this restriction significantly reduces our estimation sample to slightly more than one third of our main one. Notwithstanding this, the results in Table \ref{tab:Rbst_HQ90_97} confirm all our main findings.
            
            Next, even among counties that can support a firm, not all of these counties have firms that could plausibly file for Chapter 11 bankruptcy during our period. So we restrict our sample even further to only include counties that had at least one firm file for bankruptcy at any point in our sample (i.e. received treatment). This drastically reduces the sample size to only 354 observations. Regardless, Table \ref{tab:RBST_BR_Counties90_97_OmitNYDE} shows our main findings still hold. 
            
        %%%%%%%%%%        
        %\subsubsection
        \noindent\textbf{Counties with Bankruptcy Court:}
        %%%%%%%%%%
            In our sample there may be a small number of cases where a firm does not forum shop, but nonetheless is still located a substantial distance from their local court. If this is the case the effect of the bankruptcy may not actually occur in the county the firm is located in, or at the very least could be reduced. In order to address these potential concerns we run our benchmark regressions on a sample that only includes the counties who have a bankruptcy court located in their county. While there are 90 judicial districts that handle bankruptcies, several of those districts have multiple physical court locations. Due to this there are approximately 200 counties that contain a bankruptcy court. Table \ref{tab:Rbst_court_counties_BR_90_97} and Table \ref{tab:Rbst_court_counties_90_97} shows that our results remain robust to this specification even though this greatly reduces the number of observations and bankruptcies in our sample.\footnote{Note that district-year fixed effects are not used because of perfect colinearity for many districts that have only 1 bankruptcy court. State-year then becomes our preferred fixed effect.}
            
        %%%%%%%%%%                
        %\subsubsection
        \noindent\textbf{Alternative Controls:}
        %%%%%%%%%%
            In our benchmark specification we include county level controls for the log of population and the log of the number of employees outside of the legal sector. We also run regressions were these controls are lagged one period in order to avoid any impact of bankruptcies in the control variables.  The results of this estimation are presented in Table \ref{tab:Rbst_Lags} and they confirm our findings. Note that this approach also avoids potential indirect effect of bankruptcies on the level of employment outside of the legal sector. Additionally, we incorporate time-varying controls, such as the unemployment rate at the county-year level, and the percent change in number of establishments outside the legal sector. 
            Again, our findings are robust to these alternative specifications (see Table \ref{tab:Rbst_UnemplRate} and Table \ref{tab:Rbst_LogEstab_Change}).

        %%%%%%%%%%
        %\subsubsection
        \noindent\textbf{Business Cycle:}
        %%%%%%%%%%
             A possible concern is that our estimates may be sensitive to macroeconomics conditions. Our main specification addresses these concerns in two ways.
            First, state-year fixed effects fully control for time-varying aggregate shocks at state and national level. In addition, our baseline sample period 1991-1996, can be considered largely free of recessions on an aggregate level.  To further ease these concerns,
            %First, note that our state-year fixed effects play an important role easing this concern. Second, the years in our sample, 1991 through 1996, can be considered largely free of recessions on an aggregate level. To further check this issues,  
            we drop the year 1991 from our baseline sample, to avoid potential contamination from the recession which ended in the first quarter of 1991.\footnote{
                See \citet{hamilton_2020} for more information.} 
            Table \ref{tab:Rbst_drop91} shows that our estimates are largely unaffected by this change. Further, Tables \ref{tab:Rbst_UnemplRate} and \ref{tab:Rbst_LogEstab_Change} show that our results are robust to the inclusion of alternative measures of local business cycle fluctuations.
        
        %%%%%%%%%%
        %\subsubsection
        \noindent\textbf{Alternative Measures for Bankruptcy Treatment:}
        %%%%%%%%%%
            Table \ref{tab:Rbst_FSBR_dummy} shows that our estimates are robust to replacing the bankruptcy, and forum shopping, count variables with their respective dummies--albeit with a lower significant level.%\footnote{ Defined as indicator function that takes value 1 }.
            %our main estimation benchmark of measuring bankruptcies and forum shopped bankruptcies using binary variables instead of count one. 
            % We find that all our results hold, albeit with a lower significant level. 
            Table \ref{tab:Rbst_FSBR_dummy} shows estimates when we replace the bankruptcy (and forum shopping) count variables with their respective dummies. 
            Our main findings still hold, albeit with a lower significant level. This result is expected, due to the fact that these measurements for bankruptcies and forum shopping are less precise compared to the benchmark count variables.
        
        %%%%%%%%%%
        %\subsubsection
        \noindent\textbf{Alternative Data Source:}
        %%%%%%%%%%
            In order to further verify the validity of our results we replicate our findings by constructing the employment variables from an alternative data source. Specifically, the dependent variable for legal employment, as well as the control for non-legal employment, are constructed using data from the Bureau of Labor Statistics (\BLS) rather than \CBP \space data. 
            The results from Table \ref{tab:Rbst_BLSdata} demonstrate that even with the less complete \BLS \space data we still observe a significant and positive effect from bankruptcies that is canceled out by forum shopping. The drop in quality from the \BLS\space database is evidenced by the fact that the number of observations drops by nearly 6,000 due to missing data.
 
        %%%%%%%%%%        
        %\subsubsection
        \noindent\textbf{Spillover Effects:}
        %%%%%%%%%%
            To address the potential for spillover effects from these bankruptcies we run an additional specification which controls for potential spillover from nearby bankruptcies. To do this we create a measure of the number of bankruptcies filings in \textit{directly adjacent} counties to county $c$ in year $t$. As shown by Table \ref{tab:Rbst_AdjCounty}, we find no evidence that bankruptcies in adjacent counties have a meaningful impact on local legal employment.
            
    
        % %\subsubsection
        % \noindent\textbf{Alternative robustness layout}
        % \begin{itemize}
        %     \item Include NY and DE
        %     \item leg emp and br 1991-2001 (talk about in results)
        %     % \item counties with firm HQ
        %     % \item counties with br court br and fs version
        %     % \item lagged controls
        %     % \item control for unemp
        %     % \item control for non legal estab
        %     % \item drop 1991 (wage and emp)
        %     % \item dummy version
        %     \item alternative data source 
        %     \item fixed effects
        %     % \item counties with br at some point
        %     % \item counties with br or were adjacent to br at some point
        %     % \item adjacent county br
        % \end{itemize}
        
        % \begin{itemize}
        %     \item More relevant comparison group
        %         \begin{itemize}
        %             \item counties with br at some point 
        %             \item counties with br or were adjacent to br at some point.
        %             \item counties with firm HQ.
        %             \item counties with br court br and fs version
        %         \end{itemize}
        %     \item Results not caused by other economic conditions
        %         \begin{itemize}
        %             \item lagged controls
        %             \item control for unemp
        %             \item control for non legal estab
        %             \item drop 1991 (wage and emp)
        %         \end{itemize}
        %     \item Alternative treatment measures
        %         \begin{itemize}
        %             \item dummy version
        %             \item adjacent county br 
        %         \end{itemize}
        % \end{itemize}

        
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsection{Wage in the Legal Sector}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        Thus far we have shown the effect of bankruptcy shocks on legal sector employment levels, i.e. quantity in the market for labor in the legal sector. In this section we investigate bankruptcy shocks impact on price levels in the form of average wage to get a more complete picture of how legal sector labor markets respond to bankruptcy shocks.
        % In this section we extend our analysis to the average wage in the legal sector to get a more complete picture of how legal sector labor markets respond to bankruptcy shocks. 
        However, it is much more difficult to measure the impact of labor demand shocks on wage than on employment levels, because wages tend to be ``stickier'' than employment levels in the short run. Consistent with this predicted ``stickiness'' our results in Table \ref{tab:avg_wage_reg_noBRsplit} show a much smaller impact on wages than we saw on employment levels, and in turn lower significance with only column (3) estimating a significant impact from the bankruptcy shocks. 
        
        Yet, despite the minimal significance, the direction of the estimated effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
        Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
        
        Similar to the results on employment level, Table \ref{tab:avg_wage_reg_noBRsplit} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 
        
        \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE_noBRsplit}{tab:avg_wage_reg_noBRsplit}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}
        
        
        % OLD VERSION WITH EXTRA COLUMN FOR LP CS BR SPLIT
        \iffalse
        Table \ref{tab:avg_wage_reg} reports our results for average wage in the legal sector. Columns (1), and (2), fail to show significance and column (3) shows minimal significance for the estimated effect of a bankruptcy on average wage. 
        This result is consistent with the idea that wages tend to be ``stickier" than employment levels in the short run and require a larger shock to record a meaningful change. 
        Column (4) corroborates this hypothesis, showing that large firm bankruptcy shocks ``Bankruptcies (LP)'' indeed have a statistically and economically significant effect.
        
        Yet, the direction of the effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
        Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.
        
        Similar to the results on employment level, Table \ref{tab:avg_wage_reg} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 
        
        \RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE}{tab:avg_wage_reg}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}
        
        \fi





























% OLD RESULTS SECTION!!!!!!!!!!!!!!
\iffalse
This section provides our main results of primary interest to our work. First, we present our results on the impact of bankruptcies on  the level of legal employment. Then we discuss the findings of exploiting the forum shopping era and the  robustness checks that we performed to support our main results. Finally, we show the impact for the average wage in the legal sector.


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Legal Employment}




%% An alternative way of making our results more robust to the econometric policy, is to make table 5 all about BR (only) with different set of FEs, and perhaps different controls and discuss the main findings. Perhaps also NY and DE.  Then create a new subsection called: Exploiting the Court Competition Era where we frame the forum shopping as an identification strategy. Then we can also have a Placebo subsection. What do you think?

%% Then we run additional robustness. 


Table \ref{tab:MainEmpLvl_BRonlyFE} reports the results of our benchmark estimations following specification \eqref{eq:spec_bench_BR} where the level of legal employment at the county is our outcome variable and the number of bankruptcies is our main independent variable. Our main estimation sample correspond to all U.S. counties with non-zero legal employment but omitting Delaware and New York for the period 1991-1996 as we discuss on our methodology section (see Section \ref{subsec:Methodology} for more details). We clustered our standard errors at the county level for all the results that follows. 

The results in Table \ref{tab:MainEmpLvl_BRonlyFE} indicate that a bankruptcy filing from a firm headquartered in the county is associated with a significant increase in the level of legal employment. This impact is robust to different fixed effects specifications where we impose more demanding fixed effects along the geographical and time dimension.\footnote{We follow the Census Bureau definition of region and use 4 categories: Northeast, Midwest, South and West. In the case of the column (5) we introduce judicial district-year fixed effects. There are 94 judicial districts in the US. Hence this is akin to controlling for time-varying within state factors.} Also, the additional controls included in the specifications, county population and employment level outside the legal sector, have the expected sign and significance. 

Our preferred specification controls for county and district-year fixed effects (see Column (6) in Table \ref{tab:MainEmpLvl_BRonlyFE}) and absorb all determinants of the legal employment level that are constant at the district level and absorb all the time-varying determinants at the state level, including state GDP, state unemployment rate, as well as any other state level measure of the business condition. In this specification, the effect is around an increase of 0.77\% per active bankruptcy filing in the county (see column (6) from Table \ref{tab:MainEmpLvl_BRonlyFE}). However, note that the impact is very stable across the different specifications varying between 0.070\% and 0.086\%. Hence, for the counties that have at least one bankruptcy filing, bankruptcies represent an increase of 1.69\% of the local legal employment in the county. This translates to an increase in wages paid of around 3.5 million per year based on the average wage and the average number of workers in the legal sector for these counties.

\RegTable{MAIN_All_Counties90_97_OmitNYDE_BRonlyFE}{tab:MainEmpLvl_BRonlyFE}{Employment Level Regressions}{\tabnote{\lnLegEmp}{\regressorsBRonly}{\FEall}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}

\subsubsection{Forum Shopping}

In this subsection, we exploit the stipulation of the law known as Forum Shopping to verify our interpretation of the results by estimating specification  \eqref{eq:spec_bench_BR_FS}. Filing in a different court than the one were the firms has it headquarter was particularly easy to achieve during the period 1991-1996 (see Section \ref{sec:ForumShopping} for more details). This additional flexibility implied that the demand shock to the legal sector in the county where the firm was headquartered did not take place for certain bankruptcies filings. To get a sense of this, for large publicly traded firms the average distance from the firms headquarters to the court they filed in is 766.1 miles when the firm forum shops, compared to just 18.9 miles when the firm does not forum shop.\footnote{Computed using the \LPlong.}

% a standard bankruptcy filing for a large publicly traded firm takes place 8.7 miles from the headquarter of the firm on average but a forum shopped bankruptcy takes place 749.7 miles away.\footnote{Computed using the \LPlong.} 

We exploit this stipulation of the law in two ways: first, as a type of placebo exercises and, second, to better measure the role of bankruptcies in the local legal employment level. For the latter, once we allow heterogeneous effects for bankruptcy filings in the county and bankruptcy filings that are forum shopped, we find that the positive and significant effect on legal sector employment increases to a 1\% impact per bankruptcy filing (see column (2) from Table \ref{tab:MainEmpLvl}). In addition, column (3) also confirms this finding by showing similar results when further disaggregating the forum shopping measurement by distinguishing between large forum shopped bankruptcies (LP) and small forum shopped bankruptcies (CS).
    
Interestingly, when we exploit the stipulation of the law and  focus on the bankruptcies that are forum shopped we find that the effect of these forum shopped bankruptcies is null for legal employment. More specifically, the estimated impact on local legal employment for a forum shopped bankruptcy is -0.1\% and it is not significant (see column (2) for the second panel in Table \ref{tab:MainEmpLvl}). This combined effect remains null when the forum shopping measure is disaggregated in column (4). Hence, indicating that forum shopping exported away potential gains from bankruptcies filing in the county. The fact that bankruptcies only have a significant effect on legal employment when they are filed locally support our interpretation of the relationship between local legal employment and the bankruptcies filings. Table \ref{tab:LinCom_AvgEff} reports the combined effects of forum shopping and bankruptcy with greater detail under ``Linear Combination Tests''.  
    
Exploring the heterogeneity of the impact of forum shopping depending on the size of the filing, Column (3) in Table \ref{tab:MainEmpLvl} highlights that the null effect associated with forum shopping is mostly associated with the big bankruptcies cases. If the firm that forum shopped its bankruptcy has assets worth less than \$340 million in 2021 dollars (\$100 million in 1980 dollars), the bankruptcy case has a positive impact of about 0.5\% on legal employment. 
Which is in line with our initial estimate as reported by column (1) in Table \ref{tab:MainEmpLvl}. 
Finally, the right panel of Table \ref{tab:DescriptiveStats} shows that county year's that have a bankruptcy shock have on average 1.70 bankruptcy cases and 0.47 of those are forum shopped. This implies that the average impact of bankruptcies after including the role of forum shopping is around 1.2\% according to our results on Column (2) in Table \ref{tab:MainEmpLvl}.
% \footnote{Our results show that this impact is significant with a p-value of 0.0512} 
Table \ref{tab:LinCom_AvgEff} reports the combined effects of forum shopping and bankruptcy with greater detail under ``Avg Effect Tests''.\footnote{We also estimate alternative versions of Table \ref{tab:MainEmpLvl} where we use different set of fixed effects following the approach of Table \ref{tab:MainEmpLvl_BRonlyFE}. The tables are reported in Appendix \ref{App_Fixed_Effects} and in all cases they confirm our results.}   
% This implies that forum shopping reduces the impact by 0.07\% on legal employment.



%CB-check.
\RegTable{MAIN_All_Counties90_97_OmitNYDE}{tab:MainEmpLvl}{Employment Level Regressions}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}



    \subsubsection{Placebo Tests}

\RegTable{RBST_Placebo_All_Counties90_97_OmitNYDE}{tab:placebo}{Employment Level Regressions with lags for bankruptcy shock.}{\tabnote{\lnLegEmp}{\regressorsPLACEBO}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}

We perform several placebo test to evaluate whether there were differences in the local legal employment level in the counties affected by bankruptcies before the filings took place. In order to do this, we lagged the variable that captures the number of bankruptcies. More specifically, we use three alternative lag structures: one, two and three years before the bankruptcies actually took place. Additionally, we combined all the three lagged measures in the same specification. 

Results in Table \ref{tab:placebo} show that none of the bankruptcies measures have a significant effect and the estimated coefficients shrink by an order of magnitude. Hence, there are no significant differences in the level of local legal employment for the counties affected by bankruptcies before the bankruptcies actually take place.  These results point in the same direction that our findings exploiting the forum shopping period and reassures our finding that bankruptcies filings are associated with an positive impact on the local legal employment level.\footnote{We also run some additional placebo tests where we use binary indicators  as measures for bankruptcies. The results in Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} in the appendix also confirms our findings.}
     
\subsubsection{Robustness Checks}\label{sec:robust_check}      
\newcommand{\secnum}{\ref{sec:robust_check}}
This section reports several robustness exercises in order to ease the main concerns regarding our empirical results. \\
% 
\noindent\textbf{\secnum.1 Inclusion of New York and Delaware counties.}\\ We drop counties from New York and Delaware due to the fact that they benefit from the forum shopped cases in our main estimation sample. In order to evaluate if this is affecting our results, we reestimate our main results using an augmented version of our sample where New York and Delaware counties are included. Results are reported in Table \ref{tab:Rbst_NYDE}. Results show that a bankruptcy filing in the county increases the local legal employment level by almost a 0.1\% and that forum shopped bankruptcies has null impact on the employment level. We also consider whether bankruptcies and forum shopped filings have a different effect for New York and Delaware. We find that bankruptcies filings and forum shopped bankruptcies have no significant impact on local legal employment for counties in New York and Delaware.\\
% 
\noindent\textbf{\secnum.2 Alternative Sample Period (1991-2001).}\\ In order to explore whether our results hold when we consider a longer period, we rerun our main benchmark Table for the period 1991-2001. 
% This period corresponds to one of the longest business cycle booms since the second world war.
Importantly, these years make up the longest business cycle expansion prior to the 2008 financial crisis.  
The results in Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} are similar to our main finding that bankruptcy filings are associated with an increase in the local legal employment level.\\
% \noindent\textbf{\secnum.2 Alternative Sample Period (1991-2001).}\\ In order to explore whether our results hold when we consider a longer period, we rerun our main benchmark Table for the period 1991-2001. This period corresponds to the pre-financial crisis longest business cycle boom, since the second world war. The results in Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} are similar to our main finding that bankruptcy filings are associated with an increase in the local legal employment level.\\
% 
\noindent\textbf{\secnum.3 Counties with Headquarters.}\\ One potential issue with our estimating sample is that by including all counties where legal employment is non-zero we are including several counties that could never experience a bankruptcy filing of big corporation because there are none of this type of firm located in the county. We address these concerns by replicating our baseline results where the estimation sample is restricted to only counties that have a publicly traded company located in the county at any point between 1980 and 1997. Imposing this restriction significantly reduces our estimation sample to slightly more than one third of our main one. Notwithstanding this, the results in Table \ref{tab:Rbst_HQ90_97} confirm all our main findings. \\
% 
\noindent\textbf{\secnum.4 Counties with Bankruptcy Court.}\\ In our sample there may be a small number of cases where a firm does not forum shop, but nonetheless is still located a substantial distance from their local court. If this is the case the effect of the bankruptcy may not actually occur in the county the firm is located in, or at the very least could be reduced. In order to address these potential concerns we run our benchmark regressions on a sample that only includes the counties who have a bankruptcy court located in their county. While there are 90 judicial districts that handle bankruptcies, several of those districts have multiple physical court locations. Due to this there are approximately 200 counties that contain a bankruptcy court. Table \ref{tab:Rbst_court_counties_BR_90_97} and Table \ref{tab:Rbst_court_counties_90_97} shows that our results remain robust to this specification even though this greatly reduces the number of observations and bankruptcies in our sample.\footnote{Note that district-year fixed effects are not used because of perfect colinearity for many districts that have only 1 bankruptcy court. State-year then becomes our preferred fixed effect.}\\
% 
\noindent\textbf{\secnum.5 Alternative Controls.}\\ In our benchmark specification we include county level controls for the log of population and the log of the number of employees outside of the legal sector. We also run regressions were these controls are lagged one period in order to avoid any impact of bankruptcies in the control variables.  The results of this estimation are presented in Table \ref{tab:Rbst_Lags} and they confirm our findings. Note that this approach also avoids potential indirect effect of bankruptcies on the level of employment outside of the legal sector. Additionally, we incorporate time-varying controls, such as the unemployment rate at the county-year level, and the percent change in number of establishments outside the legal sector. 
Again, our findings are robust to these alternative specifications (see Table \ref{tab:Rbst_UnemplRate} and Table \ref{tab:Rbst_LogEstab_Change}).\\
% 
\noindent\textbf{\secnum.6 Business Cycle.}\\ 
A possible concern is that our estimates may be sensitive to macroeconomics conditions. Our main specification addresses these concerns in two ways.
First, state-year fixed effects fully control for time-varying aggregate shocks at state and national level. In addition, our baseline sample period 1991-1996, can be considered largely free of recessions on an aggregate level.  To further ease these concerns,
%First, note that our state-year fixed effects play an important role easing this concern. Second, the years in our sample, 1991 through 1996, can be considered largely free of recessions on an aggregate level. To further check this issues,  
we drop the year 1991 from our baseline sample, to avoid potential contamination from the recession which ended in the first quarter of 1991.\footnote{
    See \citet{hamilton_2020} for more information.} 
Table \ref{tab:Rbst_drop91} shows that our estimates are largely unaffected by this change. Further, Table \ref{tab:Rbst_UnemplRate} shows that our results are robust to the inclusion of alternative measures of local business cycle fluctuations as measured by the county unemployment rate.\\  
%because county level unemployment rate can be considered  a measure of business cycle conditions  
%Since the unemployment rate at the county could also be considered correlated with the business cycle conditions, our results presented in Table \ref{tab:Rbst_UnemplRate} that include the unemployment rate in the county show that our main results are robust to using different measures of the business conditions in the county.\\   
% 
\noindent\textbf{\secnum.7 Alternative Bankruptcy Measures.}\\
Table \ref{tab:Rbst_FSBR_dummy} shows that our estimates are robust to replacing the bankruptcy, and forum shopping, count variables with their respective dummies--albeit with a lower significant level.%\footnote{ Defined as indicator function that takes value 1 }.
%our main estimation benchmark of measuring bankruptcies and forum shopped bankruptcies using binary variables instead of count one. 
% We find that all our results hold, albeit with a lower significant level. 
Table \ref{tab:Rbst_FSBR_dummy} shows estimates when we replace the bankruptcy (and forum shopping) count variables with their respective dummies. 
Our main findings still hold, albeit with a lower significant level. This result is expected, due to the fact that these measurements for bankruptcies and forum shopping are less precise compared to the benchmark count variables.\\
% 
\noindent\textbf{\secnum.8 Alternative Data Source.}\\
In order to further verify the validity of our results we replicate our findings by constructing the employment variables from an alternative data source. Specifically, the dependent variable for legal employment, as well as the control for non-legal employment, are constructed using data from the Bureau of Labor Statistics (\BLS) rather than \CBP \space data. 
The results from Table \ref{tab:Rbst_BLSdata} demonstrate that even with the less complete \BLS \space data we still observe a significant and positive effect from bankruptcies that is canceled out by forum shopping. The drop in quality from the \BLS\space database is evidenced by the fact that the number of observations drops by nearly 6,000 due to missing data.\\
% 
% Even though the CBP database to be more complete and less prone to errors. This is evidenced by the fact that with \BLS\space data the number of observations drops by nearly 6,000 due to missing data. In spite of this less complete database we still see a significant and positive effect from bankruptcies, that is canceled out by forum shopping.  
% 
% 
% 
% By replicating our results using an alternative data source we further demonstrate the validity of our results. 
% 
% We evaluate whether our results are robust to constructing our employment variables an alternative data. More specifically, we use Bureau of Labor Statistics (BLS) data rather than CBP data. We expect the CBP database to be more complete and less prone to errors. This is evidenced by the fact that the number of observations drops by nearly 6,000 when using BLS data to construct measures of employment due to missing data. Even with this less complete database we see that bankruptcies still have a significant positive impact on employment and the combined effect of bankruptcies and forum shopping is not significantly different from zero. These results are reported in Table \ref{tab:Rbst_BLSdata}. \\
% 
\noindent\textbf{\secnum.9 Spillover Effects. }\\
To address the potential for spillover effects from these bankruptcies we run an additional specification which controls for potential spillover from nearby bankruptcies. To do this we create a measure of the number of bankruptcies filings in \textit{directly adjacent} counties to county $c$ in year $t$. As shown by Table \ref{tab:Rbst_AdjCounty}, we find no evidence that bankruptcies in adjacent counties have a meaningful impact on local legal employment. 

% We include these regressions in order to quell potential concerns that spillover effects from nearby counties could be affecting our results.   
% To do this we create a measure of the number of bankruptcies filings in \textit{directly adjacent} counties to county $c$ in year $t$. Table \ref{tab:Rbst_AdjCounty} show that bankruptcies in adjacent counties have no impact on the local legal employment in the county. 


% \begin{itemize}
%     \item \textbf{Include New York and Delaware counties:} We drop counties from New York and Delaware due to the fact that they benefit from the forum shopped cases in our main estimation sample. In order to evaluate if this is affecting our results, we reestimate our main results using an augmented version of our sample where New York and Delaware counties are included. Results are reported in Table \ref{tab:Rbst_NYDE}. Results show that a bankruptcy filing in the county increases the local legal employment level by almost a 0.1\% and that forum shopped bankruptcies has null impact on the employment level. We also consider whether bankruptcies and forum shopped filings have a different effect for New York and Delaware. We find that bankruptcies filings and forum shopped bankruptcies have no significant impact on local legal employment for counties in New York and Delaware.
    
%     \item \textbf{Counties with Headquarters:} One potential issue with our estimating sample is that by including all counties where legal employment is non-zero we are including several counties that could never experience a bankruptcy filing of big corporation because there are none of this type of firm located in the county. To ease this concern, we replicate our baseline results where the estimation sample is restricted to all counties that have a publicly traded company located in the county at any point between 1980 and 1997. Imposing this restriction significantly reduces our estimation sample to a slightly more than one third of our main one. Notwithstanding this, the results in Table \ref{tab:Rbst_HQ90_97} confirm all our main findings. 
    
%     \item \textbf{Extending the Period:} In order to explore whether our results hold when we consider a longer period, we rerun our main benchmark Table for the period 1991-2001. The results in Table \ref{tab:MainEmpLvl_BRonlyFE_90_02} are similar to our main finding that bankruptcy filings are associated with an increase in the local legal employment level.  
    
%     \item \textbf{Controls:} in our benchmark estimations we include the log of population at the county and the log of the number of employee outside of the legal sector in the county. We also run regressions were these controls are lagged one period in order to avoid any impact of bankruptcies in the control variables.  The results of this estimation are presented in  \ref{tab:Rbst_Lags} and they confirm our findings. Note that this approach also avoids potential indirect effect of bankruptcies on the level of employment outside of the legal sector. Additionally, we incorporate an additional time-varying control, the unemployment rate at the county-year level. Again, our results remain the same when we include this additional control (see Table \ref{tab:Rbst_UnemplRate}).
    
%     \item \textbf{Business Conditions:} A possible concern with our main results is that they might be very sensitive to the overall macroeconomics conditions. First, note that our state-year fixed effects play an important role easing this concern. Second, the years in our sample, 1991 through 1996, can be considered largely free of recessions on an aggregate level. To further check this issues,  we estimate our main results dropping the year 1991 due to the fact that the early 1990's recession ended in 1991.\footnote{See \citet{hamilton_2020} for more information.} Results are reported in Table \ref{tab:Rbst_drop91} and show that our main results are robust to dropping this year. Since the unemployment rate at the county could also be considered correlated with the business condition, our results presented in Table \ref{tab:Rbst_UnemplRate} that include the unemployment rate in the county show that our main results are robust to using different measures of the business conditions in the county.   
    
%     \item \textbf{Alternative Bankruptcy Measures:} In the Table \ref{tab:Rbst_FSBR_dummy} we show the results for our main estimation benchmark of measuring bankruptcies and forum shopped bankruptcies using binary variables instead of count one. We find that all our results hold, albeit with a lower significant level.  Note that this could be expected due to the fact that our measurement for bankruptcies and forum shopping is less precise compared to our benchmark estimation strategy.
    
%     \item \textbf{Alternative  Data Source:}
%      We evaluate whether our results are robust to constructing our employment variables an alternative data. More specifically, we use Bureau of Labor Statistics (BLS) data rather than CBP data. We expect the CBP database to be more complete and less prone to errors. This is evidenced by the fact that the number of observations drops by nearly 6,000 when using BLS data to construct measures of employment due to missing data. Even with this less complete database we see that bankruptcies still have a significant positive impact on employment and the combined effect of bankruptcies and forum shopping is not significantly different from zero. These results are reported in Table \ref{tab:Rbst_BLSdata}. 
    
%     \item \textbf{Adjacent County Bankruptcies: }
%     We include these regressions in order to quell potential concerns that spillover effects from nearby counties could be affecting our results.   
%     To do this we create a measure of the number of bankruptcies filings in \textit{directly adjacent} counties to county $c$ in year $t$. Table \ref{tab:Rbst_AdjCounty} show that bankruptcies in adjacent counties have no impact on the local legal employment in the county. 
% \end{itemize}
        
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\subsection{Wage in the Legal Sector}
In this section we extend our analysis to the average wage in the legal sector to get a more complete picture of how legal sector labor markets respond to bankruptcy shocks. 
It is however much more difficult to measure the impact of labor demand shocks on wage than on employment levels, because wages tend to be ``stickier'' than employment levels in the short run. Consistent with this predicted ``stickiness'' our results in Table \ref{tab:avg_wage_reg_noBRsplit} show a much smaller impact on wages than we saw on employment levels, and in turn lower significance with only column (3) estimating a significant impact from the bankruptcy shocks. 

Yet, despite the minimal significance, the direction of the estimated effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.

Similar to the results on employment level, Table \ref{tab:avg_wage_reg_noBRsplit} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 

\RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE_noBRsplit}{tab:avg_wage_reg_noBRsplit}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}


% OLD VERSION WITH EXTRA COLUMN FOR LP CS BR SPLIT
\iffalse
Table \ref{tab:avg_wage_reg} reports our results for average wage in the legal sector. Columns (1), and (2), fail to show significance and column (3) shows minimal significance for the estimated effect of a bankruptcy on average wage. 
This result is consistent with the idea that wages tend to be ``stickier" than employment levels in the short run and require a larger shock to record a meaningful change. 
Column (4) corroborates this hypothesis, showing that large firm bankruptcy shocks ``Bankruptcies (LP)'' indeed have a statistically and economically significant effect.

Yet, the direction of the effect is puzzling. Shouldn't positive demand shocks have a positive effect on wages? The next section specializes a model with skilled and unskilled workers and reconciles this puzzling observation with a compositional effect. 
Bankruptcy shocks increase the demand in the county of both high paid attorneys and low paid paralegals and legal clerks. However, the increase in demand is relatively larger for the lower skilled workers, who tend to have a more elastic labor supply. As a result, the \textit{average} wage goes down.

Similar to the results on employment level, Table \ref{tab:avg_wage_reg} indicates that the combined effect bankruptcies and forum shopping is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 

\RegTable{MAIN_All_Counties90_97_OmitNYDE_WAGE}{tab:avg_wage_reg}{Average Annual Pay for Legal Sector.}{\tabnote{\lnavgwage}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}

\fi



% at the bottom of Table \ref{tab:avg_wage_reg} the test of the linear combination of the estimates for bankruptcy and forum shopping shows that their combined effect is not significantly different from zero. 

%Which intuitively supports our model proposed mechanism that relative factor intensity ($\frac{s}{u}$) is driving the average wage down. 
    

% %%%%%% OLD
%     This section reports our results for average wage in the legal sector. While the theory predicts that the wage will go up for skilled and unskilled workers in response to the bankruptcy shock, the compositional effect is less clear. The results in Table \ref{tab:avg_wage_reg} are consistent with our models prediction that a bankruptcy shock has a null or negative effect on average wage. 
    
%     These results are particularly interesting, not only for their evidence of a compositional channel of effect, but also due to the fact that wages are generally considered to be much "stickier" than employment levels. Due to this inertia wages have to stay relatively stable, it is much more difficult for a shock to the labor market to have a significant effect on wages than employment levels. Which intuitively supports our model proposed mechanism that relative factor intensity ($\frac{s}{u}$) is driving the average wage down. 
    
%     Looking at Table \ref{tab:avg_wage_reg} columns (1), (2), and (3) fail to show significance for the estimated effect of a bankruptcy on average wage. This is consistent with the idea that wages tend to be sticky. Column (4) shows that the shock can in fact be significant, \textit{but only for the largest bankruptcies}, which are captured by n\_BR\_LP. 
    
%     Finally, at the bottom of the Table the test of the linear combination of the estimates for bankruptcy and forum shopping shows that their combined effect is not significantly different from zero. Thus, as we would expect, it appears that forum shopping is canceling out any shock to the local labor market for legal employment that a firm going into bankruptcy otherwise would have had. 
% %%%%% OLD

       

        

        

% \iffalse

\fi

==> Drafts/Robustness_Tables_Old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Robustness Checks}\label{App:Robust_Check}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    This section reports several robustness exercises discussed in Section \ref{sec:robust_check} aimed at easing concerns regarding our empirical results. We grouped these robustness exercises in three broad categories: (i) sample definition, (ii) controls included, and (iii) bankruptcy measurement.  In all cases our main results are unchanged.
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    \subsection{Sample}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
        In this subsection, we show that our results are robust to adjusting our sample considered in the regression analysis along several dimensions. We first include New York and Delaware counties data. Second, we extend our sample to cover the period 1991-2001. Third, we drop 1991 from our benchmark sample period. Fourth, we narrow our sample to only include counties where a publicly traded firm was located, then we focus on counties where at least a bankruptcy took place during our sample period. Finally, we limit the sample to counties where district courts are located. See Section \ref{sec:robust_check_sample} for a detailed discussion. 
  
        
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Include New York and Delaware Counties}\label{App:NYDE}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            % \newgeometry{top=3.2cm}
            
            \RegTab{RBST_All_Counties90_97_INCLUDE_NYDE}{tab:Rbst_NYDE}{Legal sector employment level with NY and DE included.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\sampleNYDE}{\sampleyears}{\source}}
    \restoregeometry
        
        
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Bankruptcy Shocks and Legal Employment- Extended Period}\label{App:legemp_91_01}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTable{MAIN_All_Counties90_02_OmitNYDE_BRonlyFE}{tab:MainEmpLvl_BRonlyFE_90_02}{Employment Level Regressions}{\tabnote{\lnLegEmp}{\regressorsBRonly}{\FEall}{\controls}{\clustercounty}{\samplerestr}{\sampleyearsExtendedPeriod}{\source}}
            
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Restricted Sample Period}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties91_97_OmitNYDE}{tab:Rbst_drop91}{Employment level regressions dropping 1991 from sample.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyearsDROPNintyOne}{\source}}
    
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{More Relevant Comparison Groups}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_HQ_Counties90_97_OmitNYDE}{tab:Rbst_HQ90_97}{Employment Level Regressions over sample of only HQ counties.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\sampleHQ}{\sampleyears}{\source}}
            
            \RegTab{RBST_BR_Counties90_97_OmitNYDE}{tab:RBST_BR_Counties90_97_OmitNYDE}{Employment Level Regressions for only county-year observations that had a BR during the period 1991-1996.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\sampleBRcounties}{\sampleyears}{\source}}
            
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Counties with Bankruptcy Courts}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTable{RBST_All_Counties90_97_OmitNYDE_BRonlyFE_CourtCounties}{tab:Rbst_court_counties_BR_90_97}{Employment Level Regressions over sample of only counties that have a bankruptcy court.}{\tabnote{\lnLegEmp}{\regressorsBRonly}{\FEall}{\controls}{\clustercounty}{\sampleBRcourts}{\sampleyears}{\source}}
            
            \RegTab{RBST_All_Counties90_97_OmitNYDE_CourtCounties}{tab:Rbst_court_counties_90_97}{Employment Level Regressions over sample of only counties that have a bankruptcy court.}{\tabnote{\lnLegEmp}{\regressors}{\countySY}{\controls}{\clustercounty}{\sampleBRcourts}{\sampleyears}{\source}}



    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    \subsection{Controls}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
        In our benchmark specification, we include county level controls for the log of population and the log of the number of employees outside of the legal sector. In this subsection, we extend our set of controls by lagging the controls and by including new time-varying county variables. 
        See Section \ref{sec:robust_check_controls} for a detailed discussion. 
    
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Lagged Controls}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties90_97_OmitNYDE_LAGS}{tab:Rbst_Lags}{Employment Level Regressions with controls lagged by 1 year.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controlsLAG}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
            
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Business Cycle}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties90_97_OmitNYDE_UnempRate}{tab:Rbst_UnemplRate}{Employment Level Regressions with control for unemployment rate.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controlsUNEMPRATE}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}
            
            \RegTab{RBST_All_Counties90_97_OmitNYDE_PERCENT_EstabChange}{tab:Rbst_LogEstab_Change}{Employment Level Regressions with control for change in the log of number of Establishments outside of legal sector.}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controlsESTABCHANGE}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceAVGWAGE}}



    \subsection{Measurement}
        In this subsection, we explore the robustness of our main results to alternative measurements of bankruptcies, forum shopping bankruptcies, and employment levels in the legal sector and non-legal sector.  In all cases, our findings are aligned with our priors.
        See Section \ref{sec:robust_check_measurement} for a detailed discussion. 
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Binary Measurement}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties90_97_OmitNYDE_Dummies}{tab:Rbst_FSBR_dummy}{Employment level regressions replacing bankruptcy and forum shop regressors with their dummy variable counterparts.}{\tabnote{\lnLegEmp}{\regressorsDUMMY}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
            
            
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Value Weighted Measurement}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTable{MAIN_90_97_OmitNYDE_ASSETS}{tab:Rbst_ValWeight}{Employment Level Regressions with value of bankrupt firms assets as measure of bankruptcy and forum shop (assets in billions of 2021 dollars).}{\tabnote{\lnLegEmp}{\regressorsASSETS}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
            
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Spillover Effects}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties90_97_OmitNYDE_ADJ}{tab:Rbst_AdjCounty}{Employment Level Regressions controlling for bankruptcies in adjacent counties.}{\tabnote{\lnLegEmp}{\regressorsADJ}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\source}}
    
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \subsubsection{Alternative Data Source}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \RegTab{RBST_All_Counties90_97_OmitNYDE_BLS}{tab:Rbst_BLSdata}{Employment Level Regressions using BLS data}{\tabnote{\lnLegEmp}{\regressors}{\countyDisY}{\controls}{\clustercounty}{\samplerestr}{\sampleyears}{\sourceNoCBP}}

==> Regressions/DisY_FE_test/MAIN_All_Counties90_02_OmitNYDE_BRonlyFE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &      0.0117\sym{***}&      0.0146\sym{***}&      0.0144\sym{***}&      0.0134\sym{***}&      0.0143\sym{***}&      0.0123\sym{***}\\
                    &   (0.00353)         &   (0.00354)         &   (0.00341)         &   (0.00323)         &   (0.00357)         &   (0.00394)         \\
\addlinespace
ln(County Population)&       0.584\sym{***}&       0.761\sym{***}&       0.627\sym{***}&       0.570\sym{***}&       0.644\sym{***}&       0.608\sym{***}\\
                    &    (0.0757)         &    (0.0785)         &    (0.0823)         &    (0.0827)         &    (0.0890)         &    (0.0905)         \\
\addlinespace
ln(Emp Non Legal)   &       0.139\sym{***}&       0.201\sym{***}&       0.232\sym{***}&       0.247\sym{***}&       0.247\sym{***}&       0.251\sym{***}\\
                    &    (0.0417)         &    (0.0485)         &    (0.0489)         &    (0.0493)         &    (0.0502)         &    (0.0514)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.972         &       0.972         &       0.972         &       0.972         &       0.973         &       0.973         \\
Observations        &       29416         &       29416         &       29416         &       29416         &       29416         &       29361         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00768\sym{**} &      0.0107\sym{***}&      0.0110\sym{***}\\
                    &   (0.00335)         &   (0.00381)         &   (0.00383)         \\
\addlinespace
Forum Shopping      &                     &     -0.0133\sym{**} &                     \\
                    &                     &   (0.00638)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0186\sym{**} \\
                    &                     &                     &   (0.00779)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00649         \\
                    &                     &                     &   (0.00917)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE_BRonlyFE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &     0.00793\sym{***}&     0.00830\sym{***}&     0.00859\sym{***}&     0.00702\sym{**} &     0.00720\sym{**} &     0.00768\sym{**} \\
                    &   (0.00280)         &   (0.00287)         &   (0.00284)         &   (0.00283)         &   (0.00330)         &   (0.00335)         \\
\addlinespace
ln(County Population)&       0.797\sym{***}&       0.750\sym{***}&       0.694\sym{***}&       0.651\sym{***}&       0.726\sym{***}&       0.715\sym{***}\\
                    &     (0.115)         &     (0.125)         &     (0.134)         &     (0.134)         &     (0.137)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.181\sym{***}&       0.166\sym{***}&       0.170\sym{***}&       0.174\sym{***}&       0.167\sym{***}&       0.170\sym{***}\\
                    &    (0.0418)         &    (0.0468)         &    (0.0474)         &    (0.0479)         &    (0.0481)         &    (0.0489)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         &       15963         &       15963         &       15931         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE_ESTABLISHMENTS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &    -0.00635\sym{**} &    -0.00761\sym{**} &    -0.00702\sym{**} \\
                    &   (0.00307)         &   (0.00346)         &   (0.00336)         \\
\addlinespace
Forum Shopping      &                     &     0.00562         &                     \\
                    &                     &   (0.00639)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &    -0.00522         \\
                    &                     &                     &   (0.00784)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &      0.0193\sym{***}\\
                    &                     &                     &   (0.00747)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.991         &       0.991         &       0.991         \\
Observations        &       17591         &       17591         &       17591         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE_LINCOM_AVGEFFECT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00768\sym{**} &      0.0107\sym{***}&      0.0110\sym{***}\\
                    &   (0.00335)         &   (0.00381)         &   (0.00383)         \\
\addlinespace
Forum Shopping      &                     &     -0.0133\sym{**} &                     \\
                    &                     &   (0.00638)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0186\sym{**} \\
                    &                     &                     &   (0.00779)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00649         \\
                    &                     &                     &   (0.00917)         \\
\midrule
                    &                     &                     &                     \\
\textbf{Linear Combination Tests:}&                     &                     &                     \\
Forum Shopped Bankruptcies&                     &    -0.00264         &                     \\
                    &                     &    (0.0055)         &                     \\
Forum Shopped Bankruptcies LP&                     &                     &    -0.00763         \\
                    &                     &                     &   (0.00653)         \\
Forum Shopped Bankruptcies non-LP&                     &                     &     0.00450         \\
                    &                     &                     &   (0.00907)         \\
\midrule            &                     &                     &                     \\
\textbf{Avg Effect Tests:}&                     &                     &                     \\
Bankruptcies        &0.0131\sym{**}         &                     &                     \\
                    &    (0.0057)         &                     &                     \\
Forum Shopped Bankruptcies&                     &0.0113\sym{**}         &                     \\
                    &                     &   (0.00556)         &                     \\
Forum Shopped Bankruptcies LP&                     &                     &0.0125\sym{*}         \\
                    &                     &                     &   (0.00554)         \\
Forum Shopped Bankruptcies non-LP&                     &                     &0.0175\sym{**}         \\
                    &                     &                     &   (0.00634)         \\
\midrule            &                     &                     &                     \\
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE_WAGE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Bankruptcies        &   -0.000808         &    -0.00345         &    -0.00386         &                     \\
                    &   (0.00236)         &   (0.00246)         &   (0.00252)         &                     \\
\addlinespace
Bankruptcies (LP)   &                     &                     &                     &     -0.0170\sym{**} \\
                    &                     &                     &                     &   (0.00746)         \\
\addlinespace
Bankruptcies (CS)   &                     &                     &                     &    0.000752         \\
                    &                     &                     &                     &   (0.00297)         \\
\addlinespace
Forum Shopping      &                     &      0.0118\sym{**} &                     &                     \\
                    &                     &   (0.00598)         &                     &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &      0.0186\sym{**} &      0.0321\sym{***}\\
                    &                     &                     &   (0.00913)         &    (0.0115)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     0.00296         &    -0.00173         \\
                    &                     &                     &   (0.00652)         &   (0.00637)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.932         &       0.932         &       0.932         &       0.932         \\
Observations        &       10684         &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties90_97_OmitNYDE_WAGE_noBRsplit.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &   -0.000808         &    -0.00345         &    -0.00386         \\
                    &   (0.00236)         &   (0.00246)         &   (0.00252)         \\
\addlinespace
Forum Shopping      &                     &      0.0118\sym{**} &                     \\
                    &                     &   (0.00598)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &      0.0186\sym{**} \\
                    &                     &                     &   (0.00913)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     0.00296         \\
                    &                     &                     &   (0.00652)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.932         &       0.932         &       0.932         \\
Observations        &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/MAIN_All_Counties96_02_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &      0.0120\sym{**} &     0.00313         &     0.00319         \\
                    &   (0.00497)         &   (0.00633)         &   (0.00633)         \\
\addlinespace
Forum Shopping      &                     &      0.0176\sym{*}  &                     \\
                    &                     &   (0.00929)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &      0.0185\sym{*}  \\
                    &                     &                     &   (0.00966)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &      0.0108         \\
                    &                     &                     &    (0.0266)         \\
\addlinespace
ln(County Population)&       0.404\sym{***}&       0.403\sym{***}&       0.403\sym{***}\\
                    &     (0.135)         &     (0.135)         &     (0.135)         \\
\addlinespace
ln(Emp Non Legal)   &       0.107         &       0.106         &       0.106         \\
                    &    (0.0787)         &    (0.0788)         &    (0.0788)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.978         &       0.978         &       0.978         \\
Observations        &       13295         &       13295         &       13295         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_02_OmitNYDE_BRonlyFE_ESTABLISHMENTS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &    -0.00221         &    -0.00206         &    -0.00151         &    -0.00125         &    -0.00115         &   -0.000750         \\
                    &   (0.00240)         &   (0.00267)         &   (0.00263)         &   (0.00262)         &   (0.00281)         &   (0.00260)         \\
\addlinespace
ln(County Population)&       0.734\sym{***}&       0.544\sym{***}&       0.582\sym{***}&       0.608\sym{***}&       0.602\sym{***}&       0.583\sym{***}\\
                    &    (0.0589)         &    (0.0594)         &    (0.0626)         &    (0.0618)         &    (0.0662)         &    (0.0670)         \\
\addlinespace
ln(Emp Non Legal)   &       0.291\sym{***}&       0.156\sym{***}&       0.150\sym{***}&       0.144\sym{***}&       0.140\sym{***}&       0.144\sym{***}\\
                    &    (0.0322)         &    (0.0343)         &    (0.0348)         &    (0.0348)         &    (0.0350)         &    (0.0357)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.985         &       0.985         &       0.985         &       0.985         \\
Observations        &       32416         &       32416         &       32416         &       32416         &       32416         &       32354         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_NYDE_Interact.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00770\sym{**} &      0.0107\sym{***}&      0.0110\sym{***}\\
                    &   (0.00335)         &   (0.00382)         &   (0.00383)         \\
\addlinespace
Bankruptcies x NYDE &    -0.00488         &    -0.00518         &    -0.00534         \\
                    &   (0.00792)         &   (0.00843)         &   (0.00861)         \\
\addlinespace
Forum Shopping      &                     &     -0.0133\sym{**} &                     \\
                    &                     &   (0.00639)         &                     \\
\addlinespace
Forum Shopping x NYDE&                     &     0.00396         &                     \\
                    &                     &    (0.0111)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0186\sym{**} \\
                    &                     &                     &   (0.00779)         \\
\addlinespace
Forum Shopping (LP) x NYDE&                     &                     &     0.00301         \\
                    &                     &                     &   (0.00945)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00648         \\
                    &                     &                     &   (0.00918)         \\
\addlinespace
Forum Shopping (CS) x NYDE&                     &                     &     0.00558         \\
                    &                     &                     &    (0.0267)         \\
\addlinespace
ln(Emp Non Legal)   &       0.169\sym{***}&       0.169\sym{***}&       0.169\sym{***}\\
                    &    (0.0486)         &    (0.0486)         &    (0.0486)         \\
\addlinespace
ln(County Population)&       0.710\sym{***}&       0.710\sym{***}&       0.710\sym{***}\\
                    &     (0.143)         &     (0.143)         &     (0.143)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.985         &       0.985         &       0.985         \\
Observations        &       16314         &       16314         &       16314         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_ADJ.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00658\sym{*}  &     0.00955\sym{**} &     0.00986\sym{**} \\
                    &   (0.00358)         &   (0.00406)         &   (0.00408)         \\
\addlinespace
Adjacent County Bankruptcies&    -0.00337         &    -0.00336         &    -0.00334         \\
                    &   (0.00358)         &   (0.00358)         &   (0.00358)         \\
\addlinespace
Forum Shopping      &                     &     -0.0132\sym{**} &                     \\
                    &                     &   (0.00634)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0183\sym{**} \\
                    &                     &                     &   (0.00774)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00658         \\
                    &                     &                     &   (0.00915)         \\
\addlinespace
ln(County Population)&       0.711\sym{***}&       0.711\sym{***}&       0.711\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0489)         &    (0.0490)         &    (0.0490)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_BLS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00569\sym{**} &     0.00831\sym{**} &     0.00839\sym{**} \\
                    &   (0.00282)         &   (0.00327)         &   (0.00330)         \\
\addlinespace
Forum Shopping      &                     &     -0.0117\sym{**} &                     \\
                    &                     &   (0.00518)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0129\sym{*}  \\
                    &                     &                     &   (0.00689)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     -0.0100\sym{*}  \\
                    &                     &                     &   (0.00608)         \\
\addlinespace
ln\_EmpNoLegal\_BLS   &       0.210\sym{***}&       0.210\sym{***}&       0.210\sym{***}\\
                    &    (0.0556)         &    (0.0556)         &    (0.0556)         \\
\addlinespace
ln(County Population)&       0.640\sym{***}&       0.640\sym{***}&       0.640\sym{***}\\
                    &     (0.121)         &     (0.121)         &     (0.121)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.996         &       0.996         &       0.996         \\
Observations        &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_BR_Counties.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Forum Shopping      &     0.00419         &                     \\
                    &   (0.00816)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &    -0.00248         \\
                    &                     &   (0.00862)         \\
\addlinespace
Forum Shopping (CS) &                     &      0.0124         \\
                    &                     &    (0.0134)         \\
\addlinespace
ln(Emp Non Legal)   &      0.0248         &      0.0182         \\
                    &     (0.324)         &     (0.326)         \\
\addlinespace
ln(County Population)&       2.229\sym{***}&       2.183\sym{***}\\
                    &     (0.776)         &     (0.783)         \\
\midrule
County FE           &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         \\
R-Squared           &       0.998         &       0.998         \\
Observations        &         227         &         227         \\
\bottomrule
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_BRonlyFE_CourtCounties.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &     0.00554\sym{**} &     0.00757\sym{***}&     0.00801\sym{***}&     0.00662\sym{***}&     0.00874\sym{**} &     0.00905\sym{*}  \\
                    &   (0.00230)         &   (0.00237)         &   (0.00205)         &   (0.00223)         &   (0.00390)         &   (0.00477)         \\
\addlinespace
ln(County Population)&       0.266         &       0.180         &       0.405\sym{**} &       0.417\sym{**} &       0.424\sym{*}  &       0.309         \\
                    &     (0.164)         &     (0.162)         &     (0.175)         &     (0.180)         &     (0.233)         &     (0.275)         \\
\addlinespace
ln(Emp Non Legal)   &       0.441\sym{***}&       0.433\sym{***}&       0.350\sym{***}&       0.331\sym{***}&       0.296\sym{**} &       0.336\sym{***}\\
                    &    (0.0873)         &     (0.120)         &     (0.118)         &     (0.114)         &     (0.129)         &     (0.127)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.998         &       0.999         &       0.999         &       0.999         &       0.999         &       0.999         \\
Observations        &        1116         &        1116         &        1116         &        1116         &        1074         &         972         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_BRonlyFE_ESTABLISHMENTS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &    -0.00939\sym{***}&    -0.00820\sym{***}&    -0.00758\sym{***}&    -0.00832\sym{***}&    -0.00737\sym{**} &    -0.00635\sym{**} \\
                    &   (0.00286)         &   (0.00265)         &   (0.00257)         &   (0.00262)         &   (0.00290)         &   (0.00307)         \\
\addlinespace
ln(County Population)&       0.907\sym{***}&       0.767\sym{***}&       0.721\sym{***}&       0.688\sym{***}&       0.730\sym{***}&       0.700\sym{***}\\
                    &    (0.0826)         &    (0.0875)         &    (0.0921)         &    (0.0929)         &    (0.0995)         &     (0.102)         \\
\addlinespace
ln(Emp Non Legal)   &      0.0959\sym{***}&      0.0534\sym{*}  &      0.0598\sym{*}  &      0.0658\sym{**} &      0.0594\sym{*}  &      0.0631\sym{*}  \\
                    &    (0.0281)         &    (0.0309)         &    (0.0314)         &    (0.0317)         &    (0.0319)         &    (0.0324)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.990         &       0.990         &       0.990         &       0.990         &       0.990         &       0.991         \\
Observations        &       17627         &       17627         &       17627         &       17627         &       17627         &       17591         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_CourtCounties.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00905\sym{*}  &     0.00921\sym{*}  &     0.00936         \\
                    &   (0.00477)         &   (0.00517)         &   (0.00590)         \\
\addlinespace
Forum Shopping      &                     &   -0.000856         &                     \\
                    &                     &   (0.00634)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &    -0.00204         \\
                    &                     &                     &    (0.0104)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     0.00188         \\
                    &                     &                     &    (0.0157)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.999         &       0.999         &       0.999         \\
Observations        &         972         &         972         &         972         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_Dummies.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcy          &      0.0141         &      0.0192\sym{*}  &      0.0193\sym{*}  \\
                    &   (0.00862)         &    (0.0104)         &    (0.0104)         \\
\addlinespace
Forum Shop          &                     &     -0.0165         &                     \\
                    &                     &    (0.0103)         &                     \\
\addlinespace
Forum Shop (LP)     &                     &                     &     -0.0212\sym{*}  \\
                    &                     &                     &    (0.0114)         \\
\addlinespace
FS\_CS               &                     &                     &    -0.00987         \\
                    &                     &                     &    (0.0132)         \\
\addlinespace
ln(County Population)&       0.715\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0489)         &    (0.0489)         &    (0.0489)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_EstabChange.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00941\sym{**} &      0.0126\sym{***}&      0.0130\sym{***}\\
                    &   (0.00376)         &   (0.00424)         &   (0.00425)         \\
\addlinespace
Forum Shopping      &                     &     -0.0142\sym{**} &                     \\
                    &                     &   (0.00652)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0211\sym{***}\\
                    &                     &                     &   (0.00818)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00550         \\
                    &                     &                     &   (0.00892)         \\
\addlinespace
ln(County Population)&       0.707\sym{***}&       0.707\sym{***}&       0.707\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.166\sym{***}&       0.166\sym{***}&       0.166\sym{***}\\
                    &    (0.0486)         &    (0.0487)         &    (0.0487)         \\
\addlinespace
$\Delta$(Non-Legal Establishments)&   0.0000381\sym{**} &   0.0000381\sym{**} &   0.0000386\sym{***}\\
                    & (0.0000151)         & (0.0000150)         & (0.0000148)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15925         &       15925         &       15925         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_LAGS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00803\sym{**} &      0.0107\sym{***}&      0.0110\sym{***}\\
                    &   (0.00329)         &   (0.00380)         &   (0.00383)         \\
\addlinespace
Forum Shopping      &                     &     -0.0119\sym{*}  &                     \\
                    &                     &   (0.00652)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0169\sym{**} \\
                    &                     &                     &   (0.00780)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00530         \\
                    &                     &                     &   (0.00935)         \\
\addlinespace
L.ln(Emp Non Legal) &       0.126\sym{***}&       0.126\sym{***}&       0.126\sym{***}\\
                    &    (0.0402)         &    (0.0402)         &    (0.0402)         \\
\addlinespace
L.ln(County Population)&       0.855\sym{***}&       0.855\sym{***}&       0.855\sym{***}\\
                    &     (0.149)         &     (0.149)         &     (0.149)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_PERCENT_EstabChange.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00794\sym{**} &      0.0111\sym{***}&      0.0114\sym{***}\\
                    &   (0.00348)         &   (0.00393)         &   (0.00394)         \\
\addlinespace
Forum Shopping      &                     &     -0.0141\sym{**} &                     \\
                    &                     &   (0.00643)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0197\sym{**} \\
                    &                     &                     &   (0.00788)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00709         \\
                    &                     &                     &   (0.00917)         \\
\addlinespace
ln(County Population)&       0.716\sym{***}&       0.716\sym{***}&       0.716\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.161\sym{***}&       0.161\sym{***}&       0.161\sym{***}\\
                    &    (0.0481)         &    (0.0481)         &    (0.0481)         \\
\addlinespace
\%$\Delta$(Non-Legal Establishments)&      0.0774         &      0.0774         &      0.0773         \\
                    &    (0.0722)         &    (0.0722)         &    (0.0722)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15925         &       15925         &       15925         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_UnempRate.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00758\sym{**} &      0.0106\sym{***}&      0.0110\sym{***}\\
                    &   (0.00334)         &   (0.00380)         &   (0.00382)         \\
\addlinespace
Forum Shopping      &                     &     -0.0136\sym{**} &                     \\
                    &                     &   (0.00642)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0189\sym{**} \\
                    &                     &                     &   (0.00781)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00674         \\
                    &                     &                     &   (0.00918)         \\
\addlinespace
ln(County Population)&       0.719\sym{***}&       0.719\sym{***}&       0.719\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.175\sym{***}&       0.175\sym{***}&       0.175\sym{***}\\
                    &    (0.0496)         &    (0.0496)         &    (0.0496)         \\
\addlinespace
Unemployment Rate   &     0.00274         &     0.00275         &     0.00276         \\
                    &   (0.00283)         &   (0.00283)         &   (0.00283)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00847\sym{***}&      0.0105\sym{***}&      0.0108\sym{***}\\
                    &   (0.00285)         &   (0.00356)         &   (0.00361)         \\
\addlinespace
Forum Shopping      &                     &    -0.00930\sym{*}  &                     \\
                    &                     &   (0.00476)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0138\sym{**} \\
                    &                     &                     &   (0.00614)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00377         \\
                    &                     &                     &   (0.00600)         \\
\addlinespace
ln(Emp Non Legal)   &       0.167\sym{***}&       0.167\sym{***}&       0.167\sym{***}\\
                    &    (0.0463)         &    (0.0463)         &    (0.0464)         \\
\addlinespace
ln(County Population)&       0.742\sym{***}&       0.743\sym{***}&       0.743\sym{***}\\
                    &     (0.126)         &     (0.126)         &     (0.126)         \\
\addlinespace
ln(State GDP)       &      0.0509         &      0.0509         &      0.0507         \\
                    &    (0.0487)         &    (0.0487)         &    (0.0487)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county_DisY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00768\sym{**} &      0.0107\sym{***}&      0.0110\sym{***}\\
                    &   (0.00335)         &   (0.00381)         &   (0.00383)         \\
\addlinespace
Forum Shopping      &                     &     -0.0133\sym{**} &                     \\
                    &                     &   (0.00638)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0186\sym{**} \\
                    &                     &                     &   (0.00779)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00649         \\
                    &                     &                     &   (0.00917)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0489)         &    (0.0489)         &    (0.0489)         \\
\addlinespace
ln(County Population)&       0.715\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(State GDP)       &                     &                     &                     \\
                    &                     &                     &                     \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &         Yes         &         Yes         &         Yes         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county_DivY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00694\sym{**} &     0.00906\sym{**} &     0.00928\sym{***}\\
                    &   (0.00283)         &   (0.00353)         &   (0.00358)         \\
\addlinespace
Forum Shopping      &                     &    -0.00958\sym{*}  &                     \\
                    &                     &   (0.00515)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0133\sym{**} \\
                    &                     &                     &   (0.00645)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00492         \\
                    &                     &                     &   (0.00642)         \\
\addlinespace
ln(Emp Non Legal)   &       0.175\sym{***}&       0.175\sym{***}&       0.175\sym{***}\\
                    &    (0.0479)         &    (0.0479)         &    (0.0479)         \\
\addlinespace
ln(County Population)&       0.665\sym{***}&       0.665\sym{***}&       0.665\sym{***}\\
                    &     (0.134)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(State GDP)       &     -0.0927         &     -0.0932         &     -0.0932         \\
                    &     (0.120)         &     (0.120)         &     (0.120)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &         Yes         &         Yes         &         Yes         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county_RegY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00859\sym{***}&      0.0105\sym{***}&      0.0107\sym{***}\\
                    &   (0.00285)         &   (0.00360)         &   (0.00364)         \\
\addlinespace
Forum Shopping      &                     &    -0.00856\sym{*}  &                     \\
                    &                     &   (0.00500)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0113\sym{*}  \\
                    &                     &                     &   (0.00627)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00522         \\
                    &                     &                     &   (0.00646)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0476)         &    (0.0476)         &    (0.0476)         \\
\addlinespace
ln(County Population)&       0.692\sym{***}&       0.692\sym{***}&       0.692\sym{***}\\
                    &     (0.134)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(State GDP)       &     0.00925         &     0.00834         &     0.00841         \\
                    &     (0.108)         &     (0.108)         &     (0.108)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &         Yes         &         Yes         &         Yes         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county_SY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00720\sym{**} &     0.00949\sym{**} &     0.00987\sym{**} \\
                    &   (0.00330)         &   (0.00391)         &   (0.00396)         \\
\addlinespace
Forum Shopping      &                     &     -0.0104\sym{*}  &                     \\
                    &                     &   (0.00616)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0168\sym{**} \\
                    &                     &                     &   (0.00740)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00239         \\
                    &                     &                     &   (0.00827)         \\
\addlinespace
ln(Emp Non Legal)   &       0.167\sym{***}&       0.167\sym{***}&       0.167\sym{***}\\
                    &    (0.0481)         &    (0.0481)         &    (0.0481)         \\
\addlinespace
ln(County Population)&       0.726\sym{***}&       0.726\sym{***}&       0.726\sym{***}\\
                    &     (0.137)         &     (0.137)         &     (0.137)         \\
\addlinespace
ln(State GDP)       &                     &                     &                     \\
                    &                     &                     &                     \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &         Yes         &         Yes         &         Yes         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties90_97_OmitNYDE_county_year.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00831\sym{***}&      0.0106\sym{***}&      0.0109\sym{***}\\
                    &   (0.00288)         &   (0.00359)         &   (0.00363)         \\
\addlinespace
Forum Shopping      &                     &     -0.0104\sym{**} &                     \\
                    &                     &   (0.00482)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0148\sym{**} \\
                    &                     &                     &   (0.00602)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00494         \\
                    &                     &                     &   (0.00616)         \\
\addlinespace
ln(Emp Non Legal)   &       0.166\sym{***}&       0.166\sym{***}&       0.166\sym{***}\\
                    &    (0.0470)         &    (0.0470)         &    (0.0470)         \\
\addlinespace
ln(County Population)&       0.739\sym{***}&       0.739\sym{***}&       0.739\sym{***}\\
                    &     (0.126)         &     (0.126)         &     (0.126)         \\
\addlinespace
ln(State GDP)       &      0.0481         &      0.0471         &      0.0473         \\
                    &     (0.101)         &     (0.102)         &     (0.102)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &         Yes         &         Yes         &         Yes         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties91_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00831\sym{**} &      0.0117\sym{**} &      0.0120\sym{**} \\
                    &   (0.00410)         &   (0.00493)         &   (0.00494)         \\
\addlinespace
Forum Shopping      &                     &     -0.0132\sym{*}  &                     \\
                    &                     &   (0.00720)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0207\sym{**} \\
                    &                     &                     &   (0.00915)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00421         \\
                    &                     &                     &   (0.00896)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.986         &       0.986         &       0.986         \\
Observations        &       13327         &       13327         &       13327         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties91_97_OmitNYDE_WAGE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
Bankruptcies        &    0.000646         &    -0.00312         &    -0.00348         &                     \\
                    &   (0.00285)         &   (0.00310)         &   (0.00317)         &                     \\
\addlinespace
Bankruptcies (LP)   &                     &                     &                     &     -0.0177\sym{**} \\
                    &                     &                     &                     &   (0.00828)         \\
\addlinespace
Bankruptcies (CS)   &                     &                     &                     &     0.00193         \\
                    &                     &                     &                     &   (0.00357)         \\
\addlinespace
Forum Shopping      &                     &      0.0146\sym{**} &                     &                     \\
                    &                     &   (0.00688)         &                     &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &      0.0240\sym{**} &      0.0392\sym{***}\\
                    &                     &                     &    (0.0104)         &    (0.0135)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     0.00341         &    -0.00198         \\
                    &                     &                     &   (0.00710)         &   (0.00691)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.939         &       0.939         &       0.939         &       0.939         \\
Observations        &        8904         &        8904         &        8904         &        8904         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_All_Counties91_97_OmitNYDE_WAGE_noBRsplit.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &    0.000646         &    -0.00312         &    -0.00348         \\
                    &   (0.00285)         &   (0.00310)         &   (0.00317)         \\
\addlinespace
Forum Shopping      &                     &      0.0146\sym{**} &                     \\
                    &                     &   (0.00688)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &      0.0240\sym{**} \\
                    &                     &                     &    (0.0104)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &     0.00341         \\
                    &                     &                     &   (0.00710)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.939         &       0.939         &       0.939         \\
Observations        &        8904         &        8904         &        8904         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_HQ_Counties90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00563\sym{*}  &     0.00904\sym{**} &     0.00947\sym{**} \\
                    &   (0.00319)         &   (0.00384)         &   (0.00388)         \\
\addlinespace
Forum Shopping      &                     &     -0.0152\sym{**} &                     \\
                    &                     &   (0.00702)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &                     &     -0.0223\sym{***}\\
                    &                     &                     &   (0.00809)         \\
\addlinespace
Forum Shopping (CS) &                     &                     &    -0.00598         \\
                    &                     &                     &   (0.00945)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.994         &       0.994         &       0.994         \\
Observations        &        5533         &        5533         &        5533         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_Placebo_All_Counties90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
L.Bankruptcies      &     0.00231         &                     &                     &     0.00256         \\
                    &   (0.00312)         &                     &                     &   (0.00312)         \\
\addlinespace
L2.Bankruptcies     &                     &    0.000304         &                     &   -0.000529         \\
                    &                     &   (0.00280)         &                     &   (0.00256)         \\
\addlinespace
L3.Bankruptcies     &                     &                     &   -0.000118         &    0.000549         \\
                    &                     &                     &   (0.00315)         &   (0.00335)         \\
\addlinespace
ln(County Population)&       0.715\sym{***}&       0.716\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.171\sym{***}&       0.171\sym{***}\\
                    &    (0.0489)         &    (0.0489)         &    (0.0490)         &    (0.0490)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15930         &       15930         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_Placebo_All_Counties90_97_OmitNYDE_DUMMY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
L.Bankruptcy        &     0.00368         &                     &                     &     0.00413         \\
                    &   (0.00694)         &                     &                     &   (0.00679)         \\
\addlinespace
L2.Bankruptcy       &                     &    -0.00160         &                     &    -0.00205         \\
                    &                     &   (0.00606)         &                     &   (0.00581)         \\
\addlinespace
L3.Bankruptcy       &                     &                     &     0.00109         &     0.00181         \\
                    &                     &                     &   (0.00810)         &   (0.00815)         \\
\addlinespace
ln(County Population)&       0.715\sym{***}&       0.716\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.171\sym{***}&       0.171\sym{***}\\
                    &    (0.0489)         &    (0.0489)         &    (0.0490)         &    (0.0490)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15930         &       15930         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_Placebo_All_Counties90_97_OmitNYDE_DUMMY_WAGE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
L.Bankruptcy        &     -0.0103\sym{**} &                     &                     &    -0.00968\sym{*}  \\
                    &   (0.00515)         &                     &                     &   (0.00518)         \\
\addlinespace
L2.Bankruptcy       &                     &    -0.00814         &                     &    -0.00733         \\
                    &                     &   (0.00545)         &                     &   (0.00513)         \\
\addlinespace
L3.Bankruptcy       &                     &                     &     0.00104         &    0.000146         \\
                    &                     &                     &   (0.00557)         &   (0.00557)         \\
\addlinespace
ln(County Population)&     -0.0282         &     -0.0294         &     -0.0306         &     -0.0272         \\
                    &    (0.0831)         &    (0.0832)         &    (0.0831)         &    (0.0832)         \\
\addlinespace
ln(Emp Non Legal)   &      0.0485\sym{*}  &      0.0484\sym{*}  &      0.0484\sym{*}  &      0.0484\sym{*}  \\
                    &    (0.0287)         &    (0.0287)         &    (0.0287)         &    (0.0287)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.932         &       0.932         &       0.932         &       0.932         \\
Observations        &       10684         &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_Placebo_All_Counties90_97_OmitNYDE_WAGE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
L.Bankruptcies      &    -0.00197         &                     &                     &    -0.00163         \\
                    &   (0.00255)         &                     &                     &   (0.00246)         \\
\addlinespace
L2.Bankruptcies     &                     &    -0.00156         &                     &    -0.00112         \\
                    &                     &   (0.00312)         &                     &   (0.00271)         \\
\addlinespace
L3.Bankruptcies     &                     &                     &    0.000339         &    0.000183         \\
                    &                     &                     &   (0.00253)         &   (0.00244)         \\
\addlinespace
ln(County Population)&     -0.0299         &     -0.0303         &     -0.0306         &     -0.0298         \\
                    &    (0.0832)         &    (0.0832)         &    (0.0831)         &    (0.0832)         \\
\addlinespace
ln(Emp Non Legal)   &      0.0486\sym{*}  &      0.0484\sym{*}  &      0.0485\sym{*}  &      0.0485\sym{*}  \\
                    &    (0.0287)         &    (0.0287)         &    (0.0287)         &    (0.0287)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.932         &       0.932         &       0.932         &       0.932         \\
Observations        &       10684         &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/DisY_FE_test/RBST_Placebo_BR_equal_FS_90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Forum Shopping      &     -0.0117         &                     \\
                    &   (0.00800)         &                     \\
\addlinespace
Forum Shopping (LP) &                     &     -0.0148         \\
                    &                     &    (0.0101)         \\
\addlinespace
Forum Shopping (CS) &                     &    -0.00684         \\
                    &                     &    (0.0123)         \\
\addlinespace
ln(County Population)&       0.708\sym{***}&       0.708\sym{***}\\
                    &     (0.147)         &     (0.147)         \\
\addlinespace
ln(Emp Non Legal)   &       0.171\sym{***}&       0.171\sym{***}\\
                    &    (0.0494)         &    (0.0494)         \\
\midrule
County FE           &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         \\
R-Squared           &       0.981         &       0.981         \\
Observations        &       15567         &       15567         \\
\bottomrule
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/GMM.tex <==
\midrule
Parameters  &      0.0853\sym{***}&       0.264\sym{**} &       1.292\sym{***}\\
            &    (0.0307)         &     (0.120)         &     (0.150)         \\


==> Regressions/GMM_CC_Era.tex <==
\midrule
Parameters  &      0.0792\sym{*}  &       0.195         &       1.397\sym{***}\\
            &    (0.0423)         &     (0.164)         &     (0.101)         \\


==> Regressions/GMM_No_Constant.tex <==
\midrule
Parameters  &      0.0223         &     0.00933         &       1.268\sym{***}\\
            &    (0.0519)         &     (0.118)         &     (0.133)         \\


==> Regressions/GMM_Simple.tex <==
\midrule
Parameters  &      0.0750\sym{**} &       0.238\sym{*}  &      -7.942         \\
            &    (0.0325)         &     (0.124)         &     (18.16)         \\


==> Regressions/GMM_Simple_With_Cons.tex <==
\midrule
Parameters  &       0.110\sym{***}&       0.228\sym{*}  &       2.859\sym{*}  \\
            &    (0.0313)         &     (0.131)         &     (1.508)         \\


==> Regressions/GMM_With_Cons.tex <==
\midrule
Parameters  &       0.113\sym{***}&       0.280\sym{***}&       1.294\sym{***}\\
            &    (0.0289)         &     (0.108)         &     (0.149)         \\


==> Regressions/New_Layout/FE_County_Year_RegY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &     0.00793\sym{***}&     0.00948\sym{***}&     0.00830\sym{***}&      0.0101\sym{***}&     0.00859\sym{***}&      0.0100\sym{***}\\
                    &   (0.00280)         &   (0.00349)         &   (0.00287)         &   (0.00355)         &   (0.00284)         &   (0.00356)         \\
\addlinespace
Forum Shopping      &                     &    -0.00741         &                     &    -0.00873\sym{*}  &                     &    -0.00689         \\
                    &                     &   (0.00518)         &                     &   (0.00518)         &                     &   (0.00522)         \\
\addlinespace
ln(County Population)&       0.797\sym{***}&       0.797\sym{***}&       0.750\sym{***}&       0.750\sym{***}&       0.694\sym{***}&       0.694\sym{***}\\
                    &     (0.115)         &     (0.115)         &     (0.125)         &     (0.125)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.181\sym{***}&       0.182\sym{***}&       0.166\sym{***}&       0.166\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0418)         &    (0.0418)         &    (0.0468)         &    (0.0468)         &    (0.0474)         &    (0.0474)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &         Yes         &         Yes         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         &          No         &         Yes         &         Yes         \\
Division-Year       &          No         &          No         &          No         &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &          No         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors clustered at county level in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/FE_DivY_SY_DisY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Bankruptcies        &     0.00702\sym{**} &     0.00862\sym{**} &     0.00720\sym{**} &     0.00878\sym{**} &     0.00768\sym{**} &      0.0100\sym{***}\\
                    &   (0.00283)         &   (0.00348)         &   (0.00330)         &   (0.00385)         &   (0.00335)         &   (0.00373)         \\
\addlinespace
Forum Shopping      &                     &    -0.00772         &                     &    -0.00759         &                     &     -0.0111\sym{*}  \\
                    &                     &   (0.00527)         &                     &   (0.00623)         &                     &   (0.00637)         \\
\addlinespace
ln(County Population)&       0.651\sym{***}&       0.651\sym{***}&       0.726\sym{***}&       0.726\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.134)         &     (0.134)         &     (0.137)         &     (0.137)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.174\sym{***}&       0.174\sym{***}&       0.167\sym{***}&       0.167\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0479)         &    (0.0479)         &    (0.0481)         &    (0.0481)         &    (0.0489)         &    (0.0489)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         &          No         &          No         &          No         \\
Division-Year       &         Yes         &         Yes         &          No         &          No         &          No         &          No         \\
State-Year          &          No         &          No         &         Yes         &         Yes         &          No         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &         Yes         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         &       15963         &       15931         &       15931         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors clustered at county level in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/MAIN_All_Counties90_97_OmitNYDE_NYDE_Shops.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00791\sym{**} &      0.0100\sym{***}&                     \\
                    &   (0.00334)         &   (0.00373)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0100\sym{***}\\
                    &                     &                     &   (0.00373)         \\
\addlinespace
Forum Shopping to NYDE&                     &     -0.0126\sym{*}  &    -0.00252         \\
                    &                     &   (0.00659)         &   (0.00560)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_02_OmitNYDE_BRonlyFE_SHOCK.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Non-FS Bankruptcies &      0.0114\sym{**} &      0.0127\sym{**} &      0.0128\sym{**} &      0.0116\sym{**} &      0.0131\sym{**} &      0.0140\sym{***}\\
                    &   (0.00461)         &   (0.00501)         &   (0.00580)         &   (0.00541)         &   (0.00566)         &   (0.00512)         \\
\addlinespace
ln(County Population)&       1.105\sym{***}&       0.935\sym{***}&       0.893\sym{***}&       0.858\sym{***}&       0.918\sym{***}&       0.904\sym{***}\\
                    &    (0.0730)         &    (0.0743)         &    (0.0859)         &    (0.0868)         &    (0.0797)         &    (0.0785)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.335\sym{***}&       0.221\sym{***}&       0.223\sym{***}&       0.231\sym{***}&       0.219\sym{***}&       0.224\sym{***}\\
                    &    (0.0387)         &    (0.0444)         &    (0.0470)         &    (0.0483)         &    (0.0458)         &    (0.0453)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.973         &       0.974         &       0.975         &       0.975         &       0.974         &       0.974         \\
Observations        &       29877         &       29877         &       29877         &       29822         &       29877         &       29877         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors clustered at county level in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_INCLUDE_NYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00669\sym{**} &     0.00836\sym{**} &                     \\
                    &   (0.00308)         &   (0.00335)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00836\sym{**} \\
                    &                     &                     &   (0.00335)         \\
\addlinespace
Forum Shopping      &                     &    -0.00856         &   -0.000195         \\
                    &                     &   (0.00577)         &   (0.00529)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.985         &       0.985         &       0.985         \\
Observations        &       16314         &       16314         &       16314         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_ADJ.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00658\sym{*}  &     0.00889\sym{**} &                     \\
                    &   (0.00358)         &   (0.00399)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00889\sym{**} \\
                    &                     &                     &   (0.00399)         \\
\addlinespace
Forum Shopping      &                     &     -0.0109\sym{*}  &    -0.00206         \\
                    &                     &   (0.00633)         &   (0.00564)         \\
\addlinespace
Adjacent County Bankruptcies&    -0.00337         &    -0.00336         &    -0.00336         \\
                    &   (0.00358)         &   (0.00358)         &   (0.00358)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_BLS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00569\sym{**} &     0.00856\sym{***}&                     \\
                    &   (0.00282)         &   (0.00321)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00856\sym{***}\\
                    &                     &                     &   (0.00321)         \\
\addlinespace
Forum Shopping      &                     &     -0.0136\sym{***}&    -0.00508         \\
                    &                     &   (0.00496)         &   (0.00411)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.996         &       0.996         &       0.996         \\
Observations        &       10684         &       10684         &       10684         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_BRonlyFE_SHOCK.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Non-FS Bankruptcies &     0.00949\sym{***}&      0.0101\sym{***}&     0.00878\sym{**} &     0.00999\sym{***}&     0.00863\sym{**} &      0.0100\sym{***}\\
                    &   (0.00348)         &   (0.00354)         &   (0.00384)         &   (0.00375)         &   (0.00347)         &   (0.00356)         \\
\addlinespace
ln(County Population)&       0.797\sym{***}&       0.750\sym{***}&       0.726\sym{***}&       0.715\sym{***}&       0.651\sym{***}&       0.694\sym{***}\\
                    &     (0.115)         &     (0.125)         &     (0.137)         &     (0.144)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.182\sym{***}&       0.167\sym{***}&       0.167\sym{***}&       0.170\sym{***}&       0.174\sym{***}&       0.170\sym{***}\\
                    &    (0.0418)         &    (0.0468)         &    (0.0481)         &    (0.0489)         &    (0.0479)         &    (0.0474)         \\
\midrule
                    &                     &                     &                     &                     &                     &                     \\
Fixed Effects       &                     &                     &                     &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Year                &          No         &         Yes         &          No         &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &         Yes         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         &         Yes         &          No         &          No         \\
State-Year          &          No         &          No         &          No         &          No         &         Yes         &          No         \\
District-Year       &          No         &          No         &          No         &          No         &          No         &         Yes         \\
\midrule            &                     &                     &                     &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         &       15931         &       15963         &       15963         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors clustered at county level in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_CourtCounties.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00905\sym{*}  &     0.00929\sym{*}  &                     \\
                    &   (0.00477)         &   (0.00499)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00929\sym{*}  \\
                    &                     &                     &   (0.00499)         \\
\addlinespace
Forum Shopping      &                     &    -0.00150         &     0.00779         \\
                    &                     &   (0.00641)         &   (0.00683)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.999         &       0.999         &       0.999         \\
Observations        &         972         &         972         &         972         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_Dummies.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcy          &      0.0144\sym{*}  &      0.0179\sym{*}  &                     \\
                    &   (0.00866)         &    (0.0102)         &                     \\
\addlinespace
Non-FS Bankruptcy   &                     &                     &      0.0179\sym{*}  \\
                    &                     &                     &    (0.0102)         \\
\addlinespace
Forum Shop          &                     &     -0.0130         &     0.00493         \\
                    &                     &    (0.0104)         &   (0.00854)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15925         &       15925         &       15925         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_LAGS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00803\sym{**} &      0.0101\sym{***}&                     \\
                    &   (0.00329)         &   (0.00373)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0101\sym{***}\\
                    &                     &                     &   (0.00373)         \\
\addlinespace
Forum Shopping      &                     &    -0.00989         &    0.000218         \\
                    &                     &   (0.00652)         &   (0.00566)         \\
\addlinespace
L.ln(Emp Non-Legal) &       0.126\sym{***}&       0.126\sym{***}&       0.126\sym{***}\\
                    &    (0.0402)         &    (0.0402)         &    (0.0402)         \\
\addlinespace
L.ln(County Population)&       0.855\sym{***}&       0.855\sym{***}&       0.855\sym{***}\\
                    &     (0.149)         &     (0.149)         &     (0.149)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_PERCENT_EstabChange.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00794\sym{**} &      0.0104\sym{***}&                     \\
                    &   (0.00348)         &   (0.00384)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0104\sym{***}\\
                    &                     &                     &   (0.00384)         \\
\addlinespace
Forum Shopping      &                     &     -0.0119\sym{*}  &    -0.00148         \\
                    &                     &   (0.00642)         &   (0.00575)         \\
\addlinespace
ln(County Population)&       0.716\sym{***}&       0.716\sym{***}&       0.716\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.161\sym{***}&       0.161\sym{***}&       0.161\sym{***}\\
                    &    (0.0481)         &    (0.0481)         &    (0.0481)         \\
\addlinespace
\%$\Delta$(Non-Legal Establishments)&      0.0774         &      0.0774         &      0.0774         \\
                    &    (0.0722)         &    (0.0722)         &    (0.0722)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15925         &       15925         &       15925         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_UnempRate.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00758\sym{**} &     0.00998\sym{***}&                     \\
                    &   (0.00334)         &   (0.00372)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00998\sym{***}\\
                    &                     &                     &   (0.00372)         \\
\addlinespace
Forum Shopping      &                     &     -0.0114\sym{*}  &    -0.00144         \\
                    &                     &   (0.00642)         &   (0.00569)         \\
\addlinespace
ln(County Population)&       0.719\sym{***}&       0.719\sym{***}&       0.719\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.175\sym{***}&       0.175\sym{***}&       0.175\sym{***}\\
                    &    (0.0496)         &    (0.0496)         &    (0.0496)         \\
\addlinespace
Unemployment Rate   &     0.00274         &     0.00275         &     0.00275         \\
                    &   (0.00283)         &   (0.00283)         &   (0.00283)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00793\sym{***}&     0.00948\sym{***}&                     \\
                    &   (0.00280)         &   (0.00349)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00948\sym{***}\\
                    &                     &                     &   (0.00349)         \\
\addlinespace
Forum Shopping      &                     &    -0.00741         &     0.00206         \\
                    &                     &   (0.00518)         &   (0.00365)         \\
\addlinespace
ln(County Population)&       0.797\sym{***}&       0.797\sym{***}&       0.797\sym{***}\\
                    &     (0.115)         &     (0.115)         &     (0.115)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.181\sym{***}&       0.182\sym{***}&       0.182\sym{***}\\
                    &    (0.0418)         &    (0.0418)         &    (0.0418)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county_DisY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00768\sym{**} &      0.0100\sym{***}&                     \\
                    &   (0.00335)         &   (0.00373)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0100\sym{***}\\
                    &                     &                     &   (0.00373)         \\
\addlinespace
Forum Shopping      &                     &     -0.0111\sym{*}  &    -0.00108         \\
                    &                     &   (0.00637)         &   (0.00564)         \\
\addlinespace
ln(County Population)&       0.715\sym{***}&       0.715\sym{***}&       0.715\sym{***}\\
                    &     (0.144)         &     (0.144)         &     (0.144)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0489)         &    (0.0489)         &    (0.0489)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &         Yes         &         Yes         &         Yes         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county_DivY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00702\sym{**} &     0.00862\sym{**} &                     \\
                    &   (0.00283)         &   (0.00348)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00862\sym{**} \\
                    &                     &                     &   (0.00348)         \\
\addlinespace
Forum Shopping      &                     &    -0.00772         &    0.000906         \\
                    &                     &   (0.00527)         &   (0.00393)         \\
\addlinespace
ln(County Population)&       0.651\sym{***}&       0.651\sym{***}&       0.651\sym{***}\\
                    &     (0.134)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.174\sym{***}&       0.174\sym{***}&       0.174\sym{***}\\
                    &    (0.0479)         &    (0.0479)         &    (0.0479)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &         Yes         &         Yes         &         Yes         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county_RegY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00859\sym{***}&      0.0100\sym{***}&                     \\
                    &   (0.00284)         &   (0.00356)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0100\sym{***}\\
                    &                     &                     &   (0.00356)         \\
\addlinespace
Forum Shopping      &                     &    -0.00689         &     0.00314         \\
                    &                     &   (0.00522)         &   (0.00368)         \\
\addlinespace
ln(County Population)&       0.694\sym{***}&       0.694\sym{***}&       0.694\sym{***}\\
                    &     (0.134)         &     (0.134)         &     (0.134)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.170\sym{***}&       0.170\sym{***}&       0.170\sym{***}\\
                    &    (0.0474)         &    (0.0474)         &    (0.0474)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &         Yes         &         Yes         &         Yes         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county_SY.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00720\sym{**} &     0.00878\sym{**} &                     \\
                    &   (0.00330)         &   (0.00385)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00878\sym{**} \\
                    &                     &                     &   (0.00385)         \\
\addlinespace
Forum Shopping      &                     &    -0.00759         &     0.00118         \\
                    &                     &   (0.00623)         &   (0.00524)         \\
\addlinespace
ln(County Population)&       0.726\sym{***}&       0.726\sym{***}&       0.726\sym{***}\\
                    &     (0.137)         &     (0.137)         &     (0.137)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.167\sym{***}&       0.167\sym{***}&       0.167\sym{***}\\
                    &    (0.0481)         &    (0.0481)         &    (0.0481)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &          No         &          No         &          No         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &         Yes         &         Yes         &         Yes         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_97_OmitNYDE_county_year.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00830\sym{***}&      0.0101\sym{***}&                     \\
                    &   (0.00287)         &   (0.00355)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0101\sym{***}\\
                    &                     &                     &   (0.00355)         \\
\addlinespace
Forum Shopping      &                     &    -0.00873\sym{*}  &     0.00140         \\
                    &                     &   (0.00518)         &   (0.00373)         \\
\addlinespace
ln(County Population)&       0.750\sym{***}&       0.750\sym{***}&       0.750\sym{***}\\
                    &     (0.125)         &     (0.125)         &     (0.125)         \\
\addlinespace
ln(Emp Non-Legal)   &       0.166\sym{***}&       0.166\sym{***}&       0.166\sym{***}\\
                    &    (0.0468)         &    (0.0468)         &    (0.0468)         \\
\midrule
                    &                     &                     &                     \\
Fixed Effects       &                     &                     &                     \\
County              &         Yes         &         Yes         &         Yes         \\
Year                &         Yes         &         Yes         &         Yes         \\
Region-Year         &          No         &          No         &          No         \\
Division-Year       &          No         &          No         &          No         \\
State-Year          &          No         &          No         &          No         \\
District-Year       &          No         &          No         &          No         \\
\midrule            &                     &                     &                     \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties90_98_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00646\sym{*}  &     0.00966\sym{**} &                     \\
                    &   (0.00330)         &   (0.00377)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00966\sym{**} \\
                    &                     &                     &   (0.00377)         \\
\addlinespace
Forum Shopping      &                     &     -0.0151\sym{**} &    -0.00546         \\
                    &                     &   (0.00720)         &   (0.00615)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.982         &       0.982         &       0.982         \\
Observations        &       18606         &       18606         &       18606         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_All_Counties91_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00831\sym{**} &      0.0111\sym{**} &                     \\
                    &   (0.00410)         &   (0.00478)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0111\sym{**} \\
                    &                     &                     &   (0.00478)         \\
\addlinespace
Forum Shopping      &                     &     -0.0118\sym{*}  &   -0.000682         \\
                    &                     &   (0.00702)         &   (0.00583)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.986         &       0.986         &       0.986         \\
Observations        &       13327         &       13327         &       13327         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_BR_Counties90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &      0.0113\sym{**} &      0.0145\sym{***}&                     \\
                    &   (0.00468)         &   (0.00542)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &      0.0145\sym{***}\\
                    &                     &                     &   (0.00542)         \\
\addlinespace
Forum Shopping      &                     &     -0.0125         &     0.00199         \\
                    &                     &   (0.00825)         &   (0.00743)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.999         &       0.999         &       0.999         \\
Observations        &         354         &         354         &         354         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_Dummy_ValueWeight_BLS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
                    &\multicolumn{2}{c}{\textbf{Binary}}        &\multicolumn{2}{c}{\textbf{Value Weighted}}&\multicolumn{2}{c}{\textbf{BLS Data}}      \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}\\
\midrule
Bankruptcy          &      0.0141         &      0.0174\sym{*}  &                     &                     &                     &                     \\
                    &   (0.00862)         &    (0.0101)         &                     &                     &                     &                     \\
\addlinespace
Forum Shop          &                     &     -0.0121         &                     &                     &                     &                     \\
                    &                     &    (0.0102)         &                     &                     &                     &                     \\
\addlinespace
BR Firm's Assets    &                     &                     &     0.00219\sym{**} &     0.00281\sym{**} &                     &                     \\
                    &                     &                     &   (0.00103)         &   (0.00132)         &                     &                     \\
\addlinespace
FS Firm's Assets    &                     &                     &                     &    -0.00198         &                     &                     \\
                    &                     &                     &                     &   (0.00204)         &                     &                     \\
\addlinespace
Bankruptcies        &                     &                     &                     &                     &     0.00569\sym{**} &     0.00856\sym{***}\\
                    &                     &                     &                     &                     &   (0.00282)         &   (0.00321)         \\
\addlinespace
Forum Shopping      &                     &                     &                     &                     &                     &     -0.0136\sym{***}\\
                    &                     &                     &                     &                     &                     &   (0.00496)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.996         &       0.996         \\
Observations        &       15931         &       15931         &       15931         &       15931         &       10684         &       10684         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_Dummy_ValueWeight_BLS_Adj.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{8}{c}}
\toprule
                    &\multicolumn{2}{c}{\textbf{Binary}}        &\multicolumn{2}{c}{\textbf{Value Weighted}}&\multicolumn{2}{c}{\textbf{BLS Data}}      &\multicolumn{2}{c}{\textbf{Spillover}}     \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}\\
\midrule
Bankruptcy          &      0.0141         &      0.0174\sym{*}  &                     &                     &                     &                     &                     &                     \\
                    &   (0.00862)         &    (0.0101)         &                     &                     &                     &                     &                     &                     \\
\addlinespace
Forum Shop          &                     &     -0.0121         &                     &                     &                     &                     &                     &                     \\
                    &                     &    (0.0102)         &                     &                     &                     &                     &                     &                     \\
\addlinespace
BR Firm's Assets (2021 dollars)&                     &                     &     0.00219\sym{**} &     0.00281\sym{**} &                     &                     &                     &                     \\
                    &                     &                     &   (0.00103)         &   (0.00132)         &                     &                     &                     &                     \\
\addlinespace
FS Firm's Assets (2021 dollars)&                     &                     &                     &    -0.00198         &                     &                     &                     &                     \\
                    &                     &                     &                     &   (0.00204)         &                     &                     &                     &                     \\
\addlinespace
Bankruptcies        &                     &                     &                     &                     &     0.00569\sym{**} &     0.00856\sym{***}&     0.00658\sym{*}  &     0.00889\sym{**} \\
                    &                     &                     &                     &                     &   (0.00282)         &   (0.00321)         &   (0.00358)         &   (0.00399)         \\
\addlinespace
Forum Shopping      &                     &                     &                     &                     &                     &     -0.0136\sym{***}&                     &     -0.0109\sym{*}  \\
                    &                     &                     &                     &                     &                     &   (0.00496)         &                     &   (0.00633)         \\
\addlinespace
Adjacent County Bankruptcies&                     &                     &                     &                     &                     &                     &    -0.00337         &    -0.00336         \\
                    &                     &                     &                     &                     &                     &                     &   (0.00358)         &   (0.00358)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.996         &       0.996         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         &       15931         &       10684         &       10684         &       15931         &       15931         \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/RBST_HQ_Counties90_97_OmitNYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Bankruptcies        &     0.00563\sym{*}  &     0.00845\sym{**} &                     \\
                    &   (0.00319)         &   (0.00377)         &                     \\
\addlinespace
Non-FS Bankruptcies &                     &                     &     0.00845\sym{**} \\
                    &                     &                     &   (0.00377)         \\
\addlinespace
Forum Shopping      &                     &     -0.0134\sym{*}  &    -0.00498         \\
                    &                     &   (0.00708)         &   (0.00592)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.994         &       0.994         &       0.994         \\
Observations        &        5533         &        5533         &        5533         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/New_Layout/test.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{8}{c}}
\toprule
                    &\multicolumn{2}{c}{\textbf{Binary}}        &\multicolumn{2}{c}{\textbf{Value Weighted}}&\multicolumn{2}{c}{\textbf{Value Weighted}}&\multicolumn{2}{c}{\textbf{Spillover}}     \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}&\multicolumn{1}{c}{ln\_LegEmp\_BLS}&\multicolumn{1}{c}{ln(LegEmp)}&\multicolumn{1}{c}{ln(LegEmp)}\\
\midrule
Bankruptcy          &      0.0141         &      0.0174\sym{*}  &                     &                     &                     &                     &                     &                     \\
                    &   (0.00862)         &    (0.0101)         &                     &                     &                     &                     &                     &                     \\
\addlinespace
Forum Shop          &                     &     -0.0121         &                     &                     &                     &                     &                     &                     \\
                    &                     &    (0.0102)         &                     &                     &                     &                     &                     &                     \\
\addlinespace
BR Firm's Assets (2021 dollars)&                     &                     &     0.00219\sym{**} &     0.00281\sym{**} &                     &                     &                     &                     \\
                    &                     &                     &   (0.00103)         &   (0.00132)         &                     &                     &                     &                     \\
\addlinespace
FS Firm's Assets (2021 dollars)&                     &                     &                     &    -0.00198         &                     &                     &                     &                     \\
                    &                     &                     &                     &   (0.00204)         &                     &                     &                     &                     \\
\addlinespace
Bankruptcies        &                     &                     &                     &                     &     0.00569\sym{**} &     0.00856\sym{***}&     0.00658\sym{*}  &     0.00889\sym{**} \\
                    &                     &                     &                     &                     &   (0.00282)         &   (0.00321)         &   (0.00358)         &   (0.00399)         \\
\addlinespace
Forum Shopping      &                     &                     &                     &                     &                     &     -0.0136\sym{***}&                     &     -0.0109\sym{*}  \\
                    &                     &                     &                     &                     &                     &   (0.00496)         &                     &   (0.00633)         \\
\addlinespace
Adjacent County Bankruptcies&                     &                     &                     &                     &                     &                     &    -0.00337         &    -0.00336         \\
                    &                     &                     &                     &                     &                     &                     &   (0.00358)         &   (0.00358)         \\
\midrule
County FE           &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
District-Year FE    &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
R-Squared           &       0.984         &       0.984         &       0.984         &       0.984         &       0.996         &       0.996         &       0.984         &       0.984         \\
Observations        &       15931         &       15931         &       15931         &       15931         &       10684         &       10684         &       15931         &       15931         \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/Old/DepVar_exogeneity_reg.tex <==
\begin{tabular}{lcc} \hline
 & (1) & (2) \\
VARIABLES & Dependent Variable: n\_BR & Dependent Variable: n\_FS \\ \hline
 &  &  \\
ln(EmpNoLegal) & 0.0214*** & 0.00424 \\
 & (0.00800) & (0.00529) \\
ln(county\_pop) & 0.0905* & 0.0290 \\
 & (0.0504) & (0.0314) \\
Constant & -1.061** & -0.319 \\
 & (0.522) & (0.329) \\
 &  &  \\
Observations & 18,425 & 18,425 \\
R-squared & 0.762 & 0.665 \\
Fixed Effects & county SY & county SY \\
 SE-Cluster & county & county \\ \hline
\multicolumn{3}{c}{ Robust standard errors in parentheses} \\
\multicolumn{3}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{3}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/MAIN_All_Counties90_97_OmitNYDE.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00658** & 0.00938** & 0.00958** \\
 & (0.00324) & (0.00385) & (0.00388) \\
n\_FS &  & -0.0130** &  \\
 &  & (0.00635) &  \\
n\_FS\_LP &  &  & -0.0167** \\
 &  &  & (0.00701) \\
n\_FS\_CS &  &  & -0.00730 \\
 &  &  & (0.00972) \\
ln(county\_pop) & 0.726*** & 0.726*** & 0.726*** \\
 & (0.137) & (0.137) & (0.137) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0481) & (0.0481) & (0.0481) \\
Constant & -5.282*** & -5.284*** & -5.285*** \\
 & (1.358) & (1.358) & (1.358) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00658 & -0.00365 & -0.00715 \\
t-stat & 2.034 & -0.690 & -1.318 \\
 p-val & 0.0421 & 0.490 & 0.187 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/MAIN_All_Counties90_97_OmitNYDE_TEST.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{BR only}&\multicolumn{1}{c}{BR and FS}&\multicolumn{1}{c}{FS split}\\
\midrule
n\_BR                &     0.00720\sym{**} &     0.00949\sym{**} &     0.00987\sym{**} \\
                    &   (0.00330)         &   (0.00391)         &   (0.00396)         \\
\addlinespace
n\_FS                &                     &     -0.0104\sym{*}  &                     \\
                    &                     &   (0.00616)         &                     \\
\addlinespace
n\_FS\_LP             &                     &                     &     -0.0168\sym{**} \\
                    &                     &                     &   (0.00740)         \\
\addlinespace
n\_FS\_CS             &                     &                     &    -0.00239         \\
                    &                     &                     &   (0.00827)         \\
\midrule
Linear Combination  &        n\_BR         & n\_BR + n\_FS         &n\_BR + n\_FS\_LP         \\
Estimate            &     0.00720         &   -0.000879         &    -0.00688         \\
P-value             &      0.0292         &       0.863         &       0.225         \\
\hline              &                     &                     &                     \\
Fixed Effexts       &   county SY         &   county SY         &   county SY         \\
R-Squared           &       0.984         &       0.984         &       0.984         \\
Observations        &       15963         &       15963         &       15963         \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize Standard errors clustered at county level}\\
\multicolumn{4}{l}{\footnotesize SAMPLE: 1991 through 1996 omit NY and DE}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Regressions/Old/MAIN_All_Counties90_97_OmitNYDE_WAGE.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & BR only & BR and FS & FS split & BR FS split \\ \hline
 &  &  &  &  \\
n\_BR & 1.26e-05 & -0.00223 & -0.00244 &  \\
 & (0.00253) & (0.00269) & (0.00271) &  \\
n\_BR\_LP &  &  &  & -0.0148** \\
 &  &  &  & (0.00638) \\
n\_br\_CS &  &  &  & 0.00179 \\
 &  &  &  & (0.00329) \\
n\_FS &  & 0.0104* &  &  \\
 &  & (0.00606) &  &  \\
n\_FS\_LP &  &  & 0.0142* & 0.0269** \\
 &  &  & (0.00836) & (0.0105) \\
n\_FS\_CS &  &  & 0.00452 & -0.000569 \\
 &  &  & (0.00597) & (0.00625) \\
ln(county\_pop) & -0.0196 & -0.0198 & -0.0198 & -0.0191 \\
 & (0.0814) & (0.0814) & (0.0814) & (0.0814) \\
ln(EmpNoLegal) & 0.0461 & 0.0462 & 0.0459 & 0.0460 \\
 & (0.0284) & (0.0284) & (0.0284) & (0.0284) \\
Constant & 9.845*** & 9.847*** & 9.849*** & 9.841*** \\
 & (0.821) & (0.821) & (0.821) & (0.821) \\
 &  &  &  &  \\
Observations & 10,702 & 10,702 & 10,702 & 10,702 \\
R-squared & 0.930 & 0.930 & 0.930 & 0.930 \\
Fixed Effects & county SY & county SY & county SY & county SY \\
SE-Cluster & county & county & county & county \\
----- & ----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP & n\_BR\_LP + n\_FS\_LP \\
joint & 1.26e-05 & 0.00819 & 0.0118 & 0.0121 \\
t-stat & 0.00498 & 1.499 & 1.558 & 1.588 \\
 p-val & 0.996 & 0.134 & 0.119 & 0.112 \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{5}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/MAIN_All_Counties90_97_OmitNYDE_avgefct.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00658** & 0.00938** & 0.00958** \\
 & (0.00324) & (0.00385) & (0.00388) \\
n\_FS &  & -0.0130** &  \\
 &  & (0.00635) &  \\
n\_FS\_LP &  &  & -0.0167** \\
 &  &  & (0.00701) \\
n\_FS\_CS &  &  & -0.00730 \\
 &  &  & (0.00972) \\
ln(county\_pop) & 0.726*** & 0.726*** & 0.726*** \\
 & (0.137) & (0.137) & (0.137) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0481) & (0.0481) & (0.0481) \\
Constant & -5.282*** & -5.284*** & -5.285*** \\
 & (1.358) & (1.358) & (1.358) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR and n\_FS & n\_BR and n\_FS\_LP \\
joint & 0.0112 & 0.00947 & 0.0107 \\
t-stat & 2.034 & 1.731 & 1.976 \\
 p-val & 0.0421 & 0.0835 & 0.0482 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/MAIN_All_Counties96_02_OmitNYDE.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.0137*** & 0.00474 & 0.00474 \\
 & (0.00415) & (0.00523) & (0.00523) \\
n\_FS &  & 0.0208** &  \\
 &  & (0.00918) &  \\
n\_FS\_LP &  &  & 0.0208** \\
 &  &  & (0.00918) \\
ln(county\_pop) & 0.449*** & 0.448*** & 0.448*** \\
 & (0.133) & (0.133) & (0.133) \\
ln(EmpNoLegal) & 0.119 & 0.119 & 0.119 \\
 & (0.0783) & (0.0783) & (0.0783) \\
n\_FS\_CS = o, &  &  & - \\
 &  &  &  \\
Constant & -1.996 & -1.984 & -1.984 \\
 & (1.351) & (1.351) & (1.351) \\
 &  &  &  \\
Observations & 13,317 & 13,317 & 13,317 \\
R-squared & 0.978 & 0.978 & 0.978 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.0137 & 0.0256 & 0.0256 \\
t-stat & 3.298 & 3.542 & 3.542 \\
 p-val & 0.000985 & 0.000403 & 0.000403 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1997 through 2001 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_NYDE_Interact.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00660** & 0.00940** & 0.00960** \\
 & (0.00324) & (0.00385) & (0.00389) \\
n\_BR x NYDE & 0.00494 & 0.00481 & 0.00444 \\
 & (0.00767) & (0.00767) & (0.00807) \\
n\_FS &  & -0.0130** &  \\
 &  & (0.00635) &  \\
n\_FS x NYDE &  & 0.00353 &  \\
 &  & (0.00916) &  \\
n\_FS\_LP &  &  & -0.0167** \\
 &  &  & (0.00702) \\
n\_FS\_LP x NYDE &  &  & -0.000442 \\
 &  &  & (0.0172) \\
n\_FS\_CS &  &  & -0.00731 \\
 &  &  & (0.00972) \\
n\_FS\_CS x NYDE &  &  & 0.00932 \\
 &  &  & (0.0204) \\
ln(EmpNoLegal) & 0.166*** & 0.166*** & 0.166*** \\
 & (0.0478) & (0.0478) & (0.0478) \\
ln(county\_pop) & 0.721*** & 0.721*** & 0.721*** \\
 & (0.137) & (0.137) & (0.137) \\
Constant & -5.213*** & -5.215*** & -5.215*** \\
 & (1.357) & (1.357) & (1.357) \\
 &  &  &  \\
Observations & 16,346 & 16,346 & 16,346 \\
R-squared & 0.985 & 0.985 & 0.985 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.0115 & -0.00363 & -0.00712 \\
t-stat & 1.388 & -0.686 & -1.313 \\
 p-val & 0.165 & 0.493 & 0.189 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996} \\
\multicolumn{4}{c}{ NY and DE included with interaction terms.} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_ADJ.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00553 & 0.00829** & 0.00849** \\
 & (0.00337) & (0.00396) & (0.00400) \\
n\_Ch11\_adj & -0.00424 & -0.00422 & -0.00421 \\
 & (0.00340) & (0.00340) & (0.00340) \\
n\_FS &  & -0.0128** &  \\
 &  & (0.00631) &  \\
n\_FS\_LP &  &  & -0.0165** \\
 &  &  & (0.00703) \\
n\_FS\_CS &  &  & -0.00718 \\
 &  &  & (0.00966) \\
ln(county\_pop) & 0.722*** & 0.722*** & 0.722*** \\
 & (0.137) & (0.137) & (0.137) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0482) & (0.0482) & (0.0482) \\
Constant & -5.245*** & -5.247*** & -5.247*** \\
 & (1.358) & (1.358) & (1.358) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00553 & -0.00452 & -0.00797 \\
t-stat & 1.640 & -0.841 & -1.415 \\
 p-val & 0.101 & 0.401 & 0.157 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_Dummies.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
BR & 0.0143* & 0.0199** & 0.0199** \\
 & (0.00828) & (0.0100) & (0.01000) \\
FS &  & -0.0181* &  \\
 &  & (0.00957) &  \\
FS\_LP &  &  & -0.0222** \\
 &  &  & (0.0109) \\
FS\_CS &  &  & -0.0122 \\
 &  &  & (0.0116) \\
ln(county\_pop) & 0.726*** & 0.726*** & 0.726*** \\
 & (0.137) & (0.137) & (0.137) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0481) & (0.0481) & (0.0481) \\
Constant & -5.282*** & -5.284*** & -5.285*** \\
 & (1.358) & (1.358) & (1.358) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & BR & BR + FS & BR + FS\_LP \\
joint & 0.0143 & 0.00178 & -0.00222 \\
t-stat & 1.732 & 0.234 & -0.241 \\
 p-val & 0.0834 & 0.815 & 0.810 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\multicolumn{4}{c}{ Dummy variables instead of Level.} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_LAGS.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00730** & 0.00991*** & 0.0101*** \\
 & (0.00316) & (0.00376) & (0.00380) \\
n\_FS &  & -0.0122* &  \\
 &  & (0.00638) &  \\
n\_FS\_LP &  &  & -0.0154** \\
 &  &  & (0.00701) \\
n\_FS\_CS &  &  & -0.00715 \\
 &  &  & (0.00972) \\
ln(EmpNoLegal) = L, & 0.120*** & 0.120*** & 0.120*** \\
 & (0.0398) & (0.0398) & (0.0398) \\
ln(county\_pop) = L, & 0.867*** & 0.867*** & 0.867*** \\
 & (0.142) & (0.142) & (0.142) \\
Constant & -6.307*** & -6.308*** & -6.308*** \\
 & (1.404) & (1.404) & (1.404) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00730 & -0.00225 & -0.00531 \\
t-stat & 2.309 & -0.420 & -0.962 \\
 p-val & 0.0210 & 0.675 & 0.336 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_county.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00800*** & 0.0107*** & 0.0108*** \\
 & (0.00281) & (0.00352) & (0.00355) \\
n\_FS &  & -0.0127*** &  \\
 &  & (0.00485) &  \\
n\_FS\_LP &  &  & -0.0140** \\
 &  &  & (0.00579) \\
n\_FS\_CS &  &  & -0.0106 \\
 &  &  & (0.00661) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0463) & (0.0463) & (0.0464) \\
ln(county\_pop) & 0.742*** & 0.743*** & 0.743*** \\
 & (0.126) & (0.126) & (0.126) \\
ln(StateGDP) & 0.0508 & 0.0508 & 0.0508 \\
 & (0.0487) & (0.0487) & (0.0487) \\
Constant & -6.065*** & -6.069*** & -6.068*** \\
 & (1.030) & (1.030) & (1.030) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county & county & county \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00800 & -0.00191 & -0.00316 \\
t-stat & 2.848 & -0.560 & -0.785 \\
 p-val & 0.00443 & 0.575 & 0.432 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_county_DisY.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00724** & 0.0107*** & 0.0108*** \\
 & (0.00332) & (0.00379) & (0.00380) \\
n\_FS &  & -0.0156** &  \\
 &  & (0.00624) &  \\
n\_FS\_LP &  &  & -0.0182** \\
 &  &  & (0.00739) \\
n\_FS\_CS &  &  & -0.0116 \\
 &  &  & (0.0100) \\
ln(EmpNoLegal) & 0.170*** & 0.170*** & 0.170*** \\
 & (0.0489) & (0.0489) & (0.0489) \\
ln(county\_pop) & 0.715*** & 0.715*** & 0.715*** \\
 & (0.144) & (0.144) & (0.144) \\
ln(StateGDP) = o, & - & - & - \\
 &  &  &  \\
Constant & -5.193*** & -5.195*** & -5.196*** \\
 & (1.433) & (1.433) & (1.433) \\
 &  &  &  \\
Observations & 15,931 & 15,931 & 15,931 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county DisY & county DisY & county DisY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00724 & -0.00496 & -0.00737 \\
t-stat & 2.183 & -0.935 & -1.190 \\
 p-val & 0.0291 & 0.350 & 0.234 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_county_RegY.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00816*** & 0.0106*** & 0.0106*** \\
 & (0.00281) & (0.00355) & (0.00357) \\
n\_FS &  & -0.0113** &  \\
 &  & (0.00509) &  \\
n\_FS\_LP &  &  & -0.0115* \\
 &  &  & (0.00594) \\
n\_FS\_CS &  &  & -0.0109 \\
 &  &  & (0.00713) \\
ln(EmpNoLegal) & 0.170*** & 0.170*** & 0.170*** \\
 & (0.0476) & (0.0476) & (0.0476) \\
ln(county\_pop) & 0.692*** & 0.692*** & 0.692*** \\
 & (0.134) & (0.134) & (0.134) \\
ln(StateGDP) & 0.00931 & 0.00815 & 0.00816 \\
 & (0.108) & (0.108) & (0.108) \\
Constant & -5.072*** & -5.058*** & -5.058*** \\
 & (1.744) & (1.744) & (1.744) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county RegY & county RegY & county RegY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00816 & -0.000684 & -0.000904 \\
t-stat & 2.899 & -0.186 & -0.203 \\
 p-val & 0.00378 & 0.853 & 0.839 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_county_SY.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00658** & 0.00938** & 0.00958** \\
 & (0.00324) & (0.00385) & (0.00388) \\
n\_FS &  & -0.0130** &  \\
 &  & (0.00635) &  \\
n\_FS\_LP &  &  & -0.0167** \\
 &  &  & (0.00701) \\
n\_FS\_CS &  &  & -0.00730 \\
 &  &  & (0.00972) \\
ln(EmpNoLegal) & 0.167*** & 0.167*** & 0.167*** \\
 & (0.0481) & (0.0481) & (0.0481) \\
ln(county\_pop) & 0.726*** & 0.726*** & 0.726*** \\
 & (0.137) & (0.137) & (0.137) \\
ln(StateGDP) = o, & - & - & - \\
 &  &  &  \\
Constant & -5.282*** & -5.284*** & -5.285*** \\
 & (1.358) & (1.358) & (1.358) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00658 & -0.00365 & -0.00715 \\
t-stat & 2.034 & -0.690 & -1.318 \\
 p-val & 0.0421 & 0.490 & 0.187 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties90_97_OmitNYDE_county_year.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00782*** & 0.0108*** & 0.0109*** \\
 & (0.00284) & (0.00354) & (0.00357) \\
n\_FS &  & -0.0139*** &  \\
 &  & (0.00490) &  \\
n\_FS\_LP &  &  & -0.0151*** \\
 &  &  & (0.00567) \\
n\_FS\_CS &  &  & -0.0120* \\
 &  &  & (0.00686) \\
ln(EmpNoLegal) & 0.166*** & 0.166*** & 0.166*** \\
 & (0.0470) & (0.0470) & (0.0470) \\
ln(county\_pop) & 0.739*** & 0.739*** & 0.739*** \\
 & (0.126) & (0.126) & (0.126) \\
ln(StateGDP) & 0.0482 & 0.0471 & 0.0471 \\
 & (0.102) & (0.102) & (0.102) \\
Constant & -5.988*** & -5.977*** & -5.978*** \\
 & (1.587) & (1.587) & (1.587) \\
 &  &  &  \\
Observations & 15,963 & 15,963 & 15,963 \\
R-squared & 0.984 & 0.984 & 0.984 \\
Fixed Effects & county year & county year & county year \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00782 & -0.00306 & -0.00419 \\
t-stat & 2.756 & -0.856 & -1.040 \\
 p-val & 0.00588 & 0.392 & 0.298 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties91_97_OmitNYDE.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00839** & 0.0117*** & 0.0119*** \\
 & (0.00389) & (0.00451) & (0.00452) \\
n\_FS &  & -0.0141** &  \\
 &  & (0.00655) &  \\
n\_FS\_LP &  &  & -0.0205*** \\
 &  &  & (0.00760) \\
n\_FS\_CS &  &  & -0.00400 \\
 &  &  & (0.00902) \\
ln(county\_pop) & 0.671*** & 0.671*** & 0.671*** \\
 & (0.156) & (0.156) & (0.156) \\
ln(EmpNoLegal) & 0.203*** & 0.203*** & 0.203*** \\
 & (0.0602) & (0.0603) & (0.0603) \\
Constant & -5.040*** & -5.041*** & -5.044*** \\
 & (1.542) & (1.542) & (1.542) \\
 &  &  &  \\
Observations & 13,354 & 13,354 & 13,354 \\
R-squared & 0.986 & 0.986 & 0.986 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00839 & -0.00234 & -0.00861 \\
t-stat & 2.155 & -0.434 & -1.473 \\
 p-val & 0.0312 & 0.665 & 0.141 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1992 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_All_Counties91_97_OmitNYDE_WAGE.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & BR only & BR and FS & FS split & BR FS split \\ \hline
 &  &  &  &  \\
n\_BR & 0.00140 & -0.00138 & -0.00157 &  \\
 & (0.00301) & (0.00331) & (0.00332) &  \\
n\_BR\_LP &  &  &  & -0.0161** \\
 &  &  &  & (0.00681) \\
(sum) n\_br\_CS &  &  &  & 0.00363 \\
 &  &  &  & (0.00404) \\
n\_FS &  & 0.0117* &  &  \\
 &  & (0.00705) &  &  \\
n\_FS\_LP &  &  & 0.0175* & 0.0330*** \\
 &  &  & (0.00945) & (0.0120) \\
n\_FS\_CS &  &  & 0.00274 & -0.00282 \\
 &  &  & (0.00698) & (0.00731) \\
ln(county\_pop) & -0.0612 & -0.0610 & -0.0615 & -0.0606 \\
 & (0.0965) & (0.0965) & (0.0965) & (0.0965) \\
ln(EmpNoLegal) & 0.0662** & 0.0658** & 0.0657** & 0.0657** \\
 & (0.0316) & (0.0316) & (0.0316) & (0.0316) \\
Constant & 10.12*** & 10.12*** & 10.13*** & 10.12*** \\
 & (0.998) & (0.998) & (0.998) & (0.998) \\
 &  &  &  &  \\
Observations & 8,919 & 8,919 & 8,919 & 8,919 \\
R-squared & 0.938 & 0.938 & 0.938 & 0.938 \\
Fixed Effects & county SY & county SY & county SY & county SY \\
SE-Cluster & county & county & county & county \\
----- & ----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP & n\_BR\_LP + n\_FS\_LP \\
joint & 0.00140 & 0.0103 & 0.0159 & 0.0169 \\
t-stat & 0.465 & 1.655 & 1.843 & 1.946 \\
 p-val & 0.642 & 0.0980 & 0.0655 & 0.0518 \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{5}{c}{ SAMPLE: 1992 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/RBST_HQ_Counties91_97_OmitNYDE.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & BR only & BR and FS & FS split \\ \hline
 &  &  &  \\
n\_BR & 0.00675** & 0.00922** & 0.00947** \\
 & (0.00318) & (0.00379) & (0.00383) \\
n\_FS &  & -0.0115* &  \\
 &  & (0.00610) &  \\
n\_FS\_LP &  &  & -0.0161** \\
 &  &  & (0.00654) \\
n\_FS\_CS &  &  & -0.00437 \\
 &  &  & (0.00985) \\
ln(county\_pop) & 0.929*** & 0.930*** & 0.929*** \\
 & (0.178) & (0.178) & (0.178) \\
ln(EmpNoLegal) & 0.250** & 0.249** & 0.250** \\
 & (0.105) & (0.105) & (0.105) \\
Constant & -8.053*** & -8.055*** & -8.058*** \\
 & (1.697) & (1.698) & (1.699) \\
 &  &  &  \\
Observations & 5,533 & 5,533 & 5,533 \\
R-squared & 0.994 & 0.994 & 0.994 \\
Fixed Effects & county SY & county SY & county SY \\
SE-Cluster & county & county & county \\
----- & ----- & ----- & ----- \\
LinCom & n\_BR & n\_BR + n\_FS & n\_BR + n\_FS\_LP \\
joint & 0.00675 & -0.00231 & -0.00667 \\
t-stat & 2.124 & -0.459 & -1.352 \\
 p-val & 0.0339 & 0.646 & 0.177 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1992-1996; omit NY and DE; Only counties with HQ at any point from 1980-97} \\
\end{tabular}


==> Regressions/Old/control_exogeneity_reg.tex <==
\begin{tabular}{lcc} \hline
 & (1) & (2) \\
VARIABLES & Dependent Variable: ln\_cnty\_pop & Dependent Variable: ln\_EmpNoLegal \\ \hline
 &  &  \\
n\_BR & 0.00117 & 0.00443*** \\
 & (0.000921) & (0.00143) \\
n\_FS & 0.000859 &  \\
 & (0.00255) &  \\
n\_FS\_LP &  & 0.00587 \\
 &  & (0.00491) \\
n\_FS\_CS &  & -0.0102 \\
 &  & (0.0102) \\
ln(county\_pop) &  & 0.985*** \\
 &  & (0.0683) \\
ln(EmpNoLegal) & 0.0674*** &  \\
 & (0.00649) &  \\
Constant & 9.546*** & -1.312* \\
 & (0.0562) & (0.692) \\
 &  &  \\
Observations & 18,425 & 18,425 \\
R-squared & 1.000 & 0.998 \\
Fixed Effects & county SY & county SY \\
 SE-Cluster & county & county \\ \hline
\multicolumn{3}{c}{ Robust standard errors in parentheses} \\
\multicolumn{3}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{3}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Regressions/Old/nBR_exogeneity_reg.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & Lag=1 & Lag=2 & Lag=3 \\ \hline
 &  &  &  \\
ln(EmpNoLegal) = L, & 0.0246*** &  &  \\
 & (0.00915) &  &  \\
ln(county\_pop) = L, & 0.0453 &  &  \\
 & (0.0623) &  &  \\
ln(unemp rate) = L, & -0.00241 &  &  \\
 & (0.00999) &  &  \\
ln(EmpNoLegal) = L, &  & 0.0143* &  \\
 &  & (0.00808) &  \\
ln(county\_pop) = L, &  & 0.0109 &  \\
 &  & (0.0746) &  \\
ln(unemp rate) = L, &  & -0.0167* &  \\
 &  & (0.00945) &  \\
ln(EmpNoLegal) = L, &  &  & -0.00340 \\
 &  &  & (0.00804) \\
ln(county\_pop) = L, &  &  & 0.0639 \\
 &  &  & (0.0860) \\
ln(unemp rate) = L, &  &  & -0.00210 \\
 &  &  & (0.00776) \\
Constant & -0.625 & -0.165 & -0.578 \\
 & (0.622) & (0.765) & (0.883) \\
 &  &  &  \\
Observations & 18,394 & 15,327 & 12,261 \\
R-squared & 0.762 & 0.783 & 0.801 \\
Fixed Effects & county SY & county SY & county SY \\
 SE-Cluster & county & county & county \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\multicolumn{4}{c}{ SAMPLE: 1991 through 1996 omit NY and DE} \\
\end{tabular}


==> Summary_Stats/DescriptiveStats.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{cc}}
\toprule
                    &\multicolumn{2}{c}{\textbf{Full Sample}}&\multicolumn{2}{c}{\textbf{County-Year with BR}}\\
                    &        Mean&   Std. Dev.&        Mean&   Std. Dev.\\
\midrule
Legal Emp           &     265.720&    1553.482&    5029.190&    7761.030\\
\addlinespace
Legal Avg Wage      &   25611.479&   10367.845&   41602.706&    9811.927\\
\addlinespace
Bankruptcies        &       0.042&       0.371&       1.703&       1.673\\
\addlinespace
Forum Shopping      &       0.011&       0.145&       0.470&       0.800\\
\addlinespace
Forum Shopping (LP) &       0.007&       0.112&       0.286&       0.660\\
\addlinespace
Forum Shopping (CS) &       0.004&       0.082&       0.184&       0.489\\
\midrule
Observations        &       18450&            &         451&            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/avg_nfile_nfs.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccc}}
\toprule
                    &        mean&         max&       total\\
\midrule
n\_BR                &    1.702882&          14&         768\\
n\_FS                &    .5166297&           6&         233\\
n\_FS\_LP             &    .3325942&           6&         150\\
n\_FS\_CS             &    .1840355&           4&          83\\
\midrule
Observations        &         451&            &            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/avg_nfile_nfs2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\toprule
                    &        mean&          sd&         max&       total\\
\midrule
bankruptcies        &       1.703&       1.673&      14.000&     768.000\\
forum shopping      &       0.517&       0.806&       6.000&     233.000\\
forum shopping (LP) &       0.333&       0.680&       6.000&     150.000\\
forum shopping (CS) &       0.184&       0.489&       4.000&      83.000\\
\midrule
Observations        &         451&            &            &            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/avg_nfile_nfs_bronly.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\toprule
                    &        Mean&   Std. Dev.&         Max&       Total\\
\midrule
Legal Emp           &    5029.190&    7761.030&       56187&     2253077\\
Legal Avg Wage      &   41602.706&    9811.927&       65443&    18554807\\
Bankruptcies        &       1.703&       1.673&          14&         768\\
Forum Shopping      &       0.470&       0.800&           6&         212\\
Forum Shopping (LP) &       0.286&       0.660&           6&         129\\
Forum Shopping (CS) &       0.184&       0.489&           4&          83\\
\midrule
Observations        &         451&            &            &            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/avg_nfile_nfs_regsamp.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\toprule
                    &        Mean&   Std. Dev.&         Max&       Total\\
\midrule
Legal Emp           &     265.720&    1553.482&       56187&     4899344\\
Legal Avg Wage      &   25611.479&   10367.845&      157940&   274247722\\
Bankruptcies        &       0.042&       0.371&          14&         768\\
Forum Shopping      &       0.011&       0.145&           6&         212\\
Forum Shopping (LP) &       0.007&       0.112&           6&         129\\
Forum Shopping (CS) &       0.004&       0.082&           4&          83\\
\midrule
Observations        &       18450&            &            &            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/avg_nfile_nfs_regsamp_NYDE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\toprule
                    &        Mean&   Std. Dev.&         Max&       Total\\
\midrule
Legal Emp           &     295.265&    1929.912&       67896&     5559255\\
Legal Avg Wage      &   25591.525&   10342.464&      157940&   283707651\\
Bankruptcies        &       0.046&       0.414&          14&         868\\
Forum Shopping      &       0.012&       0.148&           6&         232\\
Forum Shopping (LP) &       0.007&       0.114&           6&         139\\
Forum Shopping (CS) &       0.005&       0.085&           4&          93\\
\midrule
Observations        &       18840&            &            &            \\
\bottomrule
\end{tabular}
}


==> Summary_Stats/gen_sumstats.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &           N&        mean&          sd&         min&         max\\
\midrule
Legal Emp           &       16052&     305.217&    1661.322&           1&       56187\\
Legal Avg Wage      &       10651&    25621.38&    10328.08&        7158&      157940\\
n\_BR                &       16052&    .0476576&    .3969027&           0&          14\\
n\_FS                &       16052&    .0143284&      .15918&           0&           6\\
n\_FS\_LP             &       16052&    .0091577&    .1257099&           0&           6\\
n\_FS\_CS             &       16052&    .0051707&    .0873861&           0&           4\\
County Pop.         &       16048&    88590.25&    281160.2&        1147&     9064197\\
Emp Non Legal       &       16052&    32785.33&    118582.4&          62&     3644980\\
\bottomrule
\end{tabular}
}


==> Summary_Stats/gen_sumstats_bronly.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &           N&        mean&          sd&         min&         max\\
\midrule
Legal Emp           &         448&     5029.19&     7761.03&           9&       56187\\
Legal Avg Wage      &         443&    41456.72&    9681.252&       14895&       63280\\
n\_BR                &         448&    1.707589&    1.678056&           1&          14\\
n\_BR\_LP             &         448&    .7254464&    1.050439&           0&           8\\
n\_BR\_CS             &         448&    .9821429&    1.101003&           0&           8\\
n\_FS                &         448&    .5133929&    .8081238&           0&           6\\
n\_FS\_LP             &         448&     .328125&    .6801198&           0&           6\\
n\_FS\_CS             &         448&    .1852679&      .49068&           0&           4\\
County Pop.         &         448&    917973.8&     1244072&        4044&     9064197\\
Emp Non Legal       &         448&    406210.1&    510299.8&        1074&     3644980\\
\bottomrule
\end{tabular}
}


==> Summary_Stats/tab_nfile.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccc}}
\hline\hline
                    &        freq&         pct&      cumpct\\
\hline
0                   &       15604&       97.21&       97.21\\
1                   &         313&        1.95&       99.16\\
2                   &          74&        0.46&       99.62\\
3                   &          24&        0.15&       99.77\\
4                   &          13&        0.08&       99.85\\
5                   &           9&        0.06&       99.91\\
6                   &           4&        0.02&       99.93\\
7                   &           1&        0.01&       99.94\\
8                   &           2&        0.01&       99.95\\
10                  &           5&        0.03&       99.98\\
11                  &           1&        0.01&       99.99\\
13                  &           1&        0.01&       99.99\\
14                  &           1&        0.01&      100.00\\
{hline 59}{break}Total               &       16052&      100.00&            \\
\hline\hline
\end{tabular}
}


==> Summary_Stats/tab_nfile_atleast_1_BR.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccc}}
\hline\hline
                    &        freq&         pct&      cumpct\\
\hline
1                   &         313&       69.87&       69.87\\
2                   &          74&       16.52&       86.38\\
3                   &          24&        5.36&       91.74\\
4                   &          13&        2.90&       94.64\\
5                   &           9&        2.01&       96.65\\
6                   &           4&        0.89&       97.54\\
7                   &           1&        0.22&       97.77\\
8                   &           2&        0.45&       98.21\\
10                  &           5&        1.12&       99.33\\
11                  &           1&        0.22&       99.55\\
13                  &           1&        0.22&       99.78\\
14                  &           1&        0.22&      100.00\\
{hline 59}{break}Total               &         448&      100.00&            \\
\hline\hline
\end{tabular}
}


==> To_do_list.tex <==

% \section*{to do list}
% \centering 7-12-21
% % \begin{document}[article]
% % \usepackage{hyperref}


% WHY LEGAL MARKETS MATTER
% \begin{itemize}
%     \item Legal Markets: why do we care:
%         \begin{itemize}
%             \item Account for 0.5\% of total employment BUT account for XX of wages (anything more than 3-4\% is good)
%             \item Compustat (if any) legal expenses 
%             \item Add this  \href{http://apps.olin.wustl.edu/faculty/milbourn/Investment_Legal_20180905_ssrn.pdf}{paper} (contribute to this literature by bla bla bla)
%         \end{itemize}
%     \item mention not a studied market in macro (ale)
%     \item Leg Emp Share Regs
%     \begin{itemize}
%         \item Mention in robustness and in intro maybe
%         \item lincom tests
%     \end{itemize}
%     \item Chapter 7 and 11
%     \href{https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1540-6261.2006.00872.x?casa_token=geJ73Iu2xRUAAAAA:HO-mKbicpjOdyP3ReNnLcU2c-FBSo66ukcQwG-yE5Rf-0XwRTg4t4wRHHgP0_TS_xGw3z07eI7f1KEg}
%     \item EVENT STUDY Introduction:
%         \begin{itemize}
%             \item problem of our treatment
%             \item We address these concerns in XX ways
%             \begin{itemize}
%                 \item event study
%                 \item history
%                 \item etc. 
%             \end{itemize}
%             \item Staggered adoption (heterogenous treatment).
%                 \begin{itemize}
%                     \item Linear causal effect
%                     \item NEW EVENT STUDY METHOD: \href{https://uc201f4b7f1f8f9a74fc304fa6d6.dl.dropboxusercontent.com/cd/0/inline2/BSLrv4u0PS3L9IZWaZmr68_BaWzoeuyYhIF0FVBUdB8gCAZhBhpz-9I6XvhELquNi2g7kghR8lvMynRUWsM33zQaGKkqmaLrFYU_Wt4N3O8z-_APzbphLPHk5vHJRiSM51WMejbAwX9Dyh9ziYEev6FxVs7sna1VKgVrexMhvknZLMO3ZEvlcvuuyDQBoG1H7yc2UJfyhONS-9je7rCXXb8ni68v4uQu6v5uQdM0cHlVth1YJH7KA7KgW-RUp2eoaIn8ZCKa7yR4qgQF59iR8j67HzrrrStfHnIgT4QZa0AaCvoXLmWJ3wxhI1vcYHI6SAbVWp-G093gtWThSXfNbxEEk5WBc5GGD6dCXiYBvBI8yLsaqA0GiPrv2h0IGt3rB3M/file#}{Borusyak, Jaravel, and Spiess (2021), ``Revisiting Event Study Designs: Robust and Efficient Estimation''} that consider staggered
%                 \end{itemize}
%             \item paper that discusses everything (all the approaches) \href{https://www.dropbox.com/s/rokl7clqidkkwii/ADRZ.pdf?dl=0}{paper}
%         \end{itemize}
% \end{itemize}

% \begin{itemize}
%     \item make model and struct est section connect better.
% \end{itemize}


% \newpage


% % \iffalse
% \section*{TO DO List - Finance Forum}
% Unbolded as completed.

% \begin{itemize}
%     \item Tables:
%     \begin{itemize}
%         \item We need to find a proper label for LP in the Tables.
%         \item Change n\_BR and n\_FS to proper labels.
%         \item Drop the Lincom part of the tables.  
%         \item Create one table that collects the Lincom and average effects for Table \ref{tab:MainEmpLvl}.  We need to have standard errors for the coefficients and the corresponding stars, and compute the test between N\_BR and N\_FS\_CS for the third column.  Each set of test should be a new rows. The labels for these three additional test should be: Forum Shopped Bankruptcies, Forum Shopped Bankruptcies LP and Forum Shopped Bankruptcies no-LP. This table should go to the appendix. Also each test should be accompanied for an average effect test.
        
%         \item \textbf{Make the sequence of the tables to follow the one in the text. }
%         \item Combine Tables 1 and 2 to make it in one table. Drop Max and Total.  Ideally, create the a Table that has two vertical panels one for all and the other for BR>0.
%         \item Fixed Effects references need to be more change following the next example:
        
%                 \begin{tabular}{lccccc}
%              &  &  &  &  & \tabularnewline
%             \hline 
%             Fixed Effects &  &  &  &  & \tabularnewline
%             County & Yes & Yes & Yes & Yes & Yes\tabularnewline
%             Year & No & Yes & No & No & No\tabularnewline
%             Region-Year & No & No & Yes & No & No\tabularnewline
%             State-Year & No & No & No & Yes & No\tabularnewline
%             District-Year & No & No & No & No & Yes\tabularnewline
%             \hline 
%             \end{tabular}
%     \end{itemize}
%     \item Descriptive Section
%         \begin{itemize}
%             \item Map of the BR and FR. Use the either the US tile version in R or use a map by district courts.
%             \item \textbf{Table showing the evolution by industry.}
%             \item Compute the share of BR and FS that are in NY and DE. Make sure that the descriptive tables in the paper do not include NY and DE.
%         \end{itemize}
%     \item Additional Exercises
%     \begin{itemize}
%         \item Do we have cases where all the BR are FS? If this is the case then perhaps we want to run another placebo. Estimate the impact of FS on the sample where BR==0 | BR==FS 
%         \item \textbf{Local conditions do not predict a BR in our dataset. }
%         \begin{itemize}
%             \item Running some regressions where $BR$ is our dependent variables and we use some local economy indicators such as unemployment rate, change in the number of non-legal establishments, change in gdp, change in number of employed people, etc.  Use our baseline fixed effects. SEE TABLE \ref{tab:BR_LocalConditions}
%             \item \textbf{ What are the early indicators of recessions in the macro literature? Are any of this at the county level? Make a list of this early indicators such that we discuss how we are controlling for them and how they do not predict a BR in our sample.
%             https://www.bea.gov/data/gdp/gdp-county-metro-and-other-areas change in gdp USE PERSONAL INCOME AS PROXY CITE ECONOMETRICA PAPER The Aggregate Implications of Regional Business Cycle }
%             \begin{itemize}
%                 \item During our main sample, we don't have county gdp.
%                 \item An alternative is to use this measure later in our sample, but we don't have the data processed yet.
%             \end{itemize}
%         \end{itemize}
%         \item Estimate the impact using the number of establishments in the legal sector as our dependent variable. http://www.fpeckert.me/cbp/ USE ESTAB DATA. Update: not working. 

%         \item Compute the number of business that close/open in the county outside of the legal sector and include them as additional controls.
        
%         \item Which measure of wage are we using quarter or annual? Estimate the impact using the one that we are not including in our current tables. \textbf{UPDATE: We don't have all the data for BR dates and FR dates. We might be able to collect most of them. Also, we don't have a lot of controls.}
        
%         \item Estimate the impact of BR and FR in the employment level of the counties where the district court are located. \textbf{Count the number of BR and FS for the district courts and estimate the same regressions focusing on the counties that have a district court.} Update: There are more courts than districts so we need a way to split the counts. This is not straight forward to do.
%         \item Replace Regions with Divisions in the table (or add divisions into the set of columns)
%         \item Local effect tests.  We did a regression that captures an indicator for BR in adjacent counties. \\ Run a regression where the control group is counties adjacent to a BR at some time in our sample. SEE TABLE \ref{tab:RBST_ADJBR_BR_Counties90_97_OmitNYDE} AND 
%         % \ref{tab:RBST_ADJBR_BR_Counties90_01_OmitNYDE}
%         \item Drop Column (4) for Wage Results and Update the text accordingly.
%     \end{itemize}
%     \item Robustness Check: 
%     \begin{itemize}
%       \item \textbf{Create a broader subsections inside Robustness, 
%       \\ COMBINE "TREATED COUNTY SAMPLE", "COUNTIES WITH FIRM HEADQUARTERS", AND "COUNTIES WITH BANKRUPTCY COURTS" INTO 1 SECTION FOR MORE RELEVANT COMPARISON GROUPS.} 
%         \item Rewrite the bullets on the robustness section to make it paragraphs that connect each other.
%         \item \textbf{Review: Make sure that the empirical methodology details all our analysis that we include in the robustness section.}
%     \end{itemize}
%     \item Data Work:
%         \begin{itemize}
%             \item Scrape data so that CS forum shopping captures in district shops like the LP database does. \textbf{Update: In-district FR is a big problem here. There is not a way to identify this clearly. LP is now aligned with CS FR.}
%         \end{itemize}
%     \item Mechanism Section
%     \begin{itemize}
%         \item \textbf{Fix graphs (replace $\overline{L}_{BR} \text{ with } \overline{L}$)}
%         \item \textbf{tie the writing to the data/results more than the model. }
%     \end{itemize}
    
% \end{itemize}
% % \fi

% % \iffalse
% \section*{TO DO List - Adopt a Paper}

% \begin{itemize}
%     \item Intro: All. Postpone for later.
%     \item Lit Review: AP,CB 
%     \item Forum Shopping:  AP, CB. Parts goes to the appendix.
%     \item Model \& Mechanism: AP, CB.
%     \item Empirical Methodology
%     \begin{itemize}
%         \item \textbf{X} Database construction: CB
%         \item Additional Exercises: CB.
%         \begin{itemize}
%             \item \textbf{X} Placebo: CB.
%             \item Event Study. This is after the structural estimation is ``done''.  CB
%         \end{itemize}
%         \item Threats  to Identification:
%         \begin{itemize}
%             \item Overall review: JC
%             \item Add Placebo and Event Study: JC
%         \end{itemize}
%     \end{itemize}
%     \item Results: JC, All. 
%     \item Structural Estimation: AP.
%     \item Conclusion: All. Low priority.
%     \item Tables and Figures: CB. 
%     \item Appendix
%     \begin{itemize}
%         \item Descriptive Statistics: plot of number of bankruptcy and forum shop over time
%     \end{itemize}
% \end{itemize}
% \newpage
% % \fi
% %\end{comment}


% examples: \textbf{TRUMP}, lots of airlines, \textbf{MARVEL}, harrahs hotel chain


% \subsection*{Alternative Outline of the paper}

% \textbf{CHADS VERSION 6/23}
% \begin{enumerate}
%     \item Introduction
%     \item Forum Shopping
%     \begin{itemize}
%         \item Move FS trend stuff from descriptive stats to here!
%     \end{itemize}

%     \item Empirical Methodology and Identification Challenges
%         \begin{enumerate}
%             \item Challenges to identification
%                 \begin{itemize}
%                     \item BR exogenous to local conditions\\ \textit{``The first econometric challenge is to identify if the underlying local economic conditions drive firms to file for bankruptcy. In that case, certain omitted variables (e.g., reduced local demand) could affect the firm and the corresponding county's municipal bond yields''}
%                     \item confounding factors? FS
%                     \item Equal pretrends  (placebo) (Fuzzy did?)
%                     \item Counterfactual scenario \textbf{(Matching? Nearest neighbor in euclidian distance?) }
%                 \end{itemize}
%         \end{enumerate}
%     \item Data \;\;(either in methodology section or on its own)
%     \item Results\\
%     present main results on BR
%         \begin{enumerate}
%             \item Forum shopping
%             \item Robustness Checks
%             \item Wage
%         \end{enumerate}
%     \item Model 
%         \begin{itemize}
%             \item shorten if possible        
%             \item drop mechanism section
%         \end{itemize}
%     \item Structural Estimation  
% \end{enumerate} 
% \newpage
% \begin{enumerate}
%     \item Introduction
%     \item Forum Shopping
%     \item Database construction
%     \item Reduced Form Impact with puzzling results
%     \item Model 
%     \item Structural Estimation  
% \end{enumerate} 

% \subsection*{Outline Methodology}



% \begin{enumerate}
%     \item OLS regression model with fixed effects. 
%     \item Sample all counties of the US besides NY and DE. 
%     \item Forum shopping to interpret our results as bankrupcty impact. 
%     \item Placebo to further support our interpretation.
%     \item Exogeneity of bankruptcies for big firms. 
%     \item Robustness:
%     \begin{itemize}
%         \item Sample 1: counties with HQ.
%         \item Sample 2: include NY and DE.
%         \item Sample 3: drop 1991 due to recession.  
%         \item Measurement: counts and dummies. 
%         \item Fixed Effects
%         \item Controls: Lags and additional controls. 
%         \item Spillovers
%         \item BLS data
%     \end{itemize}
%     \item Wage Impact
% \end{enumerate}
% % \fi
% % KODAK FEES: https://www.reuters.com/article/us-kodak-bankruptcy/kodak-bankruptcy-advisers-likely-to-see-240-million-payday-idUSBRE9AD1DV20131114
% % KODAK CASE: https://www.kccllc.net/kodak
% \newpage

% \section*{Outline of the Intro (everything after paragraph }
% \begin{itemize}
% \item \textbf{Event study fail} Unlike much of the literature that exploits an event study frame work, our setting is not conducive to such methods due to transitory, continuous and repeated treatment (CITATIONS ABOUT EVENT STUDY LITERATURE THAT SAYS). 
% \begin{itemize}
%     \item \textcolor{red}{\textbf{Callaway and Sant'Anna (Journal of Econometrics, 2020): Difference-in-Differences with Multiple Time Periods} \\ \textit{Assumption 1 (Irreversibility of Treatment):
% Assumption 1 states that no one is treated at time t = 1; and that once a unit becomes treated,
% that unit will remain treated in the next period}\\ \citet{callaway_difference--differences_2020}}
%     \item \textcolor{red}{\textbf{Sun and Abraham (Journal of Econometrics, 2020): Estimating Dynamic Treatment Effects in Event Studies with Heterogeneous Treatment Effects.}\\ \textit{In the general case of event studies we focus on an absorbing treatment such that the treatment status
% over time is a non-decreasing sequence of zeros and then ones....}\\ \citet{sun_estimating_2020}}
% \end{itemize}
% \item \textbf{Economic History Approach} For this reason we turn to economic history approach and use stipulations of the law to create variations (CITATIONS: \textcolor{red}{NEED A CITATION THAT CAN'T DO EQUAL PRETRENDS DUE TO MESSY TREATMENT.})\\
% \textbf{TO DO LIST}
% \begin{itemize}
%     \item Create excel files with papers on each row and columns:
%     \begin{itemize}
%         \item Paper Title, 
%         \item Journal
%         \item Abstract,
%         \item Shock description, 
%         \item One time (0) vs Continuous (1) Treatment,
%         \item Transitory (0) vs Permanent (1) Effect on Treated, 
%         \item Restrict Period to get identification Y/N, 
%         \item Identification strategy
%     \end{itemize}
%     \item Put papers in a library folder IDENTIFICATION. \textcolor{red}{SEE GOOGLE DRIVE: ForumShopping/Related Literature/History Lit}
% \end{itemize}

% \item  \textbf{Theoretical Econometric Approach} We complement this approach by exploiting recent improvements in the theoretical identification literature..  fuzzy approach (CITATIONS)
% \textbf{TO DO LIST:} Just add papers that Jeronimo mentioned.
% \begin{itemize}
%     \item \textcolor{red}{\citet{de_chaisemartin_two-way_2020} \\Stata commands: twowayfeweights, fuzzydid and did\_multiplegt}
% \end{itemize}


% \item \textbf{Why Reorganization and not also liquidations} 
% \begin{itemize}
%     \item To OPERATIONALIZE our identification strategy we focus our attention on bankruptcy REORGANIZATIONS (where forum shopping happens). 
%     \item Reorganizations are legal service intensive
%     \item In terms of shock size they involve larger bankruptcies (larger shocks)
% \end{itemize}

% \item \textbf{Incidental Contributions} In doing so we make two contributions
% \begin{itemize}
% \item First we extend database. DATA CONTRIBUTION PARAGRAPH HERE: we collect database and extend lopucki etc
% \item Incidentally, we contribute to the bankruptcy literature that has focused on the effect of forum shopping on bankruptcy outcome at general equilibrium
% \end{itemize}
% \item \textbf{Main findings} Findings on employment
% \begin{itemize}
%     \item additional exercises
%     \begin{itemize}
%         \item BR exogenous to local condition reg
%         \item placebo
%         \item tests and avg effects
%     \end{itemize}
%     \item all robustness
%     \begin{itemize}
%         \item Include NY and DE
%         \item leg emp and br 1991-2001
%         \item counties with firm HQ
%         \item counties with br court br and fs version
%         \item lagged controls
%         \item control for unemp
%         \item control for non legal estab
%         \item drop 1991 (wage and emp)
%         \item dummy version
%         \item alternative data source
%         \item fixed effects
%         \item counties with br at some point
%         \item counties with br or were adjacent to br at some point
%         \item adjacent county br
%     \end{itemize}
% \end{itemize}
% \item \textbf{Puzzle on Wages} Countervailing effect on wages
% \item \textbf{Model} Rationalize using model that allows:
% \begin{itemize}
%     \item to rationalize drop in wages
%     \item clarifies identification strategy
%     \item Structural Estimation
    
%     \textbf{TO DO LIST}
% \begin{itemize}
%     \item Create excel files with papers on each row and columns:
%     \begin{itemize}
%         \item Paper Title, 
%         \item Journal
%         \item ELASTICITY LB
%         \item ELASTICITY UB
%         \item Estimate 
%         \item Model CES (1/0)
%         \item Dynamic (1) static (0) (Adjustment Cost)
%         \item Skilled Intensive
%         description, 
%         \item Data
%     \end{itemize}
%     \item Put papers in a library folder STRUCTESTIMATION
% \end{itemize}
%     % \begin{itemize}
%         \item \textcolor{red}{\citet{blankenau_industry_2011} Only source of industry level estimates.
%     \begin{itemize}
%         \item \begin{quote}
%             \textit{``We find that the elasticity of substitution calculated from aggregate data tends to underestimate this substitutability. Nine of 13 industries have elasticities in excess of that measured by Katz and Murphy (1992).''(\citet{katz_changes_1992})}
%         \end{quote}
%         \item \begin{quote}
%             \textit{``A striking feature of the elasticity measures is that each positive measure is much larger than the 1.396 estimate for the aggregate model. The smallest estimate is 2.217, the largest is over 500, and the median is 7.988. Qualitatively, this result can be reconciled by noting that when one industry experiences an increase in the wage ratio, it may respond by hiring the most appropriate unskilled labour from another industry. This is a margin unavailable to the economy as a whole, which constrains the aggregate elasticity estimate. Thus we would expect that industry specific elasticities would, on average, exceed the aggregate elasticity''}
%         \end{quote}
%     % \end{itemize}
%     \end{itemize}}
    
    
% \end{itemize}
% \end{itemize}
% \newpage 


\begin{center}
    \textbf{ \underline{IMPORTANCE OF LEGAL INDUSTRY STATS}}
\end{center}
\begin{itemize}
    \item PAPER ABOUT LEGAL INDUSTRY: \citet{bennett_corporate_2018}
    \item \textbf{MAY 2020} TotEmp=139099570 MeanWage=56310 $\implies$ TotWage = 7.832697 trillion   \url{https://www.bls.gov/oes/current/oes_nat.htm}\\ LegEmp=1137670 LegMeanWage=92180 $\implies$ TotLegWage=104.87 billion \url{https://www.bls.gov/oes/current/naics4_541100.htm}\\
    \textbf{\underline{\large Legal Industry: 1.3\% of wages and 0.8\% of emp}}. \\ (MAY 2020 COVID: tried it with may 2019 data. almost exact same shares)
    \item Legal industry in US generated 256.66 bill in revenue in 2013, expected to be 288 bil by 2018. Market size of US corporate legal departments 160 bil in 2016 \url{https://www.statista.com/topics/2137/legal-services-industry-in-the-us/}
    
    Real estate: \url{https://www.statista.com/forecasts/885066/real-estate-and-rental-and-leasing-revenue-in-the-us}
    Education services: \url{https://www.statista.com/forecasts/311190/educational-services-revenue-in-the-us} \\~\
    
    GDP legal services: \url{https://fred.stlouisfed.org/series/USLEGALRGSP}\\
    GDP agriculture: \url{https://fred.stlouisfed.org/series/USAGRRQGSP}\\~\
    
    GDP legal nominal: \url{https://fred.stlouisfed.org/series/USLEGALNGSP} \\
    GDP agriculture nominal: \url{https://fred.stlouisfed.org/series/USAGRNQGSP}
    %GDP real estate: \url{https://fred.stlouisfed.org/series/USRERENTLEARQGSP}
    
    Legal industry GDP (nom) larger than agriculture . 
    
    \item The authors write that “over the last 25 years government data shows legal services constitute a slightly larger proportion of the nation’s GDP – now nearly 2 percent – with no hint of decline.” Let’s assume that “legal services” means work done by law firms, that our gross domestic product in 2009 was \$14.5 trillion, and that “nearly 2 percent” is 1.9\%. That calculation says \$280 billion paid for “legal services.” \\ \url{https://www.lawdepartmentmanagementblog.com/gdp-figures-legal-services-spend-and-fees-per-inside-lawyer-on-law-firms-dont-mesh/}
    \url{https://heinonline.org/HOL/Page?collection=journals&handle=hein.journals/abaj97&id=501&men_tab=srchresults}
    \item Lehman Brothers Ch11 bankruptcy spent 2.56 billion on legal consulting and professional fees. 
    \textit{Source:} \href{https://libertystreeteconomics.newyorkfed.org/2019/01/lehmans-bankruptcy-expenses/}{New York Fed}. This is most expensive BR in history (5.9 bil) and these fees make up \%43.39 (a plurality) of the cost  \\ \textit{Source:}\href{https://www.wsj.com/articles/fed-says-lehman-brothers-chapter-11-case-is-costliest-in-history-11547673357}{WSJ}.   
\end{itemize}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
    \textbf{ \large\underline{RECENT FORUM SHOPPING LEGISLATION}}
\end{center}
\begin{itemize}
    \item 
        \textbf{This has been proposed 3 times recently:} 
        \begin{enumerate}
            \item  \href{https://www.govtrack.us/congress/bills/116/hr4421}{2019-House of representatives- Did not receive vote (died)}
            \item \href{https://www.govtrack.us/congress/bills/116/s5032}{2020- Senate- Did not reveive vote (died)} 
            \item \href{https://www.govtrack.us/congress/bills/117/hr4193}{June 28, 2021- TBD still happening!} 
        \end{enumerate}
    \item 
        \textbf{Quotes from press conference of congress people who proposed 2021 bill}
        \url{https://lofgren.house.gov/media/press-releases/lofgren-buck-introduce-bipartisan-legislation-end-corporate-bankruptcy-forum}
        \begin{quote}
            \textit{``The outcome of a Chapter 11 bankruptcy proceeding can have a profound impact on the local community where a corporation is based. It is simply unfair that corporations can game the bankruptcy system by choosing a distant court where there is a cottage industry to advantage their interests. Justice is best served when corporate bankruptcies are adjudicated locally, with convenient court access for employees, retirees, and local creditors and a judge who knows the affected community''} \\-Rep. Zoe Lofgren
        \end{quote}
        \begin{quote}
            \textit{“Under current U.S. law, corporations filing Chapter 11 bankruptcy have the ability to “venue shop” and potentially choose a court that has issued lenient rulings in similar cases. Our bill will require corporations filing Chapter 11 bankruptcy to go through those proceedings in the forum they are primarily located rather than running off to a court across the country. This will eliminate companies’ ability to tilt the scale of justice and ensure the case is heard in a court familiar with all the affected stakeholders,”} \\-Rep. Ken Buck
        \end{quote}
    \item 
        \textbf{Does not look likely to pass}\\
        \textit{"Although the Reform Act is a bi-partisan bill, it seems to have little prospect of success. The bill does not yet have a Senate companion and seems unlikely to get out of committee in the House given that the Chair of the Judiciary Committee is Rep. Jerrold Nadler of New York (one of the decried “magnet districts”)."} \url{https://www.sewkis.com/publications/bankruptcy-venue-reform-redux/}
    \item August 6, 2021 news article \url{https://thehill.com/blogs/congress-blog/judicial/566729-now-is-the-time-for-bankruptcy-venue-reform}
    \item August 23, 2021 news article 
    \url{https://www.natlawreview.com/article/bankruptcy-venue-between-rock-and-hard-place}
\end{itemize}

\newpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


LA COUNTY during our sample 4054 jobs per year
440 million in wages per year for those jobs.






